FlipLLM: Efficient Bit-Flip Attacks on Multimodal LLMs using Reinforcement Learning

Generative Artificial Intelligence models, such as Large Language Models (LLMs) and Large Vision Models (VLMs), exhibit state-of-the-art performance but remain vulnerable to hardware-based threats, specifically bit-flip attacks (BFAs). Existing BFA discovery methods lack generalizability and struggle to scale, often failing to analyze the vast parameter space and complex interdependencies of modern foundation models in a reasonable time. This paper proposes FlipLLM, a reinforcement learning (RL) architecture-agnostic framework that formulates BFA discovery as a sequential decision-making problem. FlipLLM combines sensitivity-guided layer pruning with Q-learning to efficiently identify minimal, high-impact bit sets that can induce catastrophic failure. We demonstrate the effectiveness and generalizability of FlipLLM by applying it to a diverse set of models, including prominent text-only LLMs (GPT-2 Large, LLaMA 3.1 8B, and DeepSeek-V2 7B), VLMs such as LLaVA 1.6, and datasets, such as MMLU, MMLU-Pro, VQAv2, and TextVQA. Our results show that FlipLLM can identify critical bits that are vulnerable to BFAs up to 2.5x faster than SOTA methods. We demonstrate that flipping the FlipLLM-identified bits plummets the accuracy of LLaMA 3.1 8B from 69.9% to ~0.2%, and for LLaVA's VQA score from 78% to almost 0%, by flipping as few as 5 and 7 bits, respectively. Further analysis reveals that applying standard hardware protection mechanisms, such as ECC SECDED, to the FlipLLM-identified bit locations completely mitigates the BFA impact, demonstrating the practical value of our framework in guiding hardware-level defenses. FlipLLM offers the first scalable and adaptive methodology for exploring the BFA vulnerability of both language and multimodal foundation models, paving the way for comprehensive hardware-security evaluation.

==> Sections/Sec1_Introduction.tex <==
\section{Introduction}

The emergence of Large Language Models (LLMs) has fundamentally transformed the landscape of artificial intelligence, demonstrating unprecedented capabilities in natural language understanding, generation, and complex reasoning tasks \cite{brown2020language}. These models now serve as the backbone for critical applications across healthcare diagnostics, financial analysis, and autonomous systems \cite{zhang2020pegasus, bommasani2021opportunities}. However, their increasing deployment in high-stakes environments has raised crucial questions about their vulnerability to adversarial attacks, particularly at the hardware level where traditional security measures may prove insufficient \cite{hong2019terminal}.

Among hardware-based threats, bit-flip attacks (BFAs) represent a particularly insidious challenge. By exploiting physical vulnerabilities in DRAM through techniques like Rowhammer \cite{kim2014rowhammer}, attackers can modify model parameters stored in memory without requiring direct access to the system. Recent advances have demonstrated that even remote execution of such attacks is feasible \cite{cojocar2020we}, dramatically expanding the threat surface for deployed models. While BFAs have been extensively studied in traditional neural networks \cite{rakin2019bit}, their application to LLMs presents unique challenges due to the astronomical size of the parameter space and the intricate architecture of transformer models.

Current approaches to identifying vulnerable parameters in LLMs typically rely on gradient-based methods or progressive parameter search \cite{zhao2019fault}. However, these techniques face severe scalability limitations when applied to modern language models with billions of parameters. Gradient-based methods often struggle with the discrete nature of bit flips and may fail to capture complex interactions between parameters. Meanwhile, progressive search becomes computationally intractable due to the combinatorial explosion of possible bit combinations. Furthermore, existing methods frequently require architecture-specific modifications, limiting their applicability across the diverse ecosystem of transformer models \cite{hong2019terminal}.

We address these challenges by introducing a novel reinforcement learning framework for optimizing bit-flip attacks on LLMs. Our approach reframes the parameter search problem as a sequential decision-making process, where an RL agent learns to identify critical bits that maximize performance degradation while minimizing the number of required flips. This formulation offers several key advantages: (1) it efficiently explores the vast parameter space through learned policies rather than exhaustive search, (2) it naturally adapts to different model architectures by learning from interaction rather than relying on architectural assumptions, and (3) it captures complex dependencies between parameters through its sequential decision process.

Our framework comprises three key components: (1) a parameter sensitivity analyzer that identifies promising regions of the weight space, (2) an RL environment that simulates bit-flip attacks and provides feedback on their effectiveness, and (3) a Q-learning agent that learns optimal attack strategies through experience. By combining these elements, our method can discover highly effective attack points with significantly reduced computational overhead compared to existing approaches.

Experimental results on the TinyLlama model demonstrate the efficacy of our approach. Using our RL framework, we achieve a 45\% reduction in model performance with just five bit flips, compared to traditional methods requiring 15-20 flips for similar degradation. Importantly, our method accomplishes this while requiring only 10\% of the computational resources needed by gradient-based approaches. Further analysis reveals that our RL agent learns to target specific attention mechanisms and layer normalization parameters, providing new insights into the vulnerability patterns of transformer architectures.

The contributions of our work include:
\begin{itemize}
    \item A novel RL formulation of the bit-flip attack optimization problem that efficiently handles the challenges of vast parameter spaces in LLMs
    \item A scalable, model-agnostic framework that combines parameter sensitivity analysis with reinforcement learning to identify critical bits for flipping
    \item Comprehensive empirical evaluation demonstrating superior attack efficiency with reduced computational overhead
    \item New insights into the vulnerability patterns of transformer architectures, revealed through analysis of our RL agent's learned policies
\end{itemize}

Beyond immediate security implications, our work contributes to the broader understanding of robustness in neural architectures and highlights the potential of reinforcement learning in security optimization tasks. The framework we present not only advances the state-of-the-art in hardware-based attacks but also provides a foundation for developing more resilient model architectures and deployment strategies.


==> Sections/Sec2_Background_Relatedworks.tex <==
\section{Background}

% This section provides an overview of approximate computing in DNNs, fault tolerance techniques, and the challenges that arise at their intersection. We then position our work within this context, highlighting the need for novel approaches in fault detection and mitigation for AxDNNs.


% \begin{figure}[!t]
% 	\centering
% 	\vspace{-0.01in}
%         \includegraphics[width=1\linewidth]{Figs/framework_aps.pdf}
% 	%\vspace{-0.16in}
% 	\caption{Proposed Framework APS for AxDNN hardware fault detection and mitigation}
% 	\label{fig:method_aps}
% 	\vspace{-0.2in}
% \end{figure}



% \subsection{Approximate Computing in DNNs}
% Approximate computing has emerged as a promising paradigm to address the increasing computational demands of DNNs, offering significant energy savings and performance improvements \cite{mittal2016survey}. This approach exploits the inherent error resilience of DNNs, allowing for reduced precision computations and simplified hardware designs \cite{zhang2015approximate}. Recent advancements in approximate DNN accelerators have demonstrated substantial efficiency gains. For instance, Jouppi et al. \cite{jouppi2017datacenter} showed that custom accelerators using reduced precision can achieve significant performance improvements.

% However, these benefits come at the cost of increased vulnerability to hardware faults \cite{reagen2018ares}. In approximate computing environments, hardware faults present unique challenges. Unlike software-level approximations, which are controlled and predictable, hardware faults can introduce random and potentially severe errors \cite{li2017understanding}. These faults can manifest as bit flips in memory, timing violations, or computational errors in arithmetic units \cite{zhang2018thundervolt}.

% \subsection{Fault Tolerance in Deep Neural Networks}

% As DNNs increasingly power critical applications, ensuring their reliability in the face of hardware faults has become paramount. While DNNs exhibit an inherent resilience to certain types of faults due to their distributed representations and non-linear activations \cite{torres2017fault}, they remain vulnerable to critical faults that can significantly degrade performance, particularly in resource-constrained or approximate computing environments \cite{li2017understanding}.

% Recent studies have explored various fault tolerance strategies specific to DNNs:

% \begin{itemize}
%     \item Selective neuron hardening identifies and protects critical neurons through sensitivity analysis \cite{schorn2018efficient}.
%     \item Fault-aware pruning enhances robustness by strategically removing vulnerable connections \cite{he2020fault}.
%     \item Error-resilient training incorporates fault injection during the training process to improve the network's tolerance to hardware errors \cite{kim2019matic}.
%     \item Algorithmic noise tolerance leverages the error-tolerant nature of DNNs to design architectures that can operate correctly even in the presence of computational errors \cite{temam2012algorithmic}.
% \end{itemize}

% However, the effectiveness of these approaches in the context of approximate computing, where errors can be more severe and unpredictable, remains to be thoroughly investigated.

% \subsection{Challenges at the Intersection of Approximation and Fault Tolerance}

% The integration of approximate computing into AI systems introduces critical challenges in maintaining system reliability, particularly in the presence of hardware faults. These challenges stem from the fundamental tension between the intentional imprecision introduced by approximate computing and the need for reliable, accurate results in AI applications.

% One primary challenge is distinguishing between approximation errors and hardware faults. Approximate computing intentionally introduces imprecision into the computation process to reduce power consumption and increase efficiency. This intentional deviation from exact computation can be difficult to distinguish from hardware faults, as approximation errors may exhibit similar characteristics to faults induced by hardware issues \cite{li2017understanding}.

% Another significant challenge is balancing energy efficiency and reliability in approximate computing environments. Traditional fault tolerance methods, such as Error Correction Codes (ECCs) and Triple Modular Redundancy (TMR), often come at the cost of increased computation, memory, and power overheads, which can negate the energy savings achieved through approximate computing \cite{kim2020matic}. This creates a paradox where the very methods meant to ensure reliability might counteract the efficiency benefits of approximate computing.

% Furthermore, the degree of fault tolerance required is highly application-specific, with safety-critical applications demanding stringent reliability guarantees. This makes the trade-offs between efficiency and reliability especially challenging to manage in the deployment of DNNs on approximate hardware \cite{reagen2018ares}.

% \subsection{The Need for Novel Approaches}

% The interplay between approximate computing and hardware fault tolerance in DNNs remains largely unexplored. Existing studies have primarily focused on software-level resilience \cite{koppula2019eden}, leaving a critical gap in addressing hardware-level faults in approximate DNN accelerators. Conventional fault detection mechanisms, designed for exact computing environments, may either fail to detect hardware faults or misclassify approximation errors as critical faults, leading to missed detections or an excess of false positives.

% This underscores the need for novel, lightweight approaches to fault detection and mitigation that can operate efficiently within the constraints of approximate computing systems while addressing the unique challenges posed by hardware faults. Such approaches must strike a delicate balance between maintaining the energy efficiency benefits of approximate computing and ensuring the reliability necessary for critical applications.

% Our work addresses this gap by introducing a novel method for fault detection and mitigation in DNNs running on approximate hardware. By leveraging targeted correction techniques only when critical faults are detected, our approach aims to minimize computational overhead while preserving the benefits of approximate computing and ensuring network reliability.




% The rise of artificial intelligence and deep learning has driven the need for innovative computational strategies, with approximate computing emerging as a promising solution. By capitalizing on the inherent error resilience of DNNs, approximate computing offers substantial energy savings and performance enhancements through reduced precision operations and simplified hardware designs \cite{mittal2016survey, 7348659}. Notably, custom accelerators utilizing reduced precision have demonstrated significant efficiency gains \cite{jouppi2017datacenter}.

% Despite these benefits, approximate computing introduces a heightened susceptibility to hardware faults, which can manifest as unpredictable and severe errors \cite{li2017understanding}. These faults, including bit flips and timing violations, pose unique challenges distinct from the controlled imprecision of software-level approximations \cite{zhang2018thundervolt}.
% Ensuring the reliability of DNNs in the presence of hardware faults is critical, especially as these networks are increasingly deployed in mission-critical applications. Traditional fault tolerance strategies such as selective neuron hardening, fault-aware pruning, and error-resilient training have been explored to enhance robustness \cite{schorn2018efficient, jiang2024classawarepruningefficientneural, kim2018maticlearningerrorsefficient}. However, their applicability in approximate computing environments, where errors can be more severe and unpredictable, necessitates further investigation.

% The integration of approximate computing with AI systems presents a fundamental challenge: distinguishing between intentional approximation errors and hardware-induced faults. This distinction is crucial for maintaining reliability without undermining the energy efficiency gains of approximate computing \cite{li2017understanding}. Conventional methods, such as Error Correction Codes (ECCs) and Triple Modular Redundancy (TMR), often introduce significant overheads, counteracting the benefits of approximate computing \cite{9174137, CHEREZOVA2023115010}.
% Given these challenges, there is a pressing need for novel approaches to fault detection and mitigation that are tailored to the unique demands of AxDNNs. Existing solutions primarily address software-level resilience \cite{koppula2019eden}, leaving a critical gap in addressing hardware-level faults. Our research addresses this gap by introducing a JIT fault detection and mitigation strategy for AxDNNs, leveraging advanced statistical techniques to maintain energy efficiency while ensuring system reliability.




% % \section{Background and Related Work}

% % \subsection{Approximate Computing in DNNs}
% The exponential growth in artificial intelligence applications has intensified the need for energy-efficient computing paradigms, with approximate computing emerging as a promising solution for DNNs. 
% This approach leverages the inherent error resilience of DNNs to achieve substantial energy savings through reduced precision operations and simplified hardware designs \cite{mittal2016survey, 7348659}. Recent implementations of approximate computing in custom accelerators have demonstrated remarkable efficiency gains, with some architectures achieving up to 30x improvement in energy efficiency \cite{jouppi2017datacenter}. However, this efficiency comes at the cost of increased susceptibility to hardware faults, which can manifest as unpredictable errors distinct from controlled approximation-induced variations \cite{li2017understanding}.

% \subsection{Fault Tolerance in Approximate Computing}
% Traditional fault tolerance approaches in DNNs encompass various strategies, including selective neuron hardening, fault-aware pruning, and error-resilient training \cite{schorn2018efficient, jiang2024classawarepruningefficientneural}. These methods typically focus on maintaining accuracy under specific fault conditions. However, their effectiveness in approximate computing environments presents unique challenges, particularly in distinguishing between intentional approximation errors and hardware-induced faults. Conventional fault tolerance methods such as Error Correction Codes (ECCs) and Triple Modular Redundancy (TMR) often introduce prohibitive overhead, negating the energy benefits of approximate computing \cite{9174137, CHEREZOVA2023115010}.

% \subsection{Multi-Exit Neural Networks}
% Multi-exit neural networks represent a significant advancement in DNN architecture design, offering both efficiency and inherent fault tolerance capabilities \cite{kaya2019shallow}. For a multi-exit network $F$ with $N$ exits, each exit $i$ provides a prediction for input $x$, enabling early termination when sufficient confidence is achieved. Formally, the network terminates at exit $i$ if:

% \begin{equation}
%     \max(F_i(x)) > \gamma
% \end{equation}

% where $\gamma$ is a predetermined confidence threshold. This architecture is particularly relevant for fault-tolerant computing as it provides multiple redundant paths for prediction, allowing the network to maintain reliability even when certain exits are affected by hardware faults.

% \subsection{Statistical Fault Detection}
% Recent approaches to fault detection in DNNs have explored statistical techniques for distinguishing between normal operational variations and fault-induced errors. These methods typically employ various uncertainty quantification approaches, including Bayesian techniques and dropout-based methods \cite{koppula2019eden}. However, existing solutions primarily address software-level resilience, leaving a critical gap in handling hardware-level faults in approximate computing environments. Our research addresses this limitation by introducing a just-in-time (JIT) fault detection and mitigation framework that leverages statistical pattern analysis to maintain both energy efficiency and system reliability.

% The integration of these concepts—approximate computing, fault tolerance, multi-exit architectures, and statistical detection—presents unique opportunities and challenges in developing robust AI systems. While approximate computing offers significant energy benefits, ensuring reliable operation under hardware faults requires novel approaches that can effectively distinguish between intentional approximations and harmful faults while maintaining the energy efficiency advantages of approximate computing.


%The rapid expansion of AI applications has heightened demand for energy-efficient paradigms, positioning approximate computing as a promising solution that exploits DNNs' error resilience for energy savings while necessitating robust fault detection to address increased hardware fault susceptibility \cite{mittal2016survey, 7348659}.

\subsection{Statistical Fault Detection}
% Traditional fault tolerance approaches such as Error Correction Codes (ECCs) and Triple Modular Redundancy (TMR) often introduce prohibitive overheads, counteracting the benefits of approximate computing \cite{9174137, CHEREZOVA2023115010}. Recent advances in uncertainty quantification offer more efficient solutions through energy-based methods, Bayesian DNN, and Monte Carlo Dropout \cite{schorn2018efficient}, which can effectively discriminate between observed and unobserved data distribution. These methods provide a crucial metric for fault detection, typically exhibiting higher values for anomalous inputs caused by hardware faults. This approach enables efficient fault detection while maintaining the energy benefits of approximate computing, particularly in multi-exit neural networks where alternative computational paths can be leveraged for enhanced reliability \cite{jiang2024classawarepruningefficientneural, kim2018maticlearningerrorsefficient}. Our research builds upon these foundations to develop a novel JIT fault detection strategy that balances energy efficiency with system reliability in AxDNNs.
Conventional fault tolerance methods, such as Error Correction Codes (ECCs) and Triple Modular Redundancy (TMR), often impose significant overheads, undermining the advantages of approximate computing \cite{9174137, CHEREZOVA2023115010}. A comprehensive list of such techniques for AccDNN fault detection and mitigation can be found in \cite{fault-1,fault-2}. There are also recently proposed AccDNN fault repair methods that suffer from the burden of retraining \cite{retrain-1, retrain-2, 10028723}. In contrast to these methods, advances in uncertainty quantification offer more efficient alternatives, including energy-based methods \cite{liu2021energybasedoutofdistributiondetection}, Bayesian DNNs \cite{gal2016dropoutbayesianapproximationrepresenting}, and Monte Carlo Dropout \cite{kendall2017uncertaintiesneedbayesiandeep}, which can effectively distinguish between observed and unobserved data distributions. These techniques leverage metrics, such as the energy score, epistemic and aleatoric uncertainty, etc., that typically exhibit elevated values for anomalous inputs that may have been caused by hardware faults, enabling precise fault detection. 
% \textcolor{blue}{These methodological approaches predominantly focus on software-level resilience mechanisms, thereby presenting a substantial lacuna in comprehensive fault detection and mitigation strategies for hardware-level perturbations within approximate computing paradigms. Our research introduces a novel JIT fault detection and mitigation framework that systematically leverages statistical pattern analysis to simultaneously optimize energy efficiency and ensure computational reliability in inherently stochastic computational environments.}

\subsection{Multi-Exit Neural Networks}
Multi-exit neural networks represent a significant advancement in DNN architecture design, offering both efficiency and inherent fault tolerance capabilities \cite{kaya2019shallow}. For an approximate multi-exit network $F$ with $N$ exits, each exit $i$ provides a prediction for input $x$, enabling early termination when sufficient confidence is achieved. Formally, the network terminates at exit $i$ if $\max(F_i(x)) > \gamma$, where $\gamma$ is a predetermined confidence threshold. This architecture is particularly relevant for fault-tolerant computing as it provides multiple redundant paths for prediction, allowing the network to maintain reliability even when certain exits are affected by hardware faults.  Building on these statistical methods and multi-exit neural network principles, our research introduces a novel JIT fault detection strategy that optimally balances energy efficiency and system reliability in AxDNNs.
% \textcolor{blue}{While existing studies have employed multi-exit networks for fault detection and mitigation \cite{kundu2024mendnet}, these efforts have primarily focused on AccDNN without considering the nuanced requirements of approximate computing environments. To the best of the authors' knowledge, no prior research has systematically explored the application of multi-exit networks for fault management in AxDNNs.}

==> Sections/Sec3_Methodology.tex <==
% \section{Proposed Fault Detection and Mitigation Framework}

% In approximate computing for DNNs, ensuring reliability while maintaining energy efficiency is paramount. Our proposed framework enhances the MENDNet architecture \cite{kundu2024mendnet} by integrating a statistical approach for fault detection and mitigation, tailored explicitly for DNNs operating on approximate hardware. This framework is designed to operate within the constraints of energy-limited environments, where storing complete parameter sets for comparison is infeasible.

% \begin{algorithm}[!t]\small
% \caption{Proposed framework for Approximate DNNs}
% \footnotesize
% \label{alg:proposed_framework}
% \DontPrintSemicolon
% \SetKwInOut{Input}{Inputs}\SetKwInOut{Output}{Outputs}
% \Input{%
% \textit{Multi-exit approximate neural network:} $F$\;
% \textit{Confidence threshold:} $\gamma$\;
% \textit{Negative energy threshold:} $\tau$\;
% \textit{Golden model distribution parameters:} $\{\mu_l, \sigma_l\}$\;
% \textit{Input:} $x$\;
% \textit{Significance level:} $\alpha$\;
% }
% \Output{\textit{Output prediction label, Fault detection boolean}}
% \BlankLine
% $\textit{list} \leftarrow \emptyset$ \tcp{Store predictions}
% $\textit{lowest\unc\_label} \leftarrow -1$\;
% $\textit{min\unc} \leftarrow \infty$\;
% \For{$i = 1$ \KwTo $N$}{ \tcp{N is the number of exits}
% \If{$-\text{Eng}(F_i(x)) < \textit{min\unc}$}{
% $\textit{min\unc} \leftarrow -\text{Eng}(F_i(x))$\;
% $\textit{lowest\unc\_label} \leftarrow \argmax(F_i(x))$\;
% }
% \uIf{$\max(F_i(x)) > \gamma$ \textbf{and} $-\text{Eng}(F_i(x)) < \tau$}{
% \Return{$\argmax(F_i(x))$, False}\;
% }
% \uElseIf{$-\text{Eng}(F_i(x)) < \tau$}{
% $\textit{list}.\text{Add}(\argmax(F_i(x)))$\;
% }
% \Else{
% $W_i \leftarrow \text{weights of first layer}$\;
% $p\value \leftarrow \text{AndersonDarlingKSamp}(W_i, \{\mu_i, \sigma_i\})$\;
% \If{$p\value < \alpha$}{
% \For{$w \in W_i$}{
% \If{$|w - \mu_i| > 3\sigma_i$}{
% $w \leftarrow 0$\;
% }
% }
% }
% \If{$\textit{list}.\text{IsEmpty}()$ \textbf{or} $i \leq 2$}{
% \textbf{continue}\;
% }
% \Else{
% \Return{$\textit{list}.\text{Pop}()$, False}\;
% }
% }
% \If{$i = N$}{
% \uIf{$\textit{list}.\text{IsEmpty}()$}{
% \Return{$\textit{lowest\unc\_label}$, True}\;
% }
% \Else{
% \Return{$\textit{list}.\text{Pop}()$, False}\;
% }
% }
% }
% \end{algorithm}

% \subsection{Fault Detection Mechanism}
% Our framework leverages MENDNet's multi-exit architecture, which is built on top of  Shallow-deep Network (SDN) \cite{kaya2019shallow}, and energy-based uncertainty quantification as the primary fault detection mechanism. The energy-based uncertainty quantification measures the network's predictions' uncertainty by calculating the output distribution's energy. A higher energy indicates a more uncertain prediction, while a lower energy suggests a more confident prediction. Our framework leverages MENDNet's multi-exit architecture and energy-based uncertainty quantification as the primary fault detection mechanism. We introduce an uncertainty threshold $\tau$ that is used to detect potential faults. When the uncertainty (i.e., negative energy) at all exits exceeds this threshold, it indicates a significant error in the network, potentially originating from the first layer and propagating through subsequent layers. The uncertainty threshold is determined by analyzing the energy distribution of the network's outputs under normal operating conditions and selecting a value encompassing most of the distribution while excluding outliers. This threshold is then adjusted for the specific approximate computing environment based on the expected level of variability introduced by the approximation techniques employed.

% \subsection{Statistical Fault Verification}
% Upon detecting a potential fault using MENDNet's approach, our framework employs the Anderson-Darling k-sample test to verify the fault's presence. This non-parametric test compares the distribution of the first layer's weights against a pre-established approximate model distribution, which serves as our "golden model." The golden model represents the expected weight distribution of a fault-free approximate network.
% Formally, let $W = \{w_1, \ldots, w_n\}$ be the current weights of the first layer, and $G = \{g_1, \ldots, g_m\}$ be the golden model weights. The Anderson-Darling test statistic is computed as:
% \begin{equation}
% AD = -n - \frac{1}{n}\sum_{i=1}^n (2i-1)[\ln F_G(W_{(i)}) + \ln(1-F_G(W_{(n+1-i)}))]
% \end{equation}
% where $F_G$ is the empirical distribution function of $G$, and $W_{(i)}$ are the ordered statistics of $W$. A p-value is then calculated from this test statistic to determine if the current weight distribution significantly differs from the golden model, indicating a fault.
% The golden model is obtained by training the network on the target dataset using the chosen approximate computing techniques and collecting the weight distributions of the fault-free network. Multiple golden models are generated using different random seeds to account for the inherent variability in approximate computing environments, and the average weight distribution is used as the final golden model. Algorithm \ref{alg:proposed_framework} presents the pseudocode for our proposed fault detection and mitigation framework. The framework takes as input a multi-exit approximate neural network $F$, confidence threshold $\gamma$, negative energy threshold $\tau$, golden model distribution parameters $\{\mu_l, \sigma_l\}$, input $x$, and significance level $\alpha$. The output is the prediction label and a boolean indicating whether a fault was detected.
% \subsection{Fault Mitigation Strategy}
% When a fault is confirmed (i.e., p-value $<$ significance level), our framework employs a targeted mitigation strategy. We replace parameter values that deviate more than three standard deviations from the mean of the golden model distribution with zeros. This threshold was chosen based on empirical observations of the typical weight distributions in the studied networks, striking a balance between fault mitigation and preserving the network's learned representations. While this approach effectively mitigates the impact of faults, it may introduce sparsity in the network, potentially affecting its performance. The fault detection and mitigation process is performed in real-time as the network processes inputs. By leveraging the multi-exit architecture and energy-based uncertainty quantification, our framework can quickly identify potential faults and trigger the statistical verification and mitigation steps without significantly impacting the overall inference time. This real-time operation is crucial for deploying approximate DNNs in energy-constrained environments, where rapid fault detection and mitigation are essential for maintaining the network's reliability and performance.

% % \subsection{Evaluation Methodology}
% % We evaluate our framework across a spectrum of approximate multipliers from Evoapproxlib, ranging from the most accurate (but least energy-efficient) to the least accurate (but most energy-efficient). The multipliers used include \texttt{mul8s\_1KV6}, \texttt{mul8s\_1KV8}, \texttt{mul8s\_1KV9}, \texttt{mul8s\_1KVP}, \texttt{mul8s\_1L2J}, \texttt{mul8s\_1L2H}, \texttt{mul8s\_1L2N}, and \texttt{mul8s\_1L12}.

% % We conduct experiments on three datasets: MNIST, Fashion MNIST, and CIFAR-10, using various network architectures including VGG, WideResNet, and MobileNet. Faults are introduced at rates of 10\%, 30\%, and 50\% by replacing original parameter values in the first layer with noise sampled from a uniform distribution U(-2, 2). Our experimental setup utilizes the AdaPT framework (built on Evoapproxlib for PyTorch), Python 3.12, PyTorch 2.1, and CUDA 11.8, running on an NVIDIA RTX 2080 Ti GPU and an Intel Core i9 CPU. \textcolor{red}{The choice of approximate multipliers was based on their popularity in the approximate computing literature and their diverse energy-accuracy trade-offs. However, the proposed framework is not limited to these specific multipliers and can be easily extended to other approximate computing techniques.}

% % Unlike previous approaches that prioritize either energy efficiency or accuracy, our framework evaluates performance across the entire spectrum of approximate multipliers. This comprehensive evaluation allows for a nuanced understanding of the trade-offs between accuracy and energy efficiency in fault-tolerant approximate computing.
% % By applying our fault detection and mitigation strategy to networks using various approximate multipliers, we can assess how different levels of hardware approximation impact the framework's effectiveness.

% % \subsection{Results Overview}
% % Our experiments demonstrate that while the MENDNet approach is effective for accurate DNNs, it falls short in approximate computing environments. By integrating our statistical approach, we achieve up to a 20\% improvement in accuracy across various approximation levels and fault conditions. The exact improvements vary depending on the level of approximation and the specific network architecture, with the highest gains observed for the most energy-efficient multipliers (e.g., \texttt{mul8s\_1L12}) and the more complex network architectures (e.g., WideResNet). On average, our framework achieves a 12\% improvement in accuracy across all experimental settings, while maintaining the energy efficiency benefits of approximate computing.

% % This significant accuracy improvement, achieved without compromising the energy efficiency benefits of approximate computing, highlights the necessity and effectiveness of our tailored fault mitigation strategy for approximate DNNs.


% \section{Proposed Fault Detection and Mitigation Framework}

% The increasing adoption of approximate computing in AI accelerators necessitates robust fault detection and mitigation strategies that can operate within stringent energy constraints. Building upon the MENDNet architecture \cite{kundu2024mendnet}, we propose a novel framework that integrates statistical approaches to enhance fault tolerance in AxDNNs. Our method addresses the unique challenges posed by hardware approximation, where traditional fault detection techniques often fail to distinguish between intentional approximations and harmful faults.

% \subsection{Framework Overview}

% Our framework leverages a multi-exit neural network architecture, inspired by the Shallow-deep Network (SDN) concept \cite{kaya2019shallow}. It employs a two-stage fault detection mechanism: energy-based uncertainty quantification, as introduced in \cite{kundu2024mendnet}, and our novel statistical verification process. This approach allows for dynamic fault detection and mitigation at various depths of the network, adapting to both the input complexity and the current state of the approximate hardware.
% We utilize the energy score as a computationally efficient metric for uncertainty quantification, following the method proposed in \cite{kundu2024mendnet}. For a given input $x$ and network $f$, the energy score $E$ is defined as:

% \begin{equation}
% E(x; f) = -T \cdot \log \sum_{i=1}^{K} e^{f_i(x)/T}
% \end{equation}

% where $K$ is the number of classes, $f_i(x)$ is the logit score for the $i$-th class, and $T$ is the temperature parameter (set to 1 in our experiments). We introduce an adaptive uncertainty threshold $\tau$ that accounts for the varying levels of approximation across different network layers.

% When the uncertainty at any exit exceeds the threshold $\tau$, it triggers our novel statistical fault verification process. We employ the Anderson-Darling k-sample test to compare the distribution of the current layer's weights against a pre-established golden model distribution. This golden model, representing the expected weight distribution of a fault-free approximate network, is generated through multiple training instances of the network using different random seeds, accounting for the inherent variability in approximate computing environments.

% \subsection{Fault Mitigation}

% Upon detecting a fault (i.e., p-value $< \alpha$, where $\alpha$ is the significance level), our framework employs a targeted mitigation strategy. For the affected layer, we replace parameter values that deviate more than three standard deviations from the mean of the golden model distribution with zeros. This threshold strikes a balance between fault mitigation and preserving the network's learned representations, based on empirical observations of typical weight distributions in AxDNNs.

% Algorithm \ref{alg:proposed_framework} presents the pseudocode for our proposed fault detection and mitigation framework. The algorithm iteratively evaluates each network exit, leveraging both the confidence threshold $\gamma$ and the negative energy threshold $\tau$ to decide on early exits or further analysis. The confidence threshold $\gamma$ determines the minimum acceptable probability for a prediction to be considered reliable, while the negative energy threshold $\tau$ helps identify inputs with high uncertainty, signaling potential faults. The significance level $\alpha$ guides the statistical test for fault detection, ensuring that only statistically significant deviations trigger mitigation. This real-time operation is crucial for deploying AxDNNs in energy-constrained environments, where rapid fault detection and mitigation are essential for maintaining network reliability and performance.


% \begin{algorithm}[!t]\small
% \caption{Fault Detection and Mitigation Framework for AxDNNs}
% \label{alg:proposed_framework}
% \DontPrintSemicolon
% \SetKwInOut{Input}{Inputs}\SetKwInOut{Output}{Outputs}
% \Input{%
% \textit{Multi-exit approximate neural network:} $F$\;
% \textit{Confidence threshold:} $\gamma$\;
% \textit{Negative energy threshold:} $\tau$\;
% \textit{Golden model distribution parameters:} $\{\mu_l, \sigma_l\}_{l=1}^L$\;
% \textit{Input:} $x$\;
% \textit{Significance level:} $\alpha$\;
% }
% \Output{\textit{Output prediction label, Fault detection boolean}}
% \BlankLine
% $\textit{list} \leftarrow \emptyset$ \tcp{Store predictions}
% $\textit{lowest\_unc\_label} \leftarrow -1$\;
% $\textit{min\_unc} \leftarrow \infty$\;
% $\textit{fault\_detected} \leftarrow \text{False}$\;
% \For{$i = 1$ \KwTo $N$}{ \tcp{N is the number of exits}
%     \If{$-\text{Eng}(F_i(x)) < \textit{min\_unc}$}{
%         $\textit{min\_unc} \leftarrow -\text{Eng}(F_i(x))$\;
%         $\textit{lowest\_unc\_label} \leftarrow \argmax(F_i(x))$\;
%     }
%     \uIf{$\max(F_i(x)) > \gamma$ \textbf{and} $-\text{Eng}(F_i(x)) < \tau$}{
%         \Return{$\argmax(F_i(x))$, $\textit{fault\_detected}$}\;
%     }
%     \uElseIf{$-\text{Eng}(F_i(x)) < \tau$}{
%         $\textit{list}.\text{Add}(\argmax(F_i(x)))$\;
%     }
%     \Else{
%         \For{$l = 1$ \KwTo $L_i$}{ \tcp{$L_i$ is the number of layers up to exit $i$}
%             $W_l \leftarrow \text{weights of layer } l$\;
%             $p\text{-value} \leftarrow \text{AndersonDarlingKSamp}(W_l, \{\mu_l, \sigma_l\})$\;
%             \If{$p\text{-value} < \alpha$}{
%                 $\textit{fault\_detected} \leftarrow \text{True}$\;
%                 \For{$w \in W_l$}{
%                     \If{$|w - \mu_l| > 3\sigma_l$}{
%                         $w \leftarrow 0$\;
%                     }
%                 }
%                 $F \leftarrow \text{UpdateLayer}(F, l, W_l)$\;
%             }
%         }
%         \If{$\textit{list}.\text{IsEmpty}()$ \textbf{or} $i \leq 2$}{
%             \textbf{continue}\;
%         }
%         \Else{
%             \Return{$\textit{list}.\text{Pop}()$, $\textit{fault\_detected}$}\;
%         }
%     }
% }
% \If{$\textit{list}.\text{IsEmpty}()$}{
%     \Return{$\textit{lowest\_unc\_label}$, $\textit{fault\_detected}$}\;
% }
% \Else{
%     \Return{$\textit{list}.\text{Pop}()$, $\textit{fault\_detected}$}\;
% }
% \end{algorithm}


% % We evaluated our framework across a spectrum of approximate multipliers from Evoapproxlib, ranging from the most accurate (but least energy-efficient) to the least accurate (but most energy-efficient). Experiments on MNIST, Fashion MNIST, and CIFAR-10 datasets, using various network architectures (VGG, WideResNet, and MobileNet), demonstrate that our approach achieves up to a 20\% improvement in accuracy across various approximation levels and fault conditions, compared to the baseline MENDNet. This significant accuracy improvement, achieved without compromising the energy efficiency benefits of approximate computing, highlights the effectiveness of our tailored fault mitigation strategy for AxDNNs.

% \section{Proposed Fault Detection and Mitigation Framework}

% The increasing adoption of approximate computing in AI accelerators necessitates robust fault detection and mitigation strategies that can operate within stringent energy constraints. Building upon the MENDNet architecture \cite{kundu2024mendnet}, we propose a novel framework that integrates statistical approaches to enhance fault tolerance in AxDNNs. Our method addresses the unique challenges posed by hardware approximation, where traditional fault detection techniques often fail to distinguish between intentional approximations and harmful faults.

% \subsection{Framework Overview}

% Our framework leverages a multi-exit neural network architecture, inspired by the Shallow-deep Network (SDN) concept \cite{kaya2019shallow}. It employs a two-stage fault detection mechanism: energy-based uncertainty quantification, as introduced in \cite{kundu2024mendnet}, and our novel statistical verification process. This approach allows for dynamic fault detection and mitigation at various depths of the network, adapting to both the input complexity and the current state of the approximate hardware.


% \begin{figure}[!t]
% 	\centering
% 	\vspace{-0.01in}
%         \includegraphics[width=1\linewidth]{Figs/method_aps.pdf}
% 	%\vspace{-0.16in}
% 	\caption{Proposed Framework APS for AxDNN hardware fault detection and mitigation}
% 	\label{fig:method_xai}
% 	\vspace{-0.2in}
% \end{figure}

% We utilize the energy score as a computationally efficient metric for uncertainty quantification, following the method proposed in \cite{kundu2024mendnet}. For a given input $x$ and network $f$, the energy score $E$ is defined as:

% \begin{equation}
% E(x; f) = -T \cdot \log \sum_{i=1}^{K} e^{f_i(x)/T}
% \end{equation}

% where $K$ is the number of classes, $f_i(x)$ is the logit score for the $i$-th class, and $T$ is the temperature parameter (set to 1 in our experiments). We introduce an adaptive uncertainty threshold $\tau$ that accounts for the varying levels of approximation across different network layers.

% When the uncertainty at any exit exceeds the threshold $\tau$, it triggers our novel statistical fault verification process. We employ the Anderson-Darling k-sample test to compare the distribution of the current layer's weights against a pre-established golden model distribution. This golden model, representing the expected weight distribution of a fault-free approximate network, is generated through multiple training instances of the network using different random seeds, accounting for the inherent variability in approximate computing environments.


% \begin{algorithm}[!t]\small
% \caption{Fault Detection and Mitigation Framework for AxDNNs}
% \label{alg:proposed_framework}
% \DontPrintSemicolon
% \SetKwInOut{Input}{Inputs}\SetKwInOut{Output}{Outputs}
% \Input{%
% \textit{Multi-exit approximate neural network:} $F$\;
% \textit{Confidence threshold:} $\gamma$\;
% \textit{Negative energy threshold:} $\tau$\;
% \textit{Golden model distribution parameters:} $\{\mu_l, \sigma_l\}_{l=1}^L$\;
% \textit{Input:} $x$\;
% \textit{Significance level:} $\alpha$\;
% }
% \Output{\textit{Output prediction label, Fault detection boolean}}
% \BlankLine
% $\textit{list} \leftarrow \emptyset$ \tcp{Store predictions}
% $\textit{lowest\_unc\_label} \leftarrow -1$\;
% $\textit{min\_unc} \leftarrow \infty$\;
% $\textit{fault\_detected} \leftarrow \text{False}$\;
% \For{$i = 1$ \KwTo $N$}{ \tcp{N is the number of exits}
%     \If{$-\text{Eng}(F_i(x)) < \textit{min\_unc}$}{
%         $\textit{min\_unc} \leftarrow -\text{Eng}(F_i(x))$\;
%         $\textit{lowest\_unc\_label} \leftarrow \argmax(F_i(x))$\;
%     }
%     \uIf{$\max(F_i(x)) > \gamma$ \textbf{and} $-\text{Eng}(F_i(x)) < \tau$}{
%         \Return{$\argmax(F_i(x))$, $\textit{fault\_detected}$}\;
%     }
%     \uElseIf{$-\text{Eng}(F_i(x)) < \tau$}{
%         $\textit{list}.\text{Add}(\argmax(F_i(x)))$\;
%     }
%     \Else{
%         \For{$l = 1$ \KwTo $L_i$}{ \tcp{$L_i$ is the number of layers up to exit $i$}
%             $W_l \leftarrow \text{weights of layer } l$\;
%             $p\text{-value} \leftarrow \text{AndersonDarlingKSamp}(W_l, \{\mu_l, \sigma_l\})$\;
%             \If{$p\text{-value} < \alpha$}{
%                 $\textit{fault\_detected} \leftarrow \text{True}$\;
%                 \For{$w \in W_l$}{
%                     \If{$|w - \mu_l| > 3\sigma_l$}{
%                         $w \leftarrow 0$\;
%                     }
%                 }
%                 $F \leftarrow \text{UpdateLayer}(F, l, W_l)$\;
%             }
%         }
%         \If{$\textit{list}.\text{IsEmpty}()$ \textbf{or} $i \leq 2$}{
%             \textbf{continue}\;
%         }
%         \Else{
%             \Return{$\textit{list}.\text{Pop}()$, $\textit{fault\_detected}$}\;
%         }
%     }
% }
% \If{$\textit{list}.\text{IsEmpty}()$}{
%     \Return{$\textit{lowest\_unc\_label}$, $\textit{fault\_detected}$}\;
% }
% \Else{
%     \Return{$\textit{list}.\text{Pop}()$, $\textit{fault\_detected}$}\;
% }
% \end{algorithm}


% \subsection{Fault Mitigation and Algorithm}

% Upon detecting a fault (i.e., p-value $< \alpha$, where $\alpha$ is the significance level), our framework employs a targeted mitigation strategy. For the affected layer, we replace parameter values that deviate more than three standard deviations from the mean of the golden model distribution with zeros. This threshold strikes a balance between fault mitigation and preserving the network's learned representations, based on empirical observations of typical weight distributions in AxDNNs.

% Algorithm \ref{alg:proposed_framework} presents the pseudocode for our proposed fault detection and mitigation framework. The algorithm processes each input through multiple exits of the network, performing both confidence and uncertainty checks at each stage. Here's a detailed explanation of its operation:

% 1. Initialization: The algorithm initializes variables to track the lowest uncertainty prediction and store valid predictions (lines 1-4).

% 2. Exit Loop: For each exit, the algorithm:
%    a. Updates the lowest uncertainty prediction if necessary (lines 6-9).
%    b. Checks if the current exit meets both confidence and uncertainty criteria. If so, it returns the prediction immediately (lines 10-11).
%    c. If only the uncertainty criterion is met, it stores the prediction for potential later use (lines 12-13).
%    d. If high uncertainty is detected, it triggers a detailed fault check across all layers up to the current exit (lines 15-27).

% 3. Fault Detection and Mitigation: When a potential fault is detected, the algorithm:
%    a. Performs the Anderson-Darling test on each layer's weights (lines 17-18).
%    b. If a fault is confirmed, it sets the fault detection flag and mitigates the fault by zeroing out significantly deviant weights (lines 19-25).
%    c. Updates the network with the corrected weights (line 26).

% 4. Exit Strategy: After checking all exits, the algorithm returns either:
%    a. The prediction with the lowest uncertainty if no valid predictions were stored (lines 33-34).
%    b. The last stored valid prediction otherwise (lines 35-36).

% This algorithm allows for dynamic adaptation to both input complexity and potential faults, ensuring robust performance across various scenarios in approximate computing environments.

% Our framework operates in real-time as the network processes inputs, leveraging the multi-exit architecture for quick fault identification and mitigation. This real-time operation is crucial for deploying AxDNNs in energy-constrained environments, where rapid fault detection and mitigation are essential for maintaining network reliability and performance.



% \subsection{Adaptive Mitigation Strategy}
% Upon detecting a fault, APS employs an adaptive mitigation strategy that considers both the layer importance and the deviation severity. For a weight $w$ in layer $l$, if $|w - \mu_l| > T_l$, we apply:

% \begin{equation}
%     w_{corrected} = \begin{cases}
%         \mu_l & \text{if } \alpha_l > \theta_{high}\\
%         0 & \text{if } \alpha_l \leq \theta_{low}\\
%         w_{nearest} & \text{otherwise}
%     \end{cases}
% \end{equation}

% where $\theta_{high}$ and $\theta_{low}$ are importance thresholds, and $w_{nearest}$ represents the nearest valid weight value based on the layer's statistical distribution.

% \subsection{Implementation Considerations and Theoretical Analysis}
% The APS framework is designed for efficient implementation with minimal overhead. Signature storage requires only $O(L)$ space, where $L$ is the number of layers. The detection and mitigation mechanisms operate in-place, avoiding additional memory requirements during inference. Furthermore, our approach is compatible with existing approximate computing architectures, requiring no modifications to the underlying hardware.
% % \subsection{Theoretical Analysis}
% The effectiveness of APS can be analyzed through the lens of statistical error bounds. Given a fault rate $p$ and layer importance $\alpha_l$, the probability of missed detection $P_{md}$ is bounded by:

% \begin{equation}
%     P_{md} \leq \exp(-\alpha_l^2/2p)
% \end{equation}

% This bound ensures that critical layers maintain higher detection accuracy while allowing more flexibility in less crucial layers, aligning with the approximate computing paradigm.


% % \subsubsection{Model Assumptions and Scope}
% We make the following practical assumptions:
% \begin{itemize}
%     \item Faults are persistent throughout inference
%     \item Control logic remains reliable
%     \item Fault locations are unknown during runtime
%     \item Fault rates remain consistent within operational periods
% \end{itemize}

% This model specifically targets approximate multiplier arrays in neural network accelerators, where energy efficiency is achieved through intentional approximation \cite{approx_accelerators}. While our approach primarily addresses permanent faults, the detection mechanism can potentially extend to transient faults, though this remains outside our current scope.

% The fault model described above provides a realistic foundation for evaluating our proposed APS framework, particularly in the context of approximate computing where traditional fault models may be overly conservative \cite{fault_models_review}.



% \section{Proposed Framework: Adaptive Pattern Signatures (APS)}

% \subsection{Framework Overview}
% Building upon the challenges identified in our motivational study, we propose Adaptive Pattern Signatures (APS), a framework designed specifically for fault detection and mitigation in approximate neural networks. As illustrated in Fig.~\ref{fig:method_xai}, APS employs a multi-exit architecture that enables dynamic fault detection and mitigation at various network depths.

% The framework operates through three key mechanisms:
% \begin{enumerate}
%     \item Statistical signature generation for baseline behavior characterization
%     \item Layer-importance aware detection for efficient fault identification
%     \item Adaptive mitigation strategies for minimal performance impact
% \end{enumerate}

% This design addresses the unique challenges of distinguishing between intentional approximations and harmful faults while maintaining the energy efficiency benefits of approximate computing.

% \subsection{Core Components}
% \subsubsection{Statistical Signature Generation}
% For each layer $l$ in the network, APS generates a comprehensive statistical signature $S_l$:

% \begin{equation}
%     S_l = \{\mu_l, \sigma_l, Q_l, \rho_l\}
% \end{equation}

% where:
% \begin{itemize}
%     \item $\mu_l$, $\sigma_l$: Mean and standard deviation of layer weights
%     \item $Q_l$: Quartile distribution metrics
%     \item $\rho_l$: Layer-specific sparsity patterns
% \end{itemize}

% These signatures serve as reference points for fault detection while introducing minimal storage overhead. The signature generation process occurs during pre-deployment, utilizing multiple training instances to capture the inherent variability in approximate computing environments.

% \subsubsection{Layer-Importance Aware Detection}
% The framework employs a layer-specific importance factor $\alpha_l$:

% \begin{equation}
%     \alpha_l = \beta_p \cdot \gamma_s
% \end{equation}

% where $\beta_p$ represents positional importance (decreasing from input to output layers) and $\gamma_s$ captures structural importance based on layer type and connectivity. This leads to dynamic detection thresholds:

% \begin{equation}
%     T_l = (3 + \alpha_l)\sigma_l
% \end{equation}

% For uncertainty quantification, we utilize an energy-based metric $E$:

% \begin{equation}
% E(x; f) = -T \cdot \log \sum_{i=1}^{K} e^{f_i(x)/T}
% \end{equation}

% where $K$ represents output classes and $T$ is the temperature parameter.

% \subsubsection{Adaptive Mitigation Strategy}
% Upon detecting a fault, APS employs a context-aware mitigation approach:

% \begin{equation}
%     w_{corrected} = \begin{cases}
%         \mu_l & \text{if } \alpha_l > \theta_{high}\\
%         0 & \text{if } \alpha_l \leq \theta_{low}\\
%         w_{nearest} & \text{otherwise}
%     \end{cases}
% \end{equation}

% where $\theta_{high}$ and $\theta_{low}$ are importance thresholds, and $w_{nearest}$ represents the nearest valid weight value based on the layer's statistical distribution.

% \subsection{Algorithm Implementation}
% Algorithm \ref{alg:proposed_framework} details the implementation of APS, which consists of three main phases:

% 1. Initialization Phase:
%    - Initialize prediction storage and uncertainty tracking
%    - Set up fault detection flags

% 2. Detection Phase:
%    - Process each network exit
%    - Perform confidence and uncertainty checks
%    - Trigger detailed fault analysis when necessary

% 3. Mitigation Phase:
%    - Apply statistical tests for fault confirmation
%    - Execute targeted weight corrections
%    - Update network parameters

% The algorithm maintains constant-time complexity for detection and linear space complexity for signature storage, making it suitable for real-time applications.

% \subsection{Theoretical Analysis}
% The effectiveness of APS can be analyzed through statistical error bounds. Given fault rate $p$ and layer importance $\alpha_l$, the probability of missed detection $P_{md}$ is bounded by:

% \begin{equation}
%     P_{md} \leq \exp(-\alpha_l^2/2p)
% \end{equation}

% This bound ensures:
% \begin{itemize}
%     \item Higher detection accuracy in critical layers
%     \item Flexible tolerance in less crucial layers
%     \item Balanced trade-off between accuracy and efficiency
% \end{itemize}

% The space complexity for signature storage is $O(L)$, where $L$ is the number of layers, while detection and mitigation operate in-place with $O(1)$ additional memory requirements during inference.

% \subsection{Fault Model and Assumptions}
% Our framework addresses permanent stuck-at faults (SA0 and SA1) in approximate multipliers, with fault rate $p$ defined as:

% \begin{equation}
%     p = \frac{N_{faulty}}{N_{total}} \times 100\%
% \end{equation}

% Key assumptions include:
% \begin{itemize}
%     \item Faults persist throughout inference
%     \item Control logic remains reliable
%     \item Fault locations are unknown during runtime
%     \item Fault rates remain consistent within operational periods
% \end{itemize}

% The spatial distribution of faults follows a random pattern within each layer, with impact severity modeled as:

% \begin{equation}
%     I_{severity} = f(l_{pos}, b_{pos}, p)
% \end{equation}

% where $l_{pos}$ is layer position, $b_{pos}$ is bit position, and $p$ is fault rate.


% \begin{table}[t] 
% \centering
% \caption{Average Time (ms) for vanilla AxDNN, MENDNet, and APS using different approximate multipliers for each dataset} 
% \begin{tabular}{|c|c|c|c|c|}
% \hline Dataset & Approximate Multiplier & AxDNN (ms) & MENDNet (ms) & APS (ms) \\ \hline 
% MNIST & mul8s\_1KVP & 168.41 & 135.44 & 130.00 \\ 
% MNIST & mul8s\_1L2J & 172.98 & 140.86 & 135.00 \\ 
% MNIST & mul8s\_1L2H & 191.95 & 150.42 & 145.00 \\ \hline 
% Fashion MNIST & mul8s\_1KVP & 192.16 & 99.87 & 95.00 \\ 
% Fashion MNIST & mul8s\_1L2J & 206.90 & 143.45 & 137.00 \\ 
% Fashion MNIST & mul8s\_1L2H & 212.57 & 143.71 & 138.00 \\ \hline 
% CIFAR10 & mul8s\_1KVP & 205.40 & 187.21 & 180.00 \\ 
% CIFAR10 & mul8s\_1L2J & 210.41 & 196.33 & 190.00 \\ 
% CIFAR10 & mul8s\_1L2H & 224.88 & 209.48 & 200.00 \\ \hline 
% \end{tabular} 
% \label{table:average_time_approx_multipliers_all_models} 
% \end{table}


\section{Proposed EPSILON Framework for AxDNN Fault Detection \& Mitigation}
%This section introduces EPSILON, an efficient framework designed for fault detection and mitigation in AxDNNs, emphasizing its adaptability to approximate computing scenarios. EPSILON leverages multi-exit neural networks inspired by the Shallow-Deep Network (SDN) \cite{kaya2019shallow}, embedding multiple classification exits throughout the network. These exits enable early termination of computation when high-confidence predictions are achieved, reducing latency and energy consumption. Furthermore, this design inherently provides fault tolerance by offering redundant prediction paths across the network. The framework is divided into three main phases: (1) AxDNN configuration, (2) pre-deployment, and (3) runtime inference. Each phase is tailored to ensure a balance between computational efficiency and fault tolerance. The AxDNN configuration phase is user-dependent, allowing the selection of the desired network architecture and approximate hardware tailored to application-specific requirements, while the subsequent phases are where EPSILON’s core mechanisms operate to ensure robust fault detection and mitigation.

% For a multi-exit network \( F \) with \( N \) exits, each exit \( i \) produces a prediction \( F_i(x) \) for an input \( x \). Computation halts early when the confidence score surpasses a predefined threshold \( \gamma \), i.e., \( \max(F_i(x)) > \gamma \). This capability not only enhances efficiency by leveraging early exits but also ensures resilience by utilizing alternative exits in the presence of faults. The framework systematically integrates these features to optimize both runtime performance and fault mitigation.


% \section{EPSILON Framework for AxDNN Fault Detection \& Mitigation}
% This section presents EPSILON, our proposed framework for efficient fault detection and mitigation in AxDNNs. Fig \ref{fig:method_aps} illustrates the framework's architecture comprising three main phases: AxDNN configuration, pre-deployment, and runtime inference that involves fault detection and mitigation. Our framework leverages multi-exit neural networks inspired by the Shallow-deep Network (SDN) \cite{kaya2019shallow}, which incorporate multiple classification exits throughout the network architecture. For a multi-exit network $F$ with $N$ exits, each exit $i$ can provide a prediction for input $x$, terminating computation early if its confidence score exceeds a predetermined threshold $\gamma$ (i.e., $\max(F_i(x)) > \gamma$).
% This architecture enables efficient processing by allowing early termination when sufficient prediction confidence ($\max(F_i(x)) > \gamma$) is achieved at any exit $i$, while simultaneously providing inherent fault tolerance through redundant prediction paths. This architecture provides inherent fault tolerance through redundant prediction paths. 

%This section introduces EPSILON, an efficient framework for fault detection and mitigation in AxDNNs, emphasizing its adaptability to approximate computing scenarios. EPSILON leverages multi-exit neural networks inspired by the Shallow-Deep Network (SDN) \cite{kaya2019shallow}, embedding multiple classification exits throughout the network. These exits enable early termination of computation when high-confidence predictions are achieved, reducing latency and energy consumption. Furthermore, this design inherently provides fault tolerance by offering redundant prediction paths across the network. \textcolor{red}{The framework is divided into three main phases: (1) AxDNN configuration, (2) pre-deployment, and (3) runtime inference. Each phase is tailored to balance computational efficiency and fault tolerance. The AxDNN configuration phase is user-specific, allowing the selection of the desired network architecture and approximate hardware tailored to application-specific requirements. In contrast, the subsequent phases are  EPSILON’s core mechanisms to ensure robust fault detection and mitigation.}

This section introduces EPSILON, an efficient framework for fault detection and mitigation in AxDNNs, emphasizing its adaptability to approximate computing scenarios. 
% EPSILON leverages multi-exit neural networks inspired by the Shallow-Deep Network (SDN) \cite{kaya2019shallow}. 
The framework is divided into \emph{pre-deployment} and \emph{inference phase}, described in coming sub sections.  

% \subsection{Problem Formulation}
\subsection{Problem Formulation}
The primary objective of the EPSILON framework is to detect and mitigate faults within AxDNN while ensuring minimal energy consumption and computational overhead. Formally, let \( x \) denote the input data to the AxDNN, and \( F \) represent the approximate multi-exit AxDNN architecture comprising exits \( {F_i} \), where \( i \) spans the total number of exits \( N \). The framework implements a predefined confidence threshold \( \gamma \) to decide if deeper inspection is necessary based on the confidence levels of predictions at each exit. The statistical foundation of the framework is established through layer-specific signatures \( {S_l} \) for layers \( l = 1 \) to \( L \), where each signature \( S_l \) incorporates four fundamental statistical measures: mean \( \mu_l \), standard deviation \( \sigma_l \), quartiles \( Q_l \), and sparsity pattern \( \rho_l \). Layer-specific importance factors \( {\alpha_l} \) describe a set of importance factors for each layer, which influences fault detection thresholds and corrective actions. For the \( i^{th} \) exit, the network generates prediction \( pred_i \) with an associated confidence score \( conf_i \). The framework utilizes candidate valid weight values \( v \) derived from \( Q_l \), while \( W_l \) denotes the weights for layer \( l \). The fault detection threshold \( T_l \) is dynamically computed as a function of \( \sigma_l \) and layer importance factor \( \alpha_l \), incorporating an offset factor \( m \). The fault position (FP) identifies the layer at which faults manifest, enabling precise fault localization and subsequent analysis.
% The problem can be formally defined as follows:
% Given an input \( x \), a multi-exit AxDNN \( F \), and a predefined confidence threshold \( \gamma \), the goal is to determine the presence of faults during the prediction process. Each exit within the network provides a preliminary prediction and corresponding confidence level. If the confidence at any exit exceeds \( \gamma \), the framework assumes no fault and outputs the prediction. Conversely, if all exits report low confidence, further inspection is triggered to analyze layer-wise deviations from expected statistical signatures.

% For fault detection and mitigation, the EPSILON adjusts weights in real time based on pre-computed layer signatures and dynamically calculated importance factors. The process involves:
% \begin{enumerate}
%     \item Assessing each layer's output against its expected behavior using statistical signatures \( \{S_l = (\mu_l, \sigma_l, Q_l, \rho_l)\}_{l=1}^L \).
%     \item Engaging corrective mechanisms if deviations exceed certain thresholds, which are adjusted by importance factors \( \{\alpha_l\}_{l=1}^L \), reflecting the relative significance of each layer within the network.
% \end{enumerate}
% The algorithm must balance between prompt fault detection and the computational demands of real-time analysis, ensuring the framework remains feasible for deployment on resource-limited platforms.
% \textbf{Variable Descriptions in the Framework and Algorithm:}





% The variables in the EPSILON framework and algorithm are defined as follows: \( x \) represents the input data to the AxDNN. \( F \) denotes the multi-exit AxDNN, which consists of exits \( \{F_i\} \) where \( i \) incorporates the range over the number of exits \( N \). The confidence threshold \( \gamma \) is a predefined parameter used to decide if deeper inspection is necessary, based on the confidence levels of predictions at each exit. \( \{S_l\} \) is a set of statistical signatures for layers \( l = 1 \) to \( L \), where each \( S_l \) includes the mean \( \mu_l \), standard deviation \( \sigma_l \), quartiles \( Q_l \), and sparsity pattern \( \rho_l \) of the respective layer. \( \{\alpha_l\} \) describes a set of importance factors for each layer, which influence fault detection thresholds and corrective actions. The prediction at the \( i^{th} \) exit of the network is denoted by \( pred_i \), and \( conf_i \) is the confidence score associated with \( pred_i \). \( v \) is candidate valid weight values from \( Q_l \). \( W_l \) represents the weights for layer \( l \), and \( T_l \) is the dynamically calculated threshold for fault detection at layer \( l \), which depends on the standard deviation \( \sigma_l \) and the assigned layer importance \( \alpha_l \), with the offset factor \( m \). The fault position (FP) denotes the layer's location where faults are introduced.


%The primary objective of the EPSILON framework is to detect and mitigate faults within AxDNN, while ensuring minimal energy consumption and computational overhead. The EPSILON framework encompasses a comprehensive set of variables essential for fault detection in AxDNNs. Formally, let \( x \) denote the input data to the AxDNN, and \( F \) represent the approximate multi-exit AxDNN architecture comprising exits \( {F_i} \), where \( i \) spans the total number of exits \( N \). The framework implements a predefined confidence threshold \( \gamma \) to decide if deeper inspection is necessary based on the confidence levels of predictions at each exit. The statistical foundation of the framework is established through layer-specific signatures \( {S_l} \) for layers \( l = 1 \) to \( L \), where each signature \( S_l \) incorporates four fundamental statistical measures: mean \( \mu_l \), standard deviation \( \sigma_l \), quartiles \( Q_l \), and sparsity pattern \( \rho_l \). Layer-specific importance factors \( {\alpha_l} \) describes a set of importance factors for each layer, which influence fault detection thresholds and corrective actions. For the \( i^{th} \) exit, the network generates prediction \( pred_i \) with an associated confidence score \( conf_i \). The framework utilizes candidate valid weight values \( v \) derived from \( Q_l \), while \( W_l \) denotes the weights for layer \( l \). The fault detection threshold \( T_l \) is dynamically computed as a function of \( \sigma_l \) and \( \alpha_l \), incorporating an offset factor \( m \). The fault position (FP) identifies the layer at which faults manifest, enabling precise fault localization and subsequent analysis.



% These elements within the EPSILON framework collectively address the challenge of maintaining reliable AxDNN performance in approximate computing scenarios, characterized by intrinsic vulnerabilities to hardware-related faults. The algorithm ensures that detection and mitigation processes are efficiently managed, striking an optimal balance between computational load and fault tolerance.

%Each phase is tailored to balance computational efficiency and fault tolerance. The AxDNN configuration phase is user-specific, allowing the selection of the desired network architecture and approximate hardware tailored to application-specific requirements. In contrast, the subsequent phases are  EPSILON’s core mechanisms to ensure robust fault detection and mitigation.

\subsection{Pre-Deployment Phase}
%The pre-deployment phase establishes the foundation for fault detection through its key components. In our framework, fault-free multi-exit AxDNNs act as the golden model. This baseline provides the reference to derive statistical metrics and set confidence thresholds for effective fault detection. By analyzing these fault-free networks, we generate statistical signatures that characterize each layer's normal behavior. These signatures guide our detection mechanisms, ensuring that runtime deviations are accurately identified as anomalies. The confidence threshold $\gamma$ is predetermined as outlined in \cite{kaya2019shallow, kundu2024mendnet}. Next, we describe the signature generation process, followed by our layer-importance aware detection mechanism and the adaptive mitigation strategy. 
The pre-deployment phase establishes the foundation for fault detection through its key components. In our framework, fault-free multi-exit AxDNNs act as the golden model. This baseline provides the reference to derive statistical metrics and set confidence thresholds for effective fault detection. By analyzing these fault-free networks, we generate \emph{statistical signatures} that characterize each layer's normal behavior. These signatures guide our detection mechanisms, ensuring that runtime deviations are accurately identified as anomalies. The confidence threshold $\gamma$ is predetermined as outlined in \cite{kaya2019shallow, kundu2024mendnet}. Next, we describe the \emph{signature generation} process, followed by our \emph{layer-importance-aware detection} mechanism and the \emph{adaptive mitigation} strategy. 

\subsubsection{Statistical Signature Generation}
The statistical signatures in EPSILON are computationally efficient in generating and providing a compact yet comprehensive representation of normal layer behavior in fault-free AxDNNs. For each layer \( l \), a statistical signature \( S_l \) is computed as:
\begin{equation}\label{eqn-sign}
    S_l = \{\mu_l, \sigma_l, Q_l, \rho_l\}
\end{equation}

%In Equation \eqref{eqn-sign}, \( \mu_l \) and \( \sigma_l \) capture the mean and standard deviation of the layer's weights, representing central tendency and variability. Quartile metrics \( Q_l \) enhance robustness by mitigating the influence of outliers, a critical consideration in approximate settings. The sparsity pattern \( \rho_l \), which quantifies the distribution of zero and non-zero weights, is particularly relevant in approximate computing, where weights near zero are frequently quantized to zero. Deviations in \( \rho_l \) serve as sensitive indicators of structural inconsistencies or faults. These metrics collectively form a reliable baseline for detecting runtime deviations. By confining the signature generation to the pre-deployment phase, EPSILON achieves a lightweight design, ensuring the framework is well-suited for resource-constrained edge hardware deployments.
In Equation \eqref{eqn-sign}, \( \mu_l \) and \( \sigma_l \) capture the mean and standard deviation of each layer's weights, representing central tendency and variability. Quartile metrics \( Q_l \) enhance robustness by mitigating the influence of outliers, a critical consideration in approximate settings. The sparsity pattern \( \rho_l \), which quantifies the distribution of zero and non-zero weights, is particularly relevant in approximate computing, where weights near zero are frequently quantized to zero. Deviations in \( \rho_l \) serve as sensitive indicators of structural inconsistencies or faults. These metrics collectively form a baseline for detecting runtime deviations. By confining the signature generation to the pre-deployment phase, EPSILON achieves a lightweight design, ensuring the framework is well-suited for resource-constrained edge hardware deployments.


% \subsubsection{Statistical Signature Generation}
% % At the core of EPSILON's fault detection capability is its use of statistical signatures, derived from pre-trained, fault-free AxDNNs during the pre-deployment phase. 
% The statistical signatures are computationally efficient to generate and serve as a compact representation of normal layer behavior. For each layer \( l \) in the AxDNN, we compute a statistical signature \( S_l \), defined as:

% \begin{equation}
%     S_l = \{\mu_l, \sigma_l, Q_l, \rho_l\}
% \end{equation}

% where \( \mu_l \) and \( \sigma_l \) represent the mean and standard deviation of the layer's weights, capturing central tendency and variability. Quartile metrics \( Q_l \) further enhance robustness against outliers, particularly in approximate settings. The sparsity pattern \( \rho_l \) encodes the structural characteristics of the layer by quantifying the distribution of zero and non-zero weights. This is particularly relevant in approximate computing, where weights close to zero are often quantized to zero, making deviations in \( \rho_l \) a critical indicator of structural inconsistencies or faults.
% Together, these metrics form a baseline against which runtime deviations are measured. EPSILON minimizes overhead by confining the generation of these signatures to the pre-deployment phase. This ensures the detection framework remains lightweight and suitable for edge hardware deployment.


% \subsubsection{Statistical Signature Generation}
% The cornerstone of EPSILON is its ability to capture reliable statistical signatures from pre-trained multi-exit AxDNN. Unlike traditional approaches that rely on computationally expensive runtime checks \cite{reagen2018ares, zhang2018thundervolt}, our method generates comprehensive signatures during the pre-deployment phase. For each layer $l$ in the AxDNN, we compute a set of statistical metrics $S_l$ that characterize its nominal behavior:

% \begin{equation}
%     S_l = \{\mu_l, \sigma_l, Q_l, \rho_l\}
% \end{equation}

% where $\mu_l$ and $\sigma_l$ represent the mean and standard deviation of layer weights for capturing central tendency and spread, $Q_l$ captures the quartile distribution for robust outlier detection, and $\rho_l$ represents the layer's sparsity pattern for structural integrity verification. These signatures serve as reference points for fault detection while introducing minimal storage overhead.


\subsubsection{Layer-Importance Aware Detection}  
EPSILON introduces a layer-importance-aware detection mechanism to account for the varying sensitivities of AxDNN layers to hardware faults. Different layers contribute unequally to the overall network performance, and faults in critical layers can disproportionately degrade model accuracy \cite{reagen2018ares}. Early convolutional layers, which extract foundational features, are often more fault-sensitive than later layers that refine or combine high-level abstractions \cite{9424345}. To capture this variability, we define an importance factor \(\alpha_l\) for each layer \(l\) as:
\begin{equation}\label{eqn-layer-imp}
\alpha_l = \beta_p \cdot \gamma_s \quad \text{where } \beta_p \in [0,1], \gamma_s \in [0,1]
\end{equation}

In Equation \eqref{eqn-layer-imp}, \(\beta_p\) denotes the positional importance of the layer, progressively decreasing from input to output layers. This reflects the observation that faults in earlier layers tend to propagate through the network, amplifying their impact. \(\gamma_s\), on the other hand, captures the structural importance, incorporating attributes such as layer type, connectivity, and sparsity. For example, convolutional layers with high connectivity and feature extraction responsibility are assigned higher structural importance than activation layers or layers with significant sparsity \cite{reagen2018ares}. Using \(\alpha_l\), the fault detection thresholds are dynamically adjusted for each layer $l$ as:
\begin{equation}
T_l = (m + \alpha_l)\sigma_l
\label{eq:equation3}
\end{equation}

The threshold \(T_l\) scales with both the intrinsic variability (standard deviation) of the layer’s weights \(\sigma_l\) and the importance factor \(\alpha_l\) with the offset \(m\). The ranges of \([0,1]\) for \(\beta_p\) and \(\gamma_s\) are normalized to avoid over-weighting any single component and ensure balanced contributions.

% This approach strikes a balance between computational efficiency and robust fault detection. By tailoring detection sensitivity to layer importance, EPSILON prioritizes fault detection in critical layers, ensuring minimal degradation in overall model performance. Future work will investigate the empirical validation of parameter choices and explore whether additional layer-specific characteristics, such as activation distributions or learned feature importance, could further enhance the detection mechanism.


% \subsubsection{Layer-Importance Aware Detection}
% A key innovation in EPSILON is its layer-importance aware detection mechanism. The different layers in DNNs exhibit varying sensitivities to hardware faults \cite{reagen2018ares}. Early convolutional layers, being critical for feature extraction, require stricter fault detection compared to later layers \cite{9424345}. We define the importance factor $\alpha_l$ for layer $l$ as:

% \begin{equation}
%     \alpha_l = \beta_p \cdot \gamma_s \quad \text{where } \beta_p \in [0,1], \gamma_s \in [0,1]
% \end{equation}

% where $\beta_p$ represents the positional importance (decreasing from input to output layers) and $\gamma_s$ captures the structural importance based on layer type and connectivity. This importance-aware approach allows us to dynamically adjust detection thresholds:

% \begin{equation}
%     T_l = (3 + \alpha_l)\sigma_l
% \end{equation}



\SetInd{0.5em}{0.5em}
\setlength{\textfloatsep}{0pt}% Remove \textfloatsep
\SetInd{0.5em}{0.5em} 
% \hspace{5cm}
% \raggedright
\begin{algorithm}[!t]\footnotesize
\caption{Proposed EPSILON Framework}
\label{alg:proposed_framework}
\DontPrintSemicolon
\SetKwInOut{Input}{Inputs}\SetKwInOut{Output}{Outputs}
\Input{%
\textit{Multi-exit AxDNN:} $F$\\
\textit{Confidence threshold:} $\gamma$\\
\textit{Statistical signatures:} $\{S_l = (\mu_l, \sigma_l, Q_l, \rho_l)\}_{l=1}^L$\\
\textit{Layer importance factors:} $\{\alpha_l\}_{l=1}^L$\\
\textit{Input:} $x$\\
}
\Output{\textit{Prediction label, Fault detection boolean}}
\BlankLine
$\textit{list} \leftarrow \emptyset$ \tcp{Store predictions}
$\textit{all\_exits\_low\_confidence} \leftarrow \text{True}$\;

\For{$i = 1$ \KwTo $N$}{ \tcp{N is the number of exits}
    $pred_i \leftarrow F_i(x)$\;
    $conf_i \leftarrow \max(pred_i)$\;
    
    \If{$conf_i > \gamma$}{
        $\textit{all\_exits\_low\_confidence} \leftarrow \text{False}$\;
        \Return{$\argmax(pred_i)$, False}\;
    }
    $\textit{list}.\text{Add}(\argmax(pred_i))$\;
}

\If{$\textit{all\_exits\_low\_confidence}$}{
    \tcp{Activate EPSILON framework}
    $\textit{fault\_detected} \leftarrow \text{False}$\;
    
    \For{$l = 1$ \KwTo $L$}{
        $W_l \leftarrow \text{GetLayerWeights}(F, l)$\\
            $ T_l \leftarrow (m + \alpha_l)\sigma_l$\
        
        \tcp{Pattern analysis}
        $pattern\_score \leftarrow \text{ComputePatternDeviation}(W_l, \rho_l)$\;
        
        \If{$pattern\_score > T_l$}{
            $\textit{fault\_detected} \leftarrow \text{True}$\;
            
            \For{$w \in W_l$}{
                \If{$|w - \mu_l| > T_l$}{
                    $w \leftarrow \text{FindNearestValid}(w, Q_l)$\;
                }
            }
            $F \leftarrow \text{UpdateLayer}(F, l, W_l)$\;
        }
    }
    
    \tcp{Recompute prediction with corrected weights}
    $final\_pred \leftarrow F_N(x)$\
    
    \Return{$\argmax(final\_pred)$, $\textit{fault\_detected}$}\;

% $\textit{list}.\text{Pop}()$
}
% \Return{$\textit{list}.\text{Pop}()$, False}\;
\end{algorithm}


\subsection{Inference Phase}
%The EPSILON framework operates in two distinct stages during runtime to ensure both efficient and accurate fault detection and mitigation. This dual-stage approach leverages multi-exit architectures for early detection and confidence-based mitigation, followed by a more comprehensive statistical analysis when necessary. The following subsections explain these stages in detail, with references to the corresponding lines in Algorithm \ref{alg:proposed_framework}.
The EPSILON framework operates in two distinct stages during inference to ensure efficient and accurate fault detection and mitigation. This dual-stage approach leverages multi-exit architectures for early detection and confidence-based mitigation, followed by a more comprehensive statistical analysis when necessary. The overall approach is presented in Algorithm \ref{alg:proposed_framework}, and the following subsections explain these stages. The algorithm takes as input a multi-exit AxDNN model \(F\), a confidence threshold \(\gamma\), statistical signatures \(\{S_l = (\mu_l, \sigma_l, Q_l, \rho_l)\}_{l=1}^L\), layer importance factors \(\{\alpha_l\}_{l=1}^L\), and a data sample \(x\), and outputs the predicted label along with a fault detection boolean.

\subsubsection{Primary Detection through Exit Confidence}
The first stage of the runtime phase focuses on leveraging the multi-exit architecture for rapid, confidence-based fault detection. For a given input $x$, each exit $i$ computes its prediction $F_i(x)$, and the confidence $conf_i$ is determined (see Algorithm \ref{alg:proposed_framework}, Lines~3--4) as follows:
\begin{equation}
    conf_i = \max(F_i(x)) \quad \text{for exit } i \in \{1, \ldots, N\}.
\end{equation}

Next, the framework checks whether any exit produces a confidence score exceeding the predefined threshold $\gamma$ (Algorithm \ref{alg:proposed_framework}, Line~5):
\begin{equation}
    \exists i : conf_i > \gamma.
\end{equation}

If this condition is met, the network outputs the corresponding prediction along with $False$ fault boolean value and bypasses further analysis (Algorithm \ref{alg:proposed_framework}, Line~6). This early exit mechanism minimizes computational overhead during regular operation, making it effective in scenarios where the predictions remain robust under faults.

\subsubsection{EPSILON Activation and Statistical Analysis}
When none of the exits achieve the required confidence ($conf_i \leq \gamma$ for all $i$), the EPSILON framework activates its fault detection mechanism (Algorithm \ref{alg:proposed_framework}, Line~10). This stage involves evaluating statistical deviations in layer-wise patterns to identify potential faults. Each layer $l$ is associated with a reference statistical signature $\rho_l$, and the current observed signature $\rho_{current}$ is compared using the pattern score (Algorithm \ref{alg:proposed_framework}, Line~14): 
\begin{equation}
    pattern\_score_l = \sum_{i=1}^{L} |\rho_l(i) - \rho_{current}(i)|.
\end{equation}

The framework computes a dynamic threshold $T_l$ for each layer based on its reference standard deviation $\sigma_l$ and a tunable importance factor $\alpha_l$ (see Algorithm \ref{alg:proposed_framework}, Line~14). If $pattern\_score_l > T_l$, the layer is flagged as faulty (Algorithm \ref{alg:proposed_framework}, Line~16). 
% These calculations align with the pattern-deviation checks and dynamic threshold evaluations outlined in Algorithm \ref{alg:proposed_framework}. \textcolor{red}{what do you mean here?}

\subsubsection{Adaptive Mitigation Strategy}
%Once a fault is detected in a layer, EPSILON employs a targeted correction mechanism. Each weight $w$ in the faulty layer is evaluated and corrected if it deviates significantly from its expected range (Lines~17--19). The correction process adjusts weights to the nearest valid value in the set $Q_l$, representing acceptable weight ranges for the layer:
EPSILON employs a targeted correction mechanism once a fault is detected in a layer. Each weight $w$ in the faulty layer is evaluated and corrected if it deviates significantly from its expected range (Lines~17--19 in Algorithm \ref{alg:proposed_framework}). The correction process adjusts weights to the nearest valid value in the set $Q_l$, representing acceptable weight ranges for the layer as:
\begin{equation}
    w_{corrected} = \arg\min_{v \in Q_l} |w - v|.
\end{equation}

where $v$ is candidate valid weight values. This step ensures that the layer's statistical integrity is restored while mitigating the impact of the detected faults. The corrected $w_{corrected}$ are updated to the network (Line~22 in Algorithm \ref{alg:proposed_framework}) and inference is performed with the updated weights (Line~25 in Algorithm \ref{alg:proposed_framework}) and the final prediction is returned along with $True$ fault boolean value (Line~26). The complete dual-stage approach enables an optimal balance between detection accuracy and computational efficiency. 
% \textcolor{red}{The more computationally intensive pattern} analysis is activated only when necessary, resulting in an average-case complexity that remains practical for real-time applications. 
% \textcolor{red}{What is the output/rerun of the Algo? what is the job of lines like 22, 25, return etc? you did not finish describing the process.} 

% \textcolor{red}{\subsection{Fault Model}}
% Hardware faults in approximate computing systems can manifest in various forms. In this work, we focus on permanent stuck-at faults, which are particularly relevant for approximate multipliers in neural network accelerators \cite{9424345}. 
% % Our fault model encompasses the following key aspects:
% % \subsubsection{Fault Characteristics}
% We consider both stuck-at-0 (SA0) and stuck-at-1 (SA1) faults that can occur in the weight storage and computation units of AxDNN accelerators. \textcolor{red}{do you have results for SA0 in the paper?}
% %These faults typically manifest as bit flips in the binary representation of weights, affecting the least significant bits (LSBs) more frequently due to the nature of approximate computing \cite{zhang2020safaults}. 
% The fault rate $p$ (\textcolor{red}{why `p' and why not FR?}) represents the percentage of weights affected in a given layer, where:
% \begin{equation}
%     p = \frac{N_{faulty}}{N_{total}} \times 100\%,
% \end{equation}
% where $N_{faulty}$ is the number of faulty weights and $N_{total}$ is the total number of weights in the layer. The spatial distribution of faults follows a random pattern within each layer, which aligns with real-world observations in approximate hardware \cite{hardware_faults}. This randomness is particularly important as it reflects realistic fault patterns in approximate multipliers and provides worst-case scenarios for robustness analysis.


% \subsection{Runtime Phase}
% The EPSILON framework implements a two-stage fault detection and mitigation strategy, as outlined in Algorithm \ref{alg:proposed_framework}. This approach first leverages the natural fault tolerance of multi-exit architectures before engaging more sophisticated statistical analysis when needed.

% \subsubsection{Primary Detection through Exit Confidence}
% The framework initially operates through confidence monitoring at each network exit:

% \begin{equation}
%     conf_i = \max(F_i(x)) \quad \text{for exit } i \in \{1,...,N\}
% \end{equation}

% where $F_i(x)$ represents the prediction at exit $i$. Normal execution continues if any exit shows sufficient confidence:

% \begin{equation}
%     \exists i : conf_i > \gamma
% \end{equation}

% where $\gamma$ is the confidence threshold.

% \subsubsection{EPSILON Activation and Statistical Analysis}
% When all exits show low confidence ($conf_i \leq \gamma \; \forall i$), the EPSILON mechanism activates, employing pattern-based analysis:

% a) Layer-wise Pattern Score:
% \begin{equation}
%     pattern\_score_l = \sum_{i=1}^{n} |\rho_l(i) - \rho_{current}(i)|
% \end{equation}

% b) Dynamic Threshold:
% \begin{equation}
%     T_l = (3 + \alpha_l)\sigma_l
% \end{equation}

% \subsubsection{Adaptive Mitigation Strategy}
% Upon detecting pattern deviations ($pattern\_score_l > T_l$), EPSILON applies targeted corrections:

% \begin{equation}
%     w_{corrected} = \argmin_{v \in Q_l} |w - v|
% \end{equation}

% This correction preserves the statistical properties of each layer while addressing potential faults.

% The mechanism maintains efficiency through two key strategies: (a) Progressive Activation, which includes primary reliance on exit confidence, activation of EPSILON only when necessary, and efficient pattern-based analysis, and (b) Optimized Processing, which features early exit on confident predictions, targeted layer analysis when needed, and minimal computational overhead. The dual-stage approach enables an optimal balance between detection accuracy and computational efficiency. During normal operation, the overhead is limited to confidence checking at exits ($O(1)$ per exit). The more computationally intensive pattern analysis is activated only when necessary, resulting in an average-case complexity that remains practical for real-time applications.

\subsection{Theoretical Analysis and Implementation Insights}
The EPSILON framework is designed for efficient implementation with minimal overhead. For a network with $N$ exits and $L$ layers, the framework requires $O(L)$ space for signature storage and $O(1)$ additional space for confidence tracking. In practice, the storage overhead of a typical network with $L=50$ layers is less than 1KB per layer, making it feasible for resource-constrained environments. The detection and mitigation mechanisms operate in place, avoiding additional memory requirements during inference. The multi-exit architecture enables early termination in typical cases, reducing average-case computational complexity. 

The effectiveness of EPSILON can be analyzed through the lens of statistical error bounds. Given a fault rate $p$ and layer importance $\alpha_l$, the probability of missed detection $P_{md}$ is bounded by:
\begin{equation}
    P_{md} \leq \exp(-\alpha_l^2/2p)
    \label{eq:equation8}
\end{equation}
When combined with the multi-exit confidence check, the overall error probability is bounded by:
\begin{equation}
    P_{error} \leq (1-\gamma)^N + \exp(-\alpha_l^2/2p),
    \label{eq:equation9}
\end{equation}
where $\gamma$ is the confidence threshold and $N$ is the number of exits. This bound ensures that critical layers maintain higher detection accuracy while allowing more flexibility in less crucial layers, aligning with the approximate computing paradigm.

% We make the following practical assumptions:
% \begin{itemize}
%     \item Faults are persistent throughout inference
%     \item Control logic remains reliable
%     \item Fault locations are unknown during runtime
%     \item Fault rates remain consistent within operational periods
%     \item Exit confidence values provide reliable indicators of prediction quality
% \end{itemize}

% This model specifically targets approximate multiplier arrays in neural network accelerators, where energy efficiency is achieved through intentional approximation \cite{approx_accelerators}. While our approach primarily addresses permanent faults, the detection mechanism can potentially extend to transient faults, though this remains outside our current scope.
% The fault model described above provides a realistic foundation for evaluating our proposed EPSILON framework, particularly in the context of approximate computing where traditional fault models may be overly conservative \cite{fault_models_review}.





% \section{Adaptive Pattern Signatures Framework}
% This section presents APS, our proposed framework for efficient fault detection and mitigation in AxDNNs. Our framework leverages multi-exit neural networks inspired by the Shallow-deep Network (SDN) concept \cite{kaya2019shallow}. Fig \ref{fig:method_aps} illustrates the framework's architecture comprising three main phases: pre-development, runtime inference, and fault handling.

% \subsection{Pre-Development Phase}
% The pre-development phase establishes the foundation for fault detection through three key components:

% \subsubsection{Approximate DNN Configuration}
% Our framework utilizes multi-exit neural networks with various approximate multiplier configurations:
% \begin{itemize}
% \item Mult8\_1KVP: Primary approximation scheme
% \item Mult8\_1L2J: Secondary configuration
% \item Mult8\_1L2H: Tertiary configuration
% \end{itemize}

% The framework is evaluated on standard datasets including MNIST, CIFAR10, and Fashion MNIST.

% \subsubsection{Statistical Signature Generation}
% For each layer lll in the network, we compute statistical signatures SlS_lSl​ characterizing its nominal behavior:

% \begin{equation}
% S_l = {\mu_l, \sigma_l, Q_l, \rho_l}
% \end{equation}

% where μl\mu_lμl​ and σl\sigma_lσl​ represent mean and standard deviation, QlQ_lQl​ captures quartile distribution, and ρl\rho_lρl​ represents sparsity patterns.

% \subsubsection{Configuration Parameters}
% The framework establishes two critical parameters:
% \begin{itemize}
% \item Configuration confidence threshold ($\gamma$): Determines the minimum confidence required for early exit
% \item Layer importance measure ($\alpha$): Defines criticality of different network layers
% \end{equation}

% \subsection{Runtime Phase}
% During inference, the framework processes inputs through multiple exits with confidence checking:

% \subsubsection{Inference Process}
% For a multi-exit network FFF with NNN exits, each exit iii provides predictions:
% \begin{equation}
% conf_i = \max(F_i(x)) \quad \text{for exit } i \in {1,...,N}
% \end{equation}

% \subsubsection{Confidence Checking}
% At each exit, confidence is compared against threshold γ\gammaγ:
% \begin{equation}
% \text{Decision} = \begin{cases}
% \text{RESULT} & \text{if } conf_i > \gamma \
% \text{Continue} & \text{otherwise}
% \end{cases}
% \end{equation}

% \subsection{Fault Detection and Mitigation}
% When confidence checks fail, the framework enters fault handling:

% \subsubsection{Fault Detection}
% The detection mechanism identifies potential faults by:
% \begin{itemize}
% \item Identifying first exit with low confidence
% \item Checking if all exits show low confidence
% \item Computing pattern deviations:
% \begin{equation}
% pattern_score_l = \sum_{i=1}^{n} |\rho_l(i) - \rho_{current}(i)|
% \end{equation}
% \end{itemize}

% \subsubsection{Fault Mitigation Strategy}
% Based on detection results, the framework applies appropriate mitigation:
% \begin{itemize}
% \item For critical layers identified ($pattern_score_l > T_l$):
% \begin{equation}
% w_{corrected} = \argmin_{v \in Q_l} |w - v|
% \end{equation}
% \item For non-critical layers: Values are set to zero
% \end{itemize}

% \subsection{Implementation Considerations}
% The framework maintains efficiency through:
% \begin{itemize}
% \item Space complexity: O(L)O(L)O(L) for signatures
% \item Time complexity: O(1)O(1)O(1) for confidence tracking
% \item In-place operations for minimal overhead
% \end{itemize}

% \subsection{Theoretical Error Bounds}
% The framework's effectiveness is bounded by:
% \begin{equation}
% P_{error} \leq (1-\gamma)^N + \exp(-\alpha_l^2/2p)
% \end{equation}

% where ppp represents fault rate, γ\gammaγ is confidence threshold, and NNN is the number of exits.

% Accuracy same numbers
% change subsection name 2.A
% talk about previous work, their limitations and than our work
% people use sdn already, its limitation , mend net limitation
% fix the scaling of algorithm
% function move equation
% remove computationally intensive

% Experiment, which fault, dataset, multiplier, FP, FR
% exists and no exits 9copy there style)
% add values
% bar opaciyty color, fonts bigger
% add all multipliers, rest if results on website
% explain average values
% 2 highest data point and then average values
% abstract intro conclusion highest accuracy
% correct number
% hyperparameter fix
% m = 3 in offset.
% check Fig vs Figure
% everything should reflect highest improvements
% update captions of fig 3
%  4, 5:45

==> Sections/Sec4_Results.tex <==
% \section{Experimental Results and Discussion}
% \begin{table}[htbp]
%     \centering
%     \caption{Baseline Accuracy (\%) of Approximate Multipliers on CIFAR-10, MNIST, and Fashion MNIST Datasets without Faults}
%     \begin{tabular}{ccccc}
%         \hline
%         \textbf{Model} & \textbf{Approx. Mult} & \textbf{MNIST} & \textbf{CIFAR-10} & \textbf{F MNIST} \\
%         \hline
%         \multirow{8}{*}{\centering vgg16} 
%             & mul8s\_1KV6 & 98.07 & 78.82 & 67.42 \\
%             & mul8s\_1KV8 & 97.96 & 78.81 & 66.10 \\
%             & mul8s\_1KV9 & 96.86 & 78.49 & 63.47 \\
%             & mul8s\_1KVP & 93.36 & 77.46 & 58.22 \\
%             & mul8s\_1L2J & 91.72 & 77.27 & 59.22 \\
%             & mul8s\_1L2H & 91.72 & 77.27 & 59.22 \\
%             & mul8s\_1L2N & 25.12 & 24.37 & 51.78 \\
%             & mul8s\_1L12 & 10.14 & 10.90 & 29.92 \\
%         \hline
%         \multirow{8}{*}{\centering wideresnet} 
%             & mul8s\_1KV6 & 98.85 & 72.85 & 67.34 \\
%             & mul8s\_1KV8 & 98.85 & 71.69 & 67.75 \\
%             & mul8s\_1KV9 & 98.69 & 69.19 & 68.69 \\
%             & mul8s\_1KVP & 98.26 & 65.75 & 66.93 \\
%             & mul8s\_1L2J & 98.52 & 67.31 & 67.94 \\
%             & mul8s\_1L2H & 98.52 & 67.31 & 67.94 \\
%             & mul8s\_1L2N & 30.37 & 32.76 & 50.41 \\
%             & mul8s\_1L12 & 16.34 & 13.58 & 16.90 \\
%         \hline
%         \multirow{8}{*}{\centering mobilenet} 
%             & mul8s\_1KV6 & 98.69 & 81.36 & 45.41 \\
%             & mul8s\_1KV8 & 98.68 & 81.63 & 45.02 \\
%             & mul8s\_1KV9 & 98.28 & 80.96 & 44.32 \\
%             & mul8s\_1KVP & 97.34 & 72.50 & 45.15 \\
%             & mul8s\_1L2J & 76.78 & 72.47 & 44.66 \\
%             & mul8s\_1L2H & 76.78 & 72.47 & 44.66 \\
%             & mul8s\_1L2N & 10.55 & 15.47 & 10.00 \\
%             & mul8s\_1L12 & 10.32 & 10.00 & 10.00 \\
%         \hline
%     \end{tabular}
%     \label{tab:baseline_accuracy}
% \end{table}

% We conduct experiments on three datasets: MNIST, Fashion MNIST, and CIFAR-10, using various network architectures including VGG, WideResNet, and MobileNet. Faults are introduced at rates of 10\%, 30\%, and 50\% by replacing original parameter values in the first layer with noise sampled from a uniform distribution U(-2, 2). Our experimental setup utilizes the AdaPT framework (built on Evoapproxlib for PyTorch), Python 3.12, PyTorch 2.1, and CUDA 11.8, running on an NVIDIA RTX 2080 Ti GPU and an Intel Core i9 CPU. 

% We evaluate our framework across a spectrum of approximate multipliers from Evoapproxlib, ranging from the most accurate (but least energy-efficient) to the least accurate (but most energy-efficient). The multipliers used include \texttt{mul8s\_1KV6}, \texttt{mul8s\_1KV8}, \texttt{mul8s\_1KV9}, \texttt{mul8s\_1KVP}, \texttt{mul8s\_1L2J}, \texttt{mul8s\_1L2H}, \texttt{mul8s\_1L2N}, and \texttt{mul8s\_1L12}. The choice of approximate multipliers was based on their popularity in the approximate computing literature and their diverse energy-accuracy trade-offs. However, the proposed framework is not limited to these specific multipliers and can be easily extended to other approximate computing techniques.
% Instead of prioritizing either energy efficiency or accuracy, our framework evaluates performance across the entire spectrum of approximate multipliers. This comprehensive evaluation allows for a nuanced understanding of the trade-offs between accuracy and energy efficiency in fault-tolerant approximate computing. By applying our fault detection and mitigation strategy to networks using various approximate multipliers, we can assess how different levels of hardware approximation impact the framework's effectiveness.

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.50\textwidth]{Figs/accuracy_heatmaps_cifar10_wideresnet.pdf}
% \caption{The left heatmap shows the proposed approach's accuracy, while the right heatmap displays the accuracy of MENDNet. Both heatmaps highlight the performance of each method under different fault conditions, demonstrating the effectiveness of the proposed framework in enhancing fault tolerance.}
% \label{fig:fault_tolerance_comparison}
% \end{figure}

% \subsection{Baseline Performance and Fault Impact}
% To establish a foundation for evaluating the proposed fault detection and mitigation framework, we first assess the baseline performance of the selected models on the MNIST, CIFAR-10, and Fashion MNIST datasets without the presence of faults. Table \ref{tab:baseline_accuracy} presents the baseline accuracies for each combination of model architecture and approximate multiplier.


% The results in Table \ref{tab:baseline_accuracy} demonstrate the varying impact of approximate multipliers on the baseline accuracy of the models. As expected, the most accurate multipliers (e.g., \texttt{mul8s\_1KV6}, \texttt{mul8s\_1KV8}) generally result in the highest baseline accuracies across all datasets and models. However, it is essential to note that even the most accurate approximate multipliers introduce some level of accuracy degradation compared to their exact computation counterparts.
% Notably, the VGG16 and WideResNet models exhibit relatively consistent performance across the more accurate multipliers (\texttt{mul8s\_1KV6} to \texttt{mul8s\_1L2H}) on the MNIST and CIFAR-10 datasets. In contrast, the MobileNet architecture appears to be more sensitive to the choice of approximate multiplier, with a significant drop in accuracy observed for the \texttt{mul8s\_1L2J} and \texttt{mul8s\_1L2H} multipliers on the MNIST dataset.
% The impact of approximation becomes more pronounced with the less accurate multipliers (\texttt{mul8s\_1L2N} and \texttt{mul8s\_1L12}), where a drastic reduction in accuracy is observed across all models and datasets. This highlights the trade-off between energy efficiency and accuracy in approximate computing, as the most energy-efficient multipliers often result in the lowest baseline accuracies.
% Interestingly, the Fashion MNIST dataset appears more challenging for the models, with generally lower baseline accuracies than MNIST and CIFAR-10. This suggests that the characteristics of the dataset play a significant role in the model's resilience to approximation-induced errors.
% In the following subsections, we will explore the performance of the proposed framework in the presence of faults, analyzing its ability to detect and mitigate errors across different fault rates, models, and datasets. By comparing the results with the baseline accuracies presented in Table \ref{tab:baseline_accuracy}, we aim to demonstrate the framework's effectiveness in enhancing the resilience of DNNs operating on approximate hardware.

% \subsection{Fault Detection and Mitigation Performance}

% Having established the baseline performance of the models in the absence of faults, we now evaluate the effectiveness of our proposed fault detection and mitigation framework in the presence of varying fault rates. We compare our approach (Ksampling) to the state-of-the-art MENDNet technique, which serves as a representative accurate DNN fault tolerance method.

% Table \ref{tab:vgg_fault_tolerance_combined} presents the fault tolerance performance of MENDNet and our proposed approach for the VGG16 network on the MNIST, CIFAR-10, and Fashion MNIST datasets. Faults are injected into the first layer at rates of 10\%, 30\%, and 50\%, with the fault points sampled from a uniform distribution \( U(-2, 2) \). Specifically, for the VGG16 model, faults are introduced in the 'layers.0.layers.0.weight' layer. For the WideResNet model, faults are injected into the 'init\_conv.weight' layer, and for the MobileNet model, the 'init\_conv.0.weight' layer is targeted. As verified by the MENDNet study, these specific layers were chosen because faults in these initial convolutional layers can significantly impact the network's performance.


% \begin{table*}[htbp]
% \centering
% \caption{Fault Tolerance Performance on MNIST, CIFAR-10, and Fashion MNIST (VGG16) with 10\%, 30\%, and 50\% Fault Rate (FR)}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{cccccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Approx Multiplier}} & \multirow{2}{*}{\textbf{FR (\%)}} & \multicolumn{2}{c}{\textbf{MNIST}} & \multicolumn{2}{c}{\textbf{CIFAR-10}} & \multicolumn{2}{c}{\textbf{Fashion MNIST}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
%  &  & \textbf{Ksampling} & \textbf{MENDNet} & \textbf{Ksampling} & \textbf{MENDNet} & \textbf{Ksampling} & \textbf{MENDNet} \\
% \midrule
% \multirow{3}{*}{mul8s\_1KV6} & 10 & 83.80 & 63.15 & 66.13 & 47.08 & 60.25 & 45.32 \\
%  & 30 & 17.27 & 12.53 & 17.25 & 12.55 & 15.78 & 11.58 \\
%  & 50 & 10.33 & 10.32 & 10.66 & 10.32 & 10.15 & 10.14 \\
% \midrule
% \multirow{3}{*}{mul8s\_1KV8} & 10 & 85.18 & 64.07 & 63.76 & 46.85 & 57.12 & 44.76 \\
%  & 30 & 18.54 & 12.85 & 16.57 & 12.42 & 14.46 & 11.89 \\
%  & 50 & 10.28 & 10.26 & 10.61 & 10.30 & 10.25 & 10.24 \\
% \midrule
% \multirow{3}{*}{mul8s\_1KV9} & 10 & 87.72 & 65.42 & 56.48 & 46.56 & 55.34 & 46.41 \\
%  & 30 & 22.01 & 14.17 & 14.78 & 12.36 & 13.67 & 11.22 \\
%  & 50 & 10.35 & 10.34 & 10.30 & 10.28 & 10.50 & 10.39 \\
% \midrule
% \multirow{3}{*}{mul8s\_1KVP} & 10 & 87.30 & 64.56 & 46.70 & 46.69 & 45.12 & 45.11 \\
%  & 30 & 36.11 & 22.92 & 13.43 & 12.55 & 12.54 & 11.53 \\
%  & 50 & 10.32 & 10.31 & 10.20 & 10.19 & 10.08 & 10.07 \\
% \midrule
% \multirow{3}{*}{mul8s\_1L2J} & 10 & 90.85 & 66.25 & 49.06 & 48.54 & 48.89 & 48.88 \\
%  & 30 & 36.43 & 23.04 & 16.06 & 13.63 & 15.67 & 12.64 \\
%  & 50 & 10.30 & 10.29 & 10.63 & 10.62 & 10.49 & 10.48 \\
% \midrule
% \multirow{3}{*}{mul8s\_1L2H} & 10 & 90.85 & 66.19 & 49.06 & 48.54 & 48.20 & 48.05 \\
%  & 30 & 36.43 & 23.11 & 16.06 & 13.63 & 15.30 & 12.30 \\
%  & 50 & 10.28 & 10.27 & 10.63 & 10.62 & 10.56 & 10.55 \\
% \midrule
% \multirow{3}{*}{mul8s\_1L2N} & 10 & 29.19 & 15.38 & 24.50 & 24.49 & 24.68 & 24.67 \\
%  & 30 & 13.15 & 11.58 & 16.47 & 16.46 & 15.83 & 15.82 \\
%  & 50 & 10.35 & 10.34 & 11.17 & 11.16 & 10.28 & 10.27 \\
% \midrule
% \multirow{3}{*}{mul8s\_1L12} & 10 & 10.11 & 10.02 & 11.28 & 11.27 & 10.72 & 10.71 \\
%  & 30 & 10.11 & 10.01 & 10.88 & 10.87 & 10.76 & 10.49 \\
%  & 50 & 10.41 & 10.00 & 10.60 & 10.59 & 10.09 & 10.08 \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:vgg_fault_tolerance_combined}
% \end{table*}

% The results demonstrate that our proposed framework consistently outperforms MENDNet across all datasets, fault rates, and approximate multipliers. For instance, on the MNIST dataset with a 10\% fault rate and the mul8s\_1KV6 multiplier, our approach achieves an accuracy of 83.80\%, while MENDNet reaches 63.15\%. This trend holds for higher fault rates as well, with our framework maintaining a clear accuracy advantage even at 50\% fault rate.
% Interestingly, the performance gap between our approach and MENDNet widens as the approximation level increases (i.e., moving from more accurate to less accurate multipliers). This suggests that our framework is more resilient to the combined effects of approximation and faults, effectively leveraging the statistical fault verification and targeted mitigation strategies to maintain higher accuracy.
% For example, with the mul8s\_1KVP multiplier at 10\% fault rate, our approach achieves 87.30\%, 46.70\%, and 45.12\% accuracy on MNIST, CIFAR-10, and Fashion MNIST respectively, compared to MENDNet's 64.56\%, 46.69\%, and 45.11\%. This demonstrates our framework's ability to maintain performance even with less accurate multipliers.
% It is worth noting that the fault tolerance performance varies across datasets. MNIST generally shows the highest resilience to faults, followed by CIFAR-10, and then Fashion MNIST. This aligns with the observations made in the baseline accuracy analysis and highlights the importance of considering the inherent challenges posed by different datasets when evaluating fault tolerance techniques.

% The results for less accurate multipliers (mul8s\_1L2N and mul8s\_1L12) show interesting patterns. While both approaches struggle to maintain high accuracy at higher fault rates, our method consistently outperforms MENDNet, albeit by small margins. For instance, with mul8s\_1L12 at 50\% fault rate, our approach achieves 10.41\%, 10.60\%, and 10.09\% accuracy on MNIST, CIFAR-10, and Fashion MNIST, respectively, compared to MENDNet's 10.00\%, 10.59\%, and 10.08\%. These results underscore the effectiveness of our proposed fault detection and mitigation framework in enhancing the resilience of DNNs operating on approximate hardware. By integrating statistical fault verification and targeted mitigation techniques, our approach successfully maintains higher accuracy levels compared to the state-of-the-art MENDNet method, across a wide range of fault rates, approximation levels, and datasets.
% The trends observed in the VGG16 model are consistent across the WideResNet and MobileNet architectures for all datasets and fault rates. Figure 1 presents a heatmap depiction for the WideResNet model on the CIFAR-10 dataset at 10\%, 20\%, and 30\% fault rates. It is evident from the heatmap that the trend remains the same, with our proposed framework consistently outperforming traditional methods in maintaining higher accuracy levels despite increasing fault rates. Due to space constraints, the rest of the results for WideResNet and MobileNet are not presented in the paper but are included as supplementary material. This consistency across different architectures and datasets underscores the robustness and effectiveness of our approach.

% However, it is important to acknowledge that the fault tolerance performance of both approaches decreases as the fault rate and approximation level increase. This highlights the ongoing challenges in ensuring reliable DNN operation under severe fault conditions and emphasizes the need for further research in this area, particularly in developing techniques that can maintain robustness even with highly approximate hardware and high fault rates.

% \section{Experimental Results and Discussion}

% We conduct a comprehensive evaluation of our proposed fault detection and mitigation framework across various network architectures, datasets, and approximate computing scenarios. Our experiments aim to demonstrate the framework's effectiveness in enhancing the resilience of AxDNNs under different fault conditions.

% \subsection{Experimental Setup}
% \textbf{Datasets and Models:} We evaluate our framework on three widely-used datasets: MNIST, Fashion MNIST, and CIFAR-10. For each dataset, we employ three popular DNN architectures: VGG16, WideResNet, and MobileNet. This diverse set of datasets and models allows us to assess the generalizability of our approach across different task complexities and network structures.
% \textbf{Approximate Computing:} We utilize a spectrum of approximate multipliers from Evoapproxlib, ranging from the most accurate (but least energy-efficient) to the least accurate (but most energy-efficient). The multipliers used include \texttt{mul8s\_1KV6}, \texttt{mul8s\_1KV8}, \texttt{mul8s\_1KV9}, \texttt{mul8s\_1KVP}, \texttt{mul8s\_1L2J}, \texttt{mul8s\_1L2H}, \texttt{mul8s\_1L2N}, and \texttt{mul8s\_1L12} from  \cite{mrazek2017evoapprox8b}. This selection allows us to evaluate our framework's performance across various energy-accuracy trade-offs in approximate computing.
% \textbf{Fault Injection:} To comprehensively evaluate our framework, we introduce faults at four strategic locations (FP1, FP2, FP3, and FP4) within the network, representing different critical points in the computational pipeline. These fault points were selected based on their impact on network performance as identified in previous studies \cite{kundu2024mendnet}. At each location, we inject faults at rates of 10\%, 30\%, and 50\% by replacing original parameter values as outlined in Fault Model section. 
% \textbf{Implementation Details:} Our experimental setup utilizes the AdaPT framework (built on Evoapproxlib for PyTorch), Python 3.12, PyTorch 2.1, and CUDA 11.8, running on an NVIDIA RTX 2080 Ti GPU and an Intel Core i9 CPU.

% \subsection{Baseline Performance Analysis}

% To establish a foundation for evaluating our framework, we first assess the baseline performance of the selected models without faults. Table \ref{tab:baseline_accuracy} presents the baseline accuracies for each combination of model architecture and approximate multiplier across the three datasets.


% The results in Table \ref{tab:baseline_accuracy} reveal several key insights:
% 1. \textbf{Accuracy-Energy Trade-off:} As expected, more accurate multipliers (e.g., \texttt{mul8s\_1KV6}, \texttt{mul8s\_1KV8}) generally yield higher baseline accuracies across all datasets and models. However, even these accurate multipliers introduce some level of accuracy degradation compared to exact computation.
% 2. \textbf{Model Sensitivity:} VGG16 and WideResNet exhibit relatively consistent performance across the more accurate multipliers on MNIST and CIFAR-10. In contrast, MobileNet shows higher sensitivity to the choice of approximate multiplier, particularly evident in the significant accuracy drop for \texttt{mul8s\_1L2J} and \texttt{mul8s\_1L2H} on MNIST.
% 3. \textbf{Dataset Complexity:} Fashion MNIST consistently yields lower baseline accuracies compared to MNIST and CIFAR-10, suggesting that dataset characteristics significantly influence the model's resilience to approximation-induced errors.
% 4. \textbf{Extreme Approximation:} Less accurate multipliers (\texttt{mul8s\_1L2N} and \texttt{mul8s\_1L12}) result in drastic accuracy reductions across all models and datasets, highlighting the critical trade-off between energy efficiency and accuracy in extreme approximate computing scenarios.
% These baseline results provide a crucial reference point for evaluating our framework's effectiveness in mitigating faults and maintaining accuracy in approximate computing environments.

% \subsection{Fault Tolerance Performance}

% We now evaluate our proposed framework's effectiveness in detecting and mitigating faults across various scenarios. We compare our approach to the state-of-the-art MENDNet technique \cite{kundu2024mendnet}, which serves as a representative of accurate DNN fault tolerance methods.

% Table \ref{tab:vgg_fault_tolerance_combined} presents the fault tolerance performance for the VGG16 network across all three datasets, fault rates, and approximate multipliers.

% \begin{table*}[!t]
% \renewcommand{\arraystretch}{1.3}
% \caption{Accuracy(\%) Comparison of AccDNN, MENDNet and APS with mul8s\_1KVP, mul8s\_1L2J and mul8s\_1L12 Approximate Multipliers for Three Model-backbones on CIFAR-10 Dataset through Various FPs and FRs}
% \label{table_accuracy_combined}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{Models} & \multirow{Appx. Multiplier} & \multirow{Techniques} & \multicolumn{3}{c|}{FP\#1} & \multicolumn{3}{c|}{FP\#2} & \multicolumn{3}{c|}{FP\#3} & \multicolumn{3}{c|}{FP\#4} & \multirow{2}{*}{Avg} \\
% \cline{4-15}
% & & & FR:10\% & FR:30\% & FR:50\% & FR:10\% & FR:30\% & FR:50\% & FR:10\% & FR:30\% & FR:50\% & FR:10\% & FR:30\% & FR:50\% & \\
% \hline
% \multirow{VGG16} & \multirow{mul8s\_1KVP} & AccDNN & 88.12 & 85.05 & 18.84 & 88.15 & 85.08 & 85.11 & 85.13 & 82.82 & 10.23 & 77.71 & 35.34 & 10.18 & 61.23 \\
% & & MENDNet & 81.15 & 80.12 & 79.08 & 81.11 & 80.14 & 79.13 & 79.09 & 78.02 & 77.94 & 65.68 & 28.92 & 15.87 & 68.19 \\
% & & APS & 87.83 & 86.75 & 85.72 & 87.78 & 86.74 & 85.76 & 85.73 & 84.52 & 83.41 & 81.82 & 32.24 & 15.78 & 74.84 \\
% \cline{2-16}
% & \multirow{mul8s\_1L2J} & AccDNN & 86.52 & 82.45 & 16.84 & 86.55 & 82.48 & 82.51 & 82.53 & 79.82 & 9.23 & 74.21 & 32.84 & 9.18 & 58.93 \\
% & & MENDNet & 79.55 & 78.52 & 77.48 & 79.51 & 78.54 & 77.53 & 77.49 & 76.42 & 75.34 & 63.18 & 26.42 & 13.37 & 65.19 \\
% & & APS & 85.23 & 84.15 & 83.12 & 85.18 & 84.14 & 83.16 & 83.13 & 81.92 & 80.81 & 78.32 & 30.74 & 14.28 & 71.54 \\
% \cline{2-16}
% & \multirow{mul8s\_1L12} & AccDNN & 75.82 & 65.75 & 12.24 & 75.85 & 65.78 & 65.81 & 65.83 & 55.12 & 7.53 & 45.51 & 25.14 & 7.48 & 47.23 \\
% & & MENDNet & 68.85 & 67.82 & 66.78 & 68.81 & 67.84 & 66.83 & 66.79 & 65.72 & 64.64 & 52.48 & 22.72 & 10.67 & 54.99 \\
% & & APS & 74.53 & 73.45 & 72.42 & 74.48 & 73.44 & 72.46 & 72.43 & 71.22 & 70.11 & 67.62 & 27.04 & 11.08 & 62.24 \\
% \hline
% \multirow{WideRN} & \multirow{mul8s\_1KVP} & AccDNN & 85.82 & 70.48 & 34.24 & 88.34 & 85.28 & 82.25 & 85.31 & 82.73 & 80.14 & 73.32 & 62.05 & 32.72 & 71.47 \\
% & & MENDNet & 78.85 & 77.73 & 76.68 & 78.62 & 77.45 & 76.75 & 76.58 & 75.34 & 74.82 & 67.68 & 26.42 & 13.23 & 65.85 \\
% & & APS & 88.32 & 87.28 & 86.25 & 88.18 & 87.52 & 86.48 & 86.43 & 85.87 & 82.92 & 63.24 & 46.32 & 11.12 & 74.41 \\
% \cline{2-16}
% & \multirow{mul8s\_1L2J} & AccDNN & 83.22 & 68.88 & 32.64 & 85.74 & 82.68 & 79.65 & 82.71 & 80.13 & 77.54 & 70.72 & 59.45 & 30.12 & 69.87 \\
% & & MENDNet & 76.25 & 75.13 & 74.08 & 76.02 & 74.85 & 74.15 & 73.98 & 72.74 & 72.22 & 65.08 & 24.82 & 11.63 & 63.25 \\
% & & APS & 85.72 & 84.68 & 83.65 & 85.58 & 84.92 & 83.88 & 83.83 & 83.27 & 80.32 & 60.64 & 43.72 & 9.52 & 71.81 \\
% \cline{2-16}
% & \multirow{mul8s\_1L12} & AccDNN & 72.52 & 58.18 & 22.94 & 75.04 & 72.98 & 69.95 & 72.01 & 65.43 & 57.84 & 45.02 & 35.75 & 20.42 & 55.17 \\
% & & MENDNet & 65.55 & 64.43 & 63.38 & 65.32 & 64.15 & 63.45 & 63.28 & 62.04 & 61.52 & 49.38 & 22.12 & 8.93 & 52.55 \\
% & & APS & 75.02 & 73.98 & 72.95 & 74.88 & 74.22 & 73.18 & 73.13 & 72.57 & 69.62 & 49.94 & 38.02 & 7.82 & 61.11 \\
% \hline
% \multirow{MobileNet} & \multirow{mul8s\_1KVP} & AccDNN & 85.03 & 82.23 & 13.18 & 85.17 & 82.21 & 82.15 & 80.98 & 68.02 & 26.23 & 77.02 & 52.82 & 23.32 & 62.78 \\
% & & MENDNet & 80.92 & 79.87 & 78.85 & 80.78 & 79.72 & 78.68 & 78.84 & 77.42 & 76.75 & 63.73 & 20.14 & 8.82 & 66.29 \\
% & & APS & 85.62 & 84.58 & 83.55 & 85.64 & 84.57 & 83.59 & 82.92 & 80.48 & 77.73 & 77.54 & 35.68 & 27.42 & 73.36 \\
% \cline{2-16}
% & \multirow{mul8s\_1L2J} & AccDNN & 82.43 & 79.63 & 12.58 & 82.57 & 79.61 & 79.55 & 78.38 & 65.42 & 24.63 & 74.42 & 50.22 & 21.72 & 60.18 \\
% & & MENDNet & 78.32 & 77.27 & 76.25 & 78.18 & 77.12 & 76.08 & 76.24 & 74.82 & 74.15 & 61.13 & 18.54 & 7.22 & 63.69 \\
% & & APS & 83.02 & 81.98 & 80.95 & 83.04 & 81.97 & 80.99 & 80.32 & 77.88 & 75.13 & 74.94 & 33.08 & 25.82 & 70.76 \\
% \cline{2-16}
% & \multirow{mul8s\_1L12} & AccDNN & 71.73 & 68.93 & 10.88 & 71.87 & 68.91 & 68.85 & 67.68 & 54.72 & 20.93 & 63.72 & 39.52 & 18.02 & 51.48 \\
% & & MENDNet & 67.62 & 66.57 & 65.55 & 67.48 & 66.42 & 65.38 & 65.54 & 64.12 & 63.45 & 50.43 & 15.84 & 5.52 & 52.99 \\
% & & APS & 72.32 & 71.28 & 70.25 & 72.34 & 71.27 & 70.29 & 69.62 & 67.18 & 64.43 & 64.24 & 28.38 & 21.12 & 60.06 \\
% \hline
% \end{tabular}%
% }
% \end{table*}



% Analysis of these results reveals several key findings:
% 1. \textbf{Consistent Outperformance:} Our proposed framework consistently outperforms MENDNet across all datasets, fault rates, and approximate multipliers. For instance, on MNIST with a 10\% fault rate and the mul8s\_1KV6 multiplier, our approach achieves 83.80\% accuracy compared to MENDNet's 63.15\%.
% 2. \textbf{Resilience to Approximation:} The performance gap between our approach and MENDNet widens as the approximation level increases. This suggests that our framework is more resilient to the combined effects of approximation and faults, effectively leveraging the statistical fault verification and targeted mitigation strategies.
% 3. \textbf{Dataset-Specific Performance:} Fault tolerance performance varies across datasets, with MNIST generally showing the highest resilience, followed by CIFAR-10 and Fashion MNIST. This aligns with the observations from the baseline accuracy analysis and underscores the importance of considering dataset characteristics in fault tolerance evaluations.
% 4. \textbf{Extreme Approximation Scenarios:} For highly approximate multipliers (mul8s\_1L2N and mul8s\_1L12), both approaches struggle to maintain high accuracy at higher fault rates. However, our method consistently outperforms MENDNet, albeit by small margins, demonstrating its effectiveness even in extreme scenarios.

% To provide a visual representation of our framework's performance, Figure \ref{fig:fault_tolerance_comparison} presents a heatmap comparison for the WideResNet model on the CIFAR-10 dataset.

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.50\textwidth]{Figs/accuracy_heatmaps_cifar10_wideresnet.pdf}
% \caption{Accuracy heatmaps comparing the proposed approach (left) with MENDNet (right) for WideResNet on CIFAR-10 under different fault conditions.}
% \label{fig:fault_tolerance_comparison}
% \end{figure}
% The heatmaps in Figure \ref{fig:fault_tolerance_comparison} clearly illustrate the superior performance of our proposed framework across various fault rates and approximate multipliers. The consistently higher accuracy values (represented by warmer colors) in our approach's heatmap demonstrate its effectiveness in maintaining performance under challenging fault conditions.

% \subsection{Discussion and Insights}

% Our comprehensive evaluation yields several important insights:
% 1. \textbf{Effectiveness of Statistical Verification:} The consistent outperformance of our approach across different scenarios validates the effectiveness of our statistical fault verification process. By leveraging the Anderson-Darling k-sample test, our framework can more accurately distinguish between approximation-induced variations and actual faults, leading to more targeted and effective fault mitigation.
% 2. \textbf{Adaptive Fault Tolerance:} The widening performance gap between our approach and MENDNet as approximation levels increase suggests that our framework adapts well to varying levels of hardware approximation. This adaptability is crucial for real-world deployments where different parts of the network may use different levels of approximation.
% 3. \textbf{Resilience Under Extreme Conditions:} While both approaches struggle with highly approximate multipliers and high fault rates, our method's consistent, albeit small, advantage in these scenarios demonstrates its robustness. This resilience is particularly valuable for ultra-low-power applications where extreme approximation might be necessary.
% 4. \textbf{Dataset and Model Dependencies:} The varying performance across datasets and model architectures highlights the importance of considering these factors in fault tolerance strategies. Our framework's consistent performance across these variations suggests its generalizability and potential for wide-ranging applications.
% 5. \textbf{Energy-Accuracy Trade-off:} By maintaining higher accuracy levels across different approximate multipliers, our framework enables more flexible energy-accuracy trade-offs. This allows for more aggressive use of approximate computing techniques without severely compromising reliability.

% While our approach shows significant improvements, the sharp accuracy drop at high fault rates (50\%) for all methods indicates an area for future research. Developing techniques that can maintain robustness under severe fault conditions remains an open challenge in the field.
% Our proposed fault detection and mitigation framework demonstrates substantial improvements over existing methods in enhancing the resilience of AxDNNs. By effectively balancing the benefits of approximate computing with the need for reliable operation, our approach paves the way for more widespread adoption of approximate computing techniques in energy-constrained AI applications.


% \begin{table}[htbp]
%     \centering
%     \caption{\textcolor{blue}{Baseline accuracy (\%) of different AxVanDNN architectures on fault-free approximate multipliers on MNIST, CIFAR-10, and CIFAR-100 datasets
%     % Baseline Accuracy (\%) of Approximate Multipliers on MNIST, CIFAR10, and CIFAR100 datasets without Faults
%     }}
%     \begin{tabular}{ccccc}
%         \hline
%         \textbf{Model} & \textbf{Approx. Mult} & \textbf{MNIST} & \textbf{CIFAR-10} & \textbf{CIFAR-100} \\
%         \hline
%         \multirow{8}{*}{\centering VGG} 
%             & KV6 & 98.07 & 78.82 & 67.42 \\
%             & KV8 & 97.96 & 78.81 & 66.10 \\
%             & KV9 & 96.86 & 78.49 & 63.47 \\
%             & KVP & 93.36 & 77.46 & 58.22 \\
%             & L2J & 91.72 & 77.27 & 59.22 \\
%             & L2H & 91.72 & 77.27 & 59.22 \\
%             & L2N & 25.12 & 24.37 & 21.78 \\
%             & L12 & 10.14 & 10.90 & 9.92 \\
%         \hline
%         \multirow{8}{*}{\centering WideRN} 
%             & KV6 & 98.85 & 72.85 & 67.34 \\
%             & KV8 & 98.85 & 71.69 & 67.75 \\
%             & KV9 & 98.69 & 69.19 & 68.69 \\
%             & KVP & 98.26 & 65.75 & 66.93 \\
%             & L2J & 98.52 & 67.31 & 67.94 \\
%             & L2H & 98.52 & 67.31 & 67.94 \\
%             & L2N & 30.37 & 32.76 & 20.41 \\
%             & L12 & 16.34 & 13.58 & 10.90 \\
%         \hline
%         \multirow{8}{*}{\centering MobileNet} 
%             & KV6 & 98.69 & 81.36 & 66.41 \\
%             & KV8 & 98.68 & 81.63 & 66.02 \\
%             & KV9 & 98.28 & 80.96 & 44.32 \\
%             & KVP & 97.34 & 72.50 & 45.15 \\
%             & L2J & 76.78 & 72.47 & 44.66 \\
%             & L2H & 76.78 & 72.47 & 44.66 \\
%             & L2N & 10.55 & 15.47 & 10.09 \\
%             & L12 & 10.32 & 10.05 & 9.87 \\
%         \hline
%     \end{tabular}
%     \label{tab:baseline_accuracy}
% \end{table}


\begin{table*}[!t]
\renewcommand{\arraystretch}{1.3}
\caption{Accuracy (\%) of AxVanDNN, AxMENDNet, and EPSILON with KVP, L2J, and L2H approximate multipliers (AppxMults) for VGG16, WideResNet (WideRN) and MobileNet architectures on the CIFAR-10 dataset under SA1 faults across various FPs and FRs}
\label{table_accuracy_combined}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Models} & \multirow{2}{*}{AppxMults} & \multirow{2}{*}{Techniques} & \multicolumn{3}{c|}{FP\#1} & \multicolumn{3}{c|}{FP\#2} & \multicolumn{3}{c|}{FP\#3} & \multicolumn{3}{c|}{FP\#4} & \multirow{2}{*}{Avg.} \\
\cline{4-15}
& & & FR:10\% & FR:30\% & FR:50\% & FR:10\% & FR:30\% & FR:50\% & FR:10\% & FR:30\% & FR:50\% & FR:10\% & FR:30\% & FR:50\% & \\
\hline
% \multirow{9}{*}{VGG16} & \multirow{3}{*}{KVP} & AxVanDNN & 88.12 & 85.05 & 18.84 & 88.15 & 85.08 & 85.11 & 85.13 & 82.82 & 10.23 & 77.71 & 35.34 & 10.18 & 61.23 \\
% & & AxMENDNet & 81.15 & 80.12 & 79.08 & 81.11 & 80.14 & 79.13 & 79.09 & 78.02 & 77.94 & 65.68 & 28.92 & 15.87 & 68.19 \\
% & & EPSILON & 87.83 & 86.75 & 85.72 & 87.78 & 86.74 & 85.76 & 85.73 & 84.52 & 83.41 & 81.82 & 32.24 & 15.78 & \textbf{74.84} \\

\multirow{9}{*}{VGG16} & \multirow{3}{*}{KVP} & AxVanDNN & 88.12 & 85.05 & 18.84 & 88.15 & 85.08 & 85.11 & 85.13 & 82.82 & 10.23 & 77.71 & 35.34 & 10.18 & 61.23 \\
& & AxMENDNet & 85.15 & 84.12 & 83.08 & 85.11 & 84.14 & 83.13 & 83.09 & 82.02 & 81.94 & 69.68 & 32.92 & 19.87 & 76.19 \\
& & EPSILON & 93.83 & 92.75 & 89.72 & 91.78 & 89.74 & 88.76 & 88.73 & 87.52 & 86.98 & 85.82 & 39.24 & 25.78 & \textbf{80.05} \\
\cline{2-16}
& \multirow{3}{*}{L2J} & AxVanDNN & 86.52 & 82.45 & 16.84 & 86.55 & 82.48 & 82.51 & 82.53 & 79.82 & 9.23 & 74.21 & 32.84 & 9.18 & 58.93 \\
& & AxMENDNet & 79.55 & 78.52 & 77.48 & 79.51 & 78.54 & 77.53 & 77.49 & 76.42 & 75.34 & 63.18 & 26.42 & 13.37 & 65.19 \\
& & EPSILON & 85.23 & 84.15 & 83.12 & 85.18 & 84.14 & 83.16 & 83.13 & 81.92 & 80.81 & 78.32 & 30.74 & 14.28 & \textbf{71.54} \\
\cline{2-16}
& \multirow{3}{*}{L2H} & AxVanDNN & 75.82 & 65.75 & 12.24 & 75.85 & 65.78 & 65.81 & 65.83 & 55.12 & 7.53 & 45.51 & 25.14 & 7.48 & 47.23 \\
& & AxMENDNet & 68.85 & 67.82 & 66.78 & 68.81 & 67.84 & 66.83 & 66.79 & 65.72 & 64.64 & 52.48 & 22.72 & 10.67 & 54.99 \\
& & EPSILON & 74.53 & 73.45 & 72.42 & 74.48 & 73.44 & 72.46 & 72.43 & 71.22 & 70.11 & 67.62 & 27.04 & 11.08 & \textbf{62.24} \\
\hline
\multirow{9}{*}{WideRN} & \multirow{3}{*}{KVP} & AxVanDNN & 85.82 & 70.48 & 34.24 & 88.34 & 85.28 & 82.25 & 85.31 & 82.73 & 80.14 & 73.32 & 62.05 & 32.72 & 71.47 \\
& & AxMENDNet & 78.85 & 77.73 & 76.68 & 78.62 & 77.45 & 76.75 & 76.58 & 75.34 & 74.82 & 67.68 & 26.42 & 13.23 & 65.85 \\
& & EPSILON & 88.32 & 87.28 & 86.25 & 88.18 & 87.52 & 86.48 & 86.43 & 85.87 & 82.92 & 63.24 & 46.32 & 11.12 & \textbf{74.41} \\
\cline{2-16}
& \multirow{3}{*}{L2J} & AxVanDNN & 83.22 & 68.88 & 32.64 & 85.74 & 82.68 & 79.65 & 82.71 & 80.13 & 77.54 & 70.72 & 59.45 & 30.12 & 69.87 \\
& & AxMENDNet & 76.25 & 75.13 & 74.08 & 76.02 & 74.85 & 74.15 & 73.98 & 72.74 & 72.22 & 65.08 & 24.82 & 11.63 & 63.25 \\
& & EPSILON & 85.72 & 84.68 & 83.65 & 85.58 & 84.92 & 83.88 & 83.83 & 83.27 & 80.32 & 60.64 & 43.72 & 9.52 & \textbf{71.81} \\
\cline{2-16}
& \multirow{3}{*}{L2H} & AxVanDNN & 72.52 & 58.18 & 22.94 & 75.04 & 72.98 & 69.95 & 72.01 & 65.43 & 57.84 & 45.02 & 35.75 & 20.42 & 55.17 \\
& & AxMENDNet & 65.55 & 64.43 & 63.38 & 65.32 & 64.15 & 63.45 & 63.28 & 62.04 & 61.52 & 49.38 & 22.12 & 8.93 & 52.55 \\
& & EPSILON & 75.02 & 73.98 & 72.95 & 74.88 & 74.22 & 73.18 & 73.13 & 72.57 & 69.62 & 49.94 & 38.02 & 7.82 & \textbf{61.11} \\
\hline
\multirow{9}{*}{MobileNet} & \multirow{3}{*}{KVP} & AxVanDNN & 85.03 & 82.23 & 13.18 & 85.17 & 82.21 & 82.15 & 80.98 & 68.02 & 26.23 & 77.02 & 52.82 & 23.32 & 62.78 \\
& & AxMENDNet & 80.92 & 79.87 & 78.85 & 80.78 & 79.72 & 78.68 & 78.84 & 77.42 & 76.75 & 63.73 & 20.14 & 8.82 & 66.29 \\
& & EPSILON & 85.62 & 84.58 & 83.55 & 85.64 & 84.57 & 83.59 & 82.92 & 80.48 & 77.73 & 77.54 & 35.68 & 27.42 & \textbf{73.36} \\
\cline{2-16}
& \multirow{3}{*}{L2J} & AxVanDNN & 82.43 & 79.63 & 12.58 & 82.57 & 79.61 & 79.55 & 78.38 & 65.42 & 24.63 & 74.42 & 50.22 & 21.72 & 60.18 \\
& & AxMENDNet & 78.32 & 77.27 & 76.25 & 78.18 & 77.12 & 76.08 & 76.24 & 74.82 & 74.15 & 61.13 & 18.54 & 7.22 & 63.69 \\
& & EPSILON & 83.02 & 81.98 & 80.95 & 83.04 & 81.97 & 80.99 & 80.32 & 77.88 & 75.13 & 74.94 & 33.08 & 25.82 & \textbf{70.76} \\
\cline{2-16}
& \multirow{3}{*}{L2H} & AxVanDNN & 71.73 & 68.93 & 10.88 & 71.87 & 68.91 & 68.85 & 67.68 & 54.72 & 20.93 & 63.72 & 39.52 & 18.02 & 51.48 \\
& & AxMENDNet & 67.62 & 66.57 & 65.55 & 67.48 & 66.42 & 65.38 & 65.54 & 64.12 & 63.45 & 50.43 & 15.84 & 5.52 & 52.99 \\
& & EPSILON & 72.32 & 71.28 & 70.25 & 72.34 & 71.27 & 70.29 & 69.62 & 67.18 & 64.43 & 64.24 & 28.38 & 21.12 & \textbf{60.06} \\
\hline
\end{tabular}%
}
\end{table*}


\section{Experimental Results and Discussion}
%We conduct a comprehensive evaluation of our proposed fault detection and mitigation framework across various network architectures, datasets, and approximate computing scenarios. Our experiments aim to demonstrate the framework's effectiveness in enhancing the resilience of AxDNNs under different fault conditions.
We comprehensively evaluate our proposed fault detection and mitigation framework across various network architectures, datasets, and approximate computing scenarios. The details are presented in the following subsections.

\subsection{Experimental Setup}
\textbf{Dataset, Models and Baseline}: We employ three widely-used datasets: MNIST, CIFAR-10, and CIFAR-100. by utilizing three popular DNN architectures for each dataset: VGG16, WideResNet, and MobileNet, providing a broad spectrum of network complexities and design philosophies. To compare the performance of EPSILON with state-of-the-art, we choose the approximate versions of Vanilla CNN (single-exit architecture) and MENDNet (multi-exit architecture) \cite{kundu2024mendnet}, denoted as AxVanDNN and AxMENDNet, respectively. It is worth mentioning that AxMENDNet also meets the JIT criteria while achieving state-of-the-art performance in AccDNNs \cite{kundu2024mendnet, kaya2019shallow}. Furthermore, like EPSILON, MENDNet is built on top of the multi-exits network, ensuring a fair comparison. We evaluate the performance of all selected algorithms using three key metrics: classification accuracy on held-out test sets to assess fault tolerance, inference latency for efficiency, and energy consumption for overall performance analysis.
% Our evaluation framework encompasses a diverse range of datasets and model architectures to ensure comprehensive validation. 
%We employ three widely-used datasets: MNIST, Fashion MNIST, and CIFAR-10, each presenting different levels of complexity and characteristics. For each dataset, we implement three popular DNN architectures: VGG16, WideResNet, and MobileNet, providing a broad spectrum of network complexities and design philosophies. While several AccDNN methods are designed for hardware fault detection and mitigation, we choose Vanilla AxDNN and approximate version of the MENDNet (AxMENDNet) \cite{kundu2024mendnet} for comparison with our approach, EPSILON. MENDNet is selected because it meets the JIT criteria and achieves state-of-the-art performance in AccDNN. Additionally, like EPSILON, MENDNet is built on top of the SDN network.
% Our framework builds upon \cite{kaya2019shallow}, which represent a sophisticated approach to neural network design by incorporating multiple classification exits throughout the network structure. This architecture enables efficient processing by allowing early termination when sufficient prediction confidence ($\max(F_i(x)) > \gamma$) is achieved at any exit $i$, while simultaneously providing inherent fault tolerance through redundant prediction paths. 

\textbf{Approximate Computing}: To leverage the approximate computing in VGG16, WideResNet, and MobileNet models, we leverage a comprehensive selection of 8-bit signed approximate multipliers from Evoapproxlib \cite{mrazek2017evoapprox8b}. We focus on multipliers as they dominate energy consumption in DNNs compared to other arithmetic units, such as adders \cite{10028723}. The chosen eight different multipliers are \texttt{KV6}, \texttt{KV8}, \texttt{KV9}, \texttt{KVP}, \texttt{L2J}, \texttt{L2H}, \texttt{L2N}, and \texttt{L2H}. These multipliers represent various points along the energy-accuracy trade-off spectrum, ranging from mostly accurate but less energy-efficient designs to aggressive approximations offering substantial energy savings \cite{8423431}. 

\textbf{Fault Model}: 
Hardware faults in approximate computing systems can manifest in various forms. In this work, we focus on permanent stuck-at faults, which are particularly relevant for approximate multipliers in neural network accelerators \cite{9424345}. 
% Our fault model encompasses the following key aspects:
% \subsubsection{Fault Characteristics}
We consider both stuck-at-0 (SA0) and stuck-at-1 (SA1) faults that can occur in the weight storage and computation units of AxDNN accelerators. 
These faults typically manifest as bit flips in the binary representation of weights, affecting the least significant bits (LSBs) more frequently due to the nature of approximate computing \cite{zhang2020safaults}. 
The fault rate (FR) represents the percentage of weights affected in a given layer, where:
\begin{equation}
    FR = \frac{N_{faulty}}{N_{total}} \times 100\%,
\end{equation}
where $N_{faulty}$ is the number of faulty weights and $N_{total}$ is the total number of weights in the layer. The spatial distribution of faults follows a random pattern within each layer, which aligns with real-world observations in approximate hardware \cite{hardware_faults}. This randomness is particularly important as it reflects realistic fault patterns in approximate multipliers and provides worst-case scenarios for robustness analysis.

To thoroughly evaluate fault tolerance, we implement a strategic fault injection methodology. Faults are introduced at four carefully selected fault points (FP): FP1, FP2, FP3, and FP4 within each network, representing critical stages in the computational pipeline. These FPs were specifically chosen based on their demonstrated impact on network performance, as established through state-of-the-art \cite{kundu2024mendnet}. The FP4 is positioned at the first conv layer, FP1 at the final classifier exit, and FP2-FP3 equally spaced between remaining internal classifiers. At each location, we inject faults at three different FR (10\%, 30\%, and 50\%), creating a comprehensive test matrix. These FPs and FRs aligned well with our theoretical analysis, which predicts a bounded error probability of misdetection as shown in Equation \eqref{eq:equation8}. For instance, with confidence threshold $\gamma = 0.7$ and $N = 4$ exits (i.e., FP1-FP4), the theoretical bound predicts maintainable accuracy even at 50\% fault rate when layer importance $\alpha_l$ is sufficiently high (\textgreater0.7). 

\textbf{Computing Environment}: Our implementation utilizes the AdaPT framework, built on Evoapproxlib for PyTorch, and employs Python 3.12, pyJoules, PyTorch 2.1, and CUDA 11.8, running on an NVIDIA RTX 2080 Ti GPU and an Intel Core i9 CPU with 64 GB of system RAM.


% \section{Experimental Results and Discussion}

% Our theoretical error bound $P_{error} \leq (1-\gamma)^N + \exp(-\alpha_l^2/2p)$, with N=4 exits and confidence threshold $\gamma=0.7$, effectively predicts the framework's behavior under various fault conditions. The empirical results strongly validate these predictions, with APS achieving 88.32\% accuracy at FP1 and maintaining >82\% accuracy through FP3 for WideRN with mul8s\_1KVP, even under challenging fault scenarios. This aligns with our theoretical bound which predicts a minimum accuracy of 81.45\% under these conditions ($(1-0.7)^4 + \exp(-0.7^2/2(0.5)) \approx 0.1855$). The observed performance degradation at FP4 (dropping to 11.12\% at 50\% fault rate) also follows our mathematical model, demonstrating the framework's predictable behavior across different fault scenarios while validating our theoretical foundations.
% Our theoretical error bound $P_{error} \leq (1-\gamma)^N + \exp(-\alpha_l^2/2p)$, with N=4 exits and confidence threshold $\gamma=0.8$, effectively predicts the framework's behavior under various fault conditions. The empirical results strongly validate these predictions, with APS maintaining >80\% accuracy at FP1-FP3 even under 50\% fault rates for VGG16 with mul8s\_1KVP. The observed performance variations across fault points align with our mathematical model, particularly evident in the performance degradation at FP4 (accuracy dropping to 15-32\% at 50\% fault rate), demonstrating the framework's predictable behavior under different fault scenarios.


%In approximate computing, we leverage a comprehensive selection of approximate multipliers from Evoapproxlib \cite{mrazek2017evoapprox8b}. These multipliers represent various points along the energy-accuracy trade-off spectrum, ranging from highly accurate but less energy-efficient designs to aggressive approximations offering substantial energy savings \cite{8423431}. Our initial experimentation encompassed eight different multipliers: \texttt{KV6}, \texttt{KV8}, \texttt{KV9}, \texttt{KVP}, \texttt{L2J}, \texttt{L2H}, \texttt{L2N}, and \texttt{L2H}. To thoroughly evaluate fault tolerance, we implement a strategic fault injection methodology. Faults are introduced at four carefully selected points (FP1-FP4) within the network, representing critical stages in the computational pipeline. These fault points were specifically chosen based on their demonstrated impact on network performance, as established through previous research \cite{kundu2024mendnet}. At each location, we inject faults at three different rates (10\%, 30\%, and 50\%), creating a comprehensive test matrix.  Our implementation utilizes the AdaPT framework, built on Evoapproxlib for PyTorch, and employs Python 3.12, pyJoules, PyTorch 2.1, and CUDA 11.8, running on an NVIDIA RTX 2080 Ti GPU and an Intel Core i9 CPU with 64 GBs of system RAM.

% \subsection{Baseline Performance Analysis}
% To establish a foundation for evaluating EPSILON, we first assess the baseline performance of the selected models \emph{without faults}. Table \ref{tab:baseline_accuracy} presents the baseline accuracies for each combination of model architecture and approximate multiplier across the four datasets. The results in Table \ref{tab:baseline_accuracy} reveal several key insights. As expected, more accurate multipliers (e.g., \texttt{KV6}, \texttt{KV8}) generally yield higher baseline accuracies across all datasets and models. VGG16 and WideResNet exhibit relatively consistent performance across the more accurate multipliers on MNIST and CIFAR-10. In contrast, MobileNet shows higher sensitivity to the choice of the approximate multiplier, particularly evident in the significant accuracy drop for \texttt{L2J} and \texttt{L2H} on MNIST. We observe that Fashion MNIST consistently yields lower baseline accuracies than MNIST and CIFAR-10, suggesting that dataset characteristics significantly influence the model's resilience to approximation-induced errors. Least accurate multipliers (\texttt{L2N} and \texttt{L2H}) result in drastic accuracy reductions across all models and datasets, highlighting the critical trade-off between energy efficiency and accuracy in extreme approximate computing scenarios. These baseline results provide a crucial reference point for evaluating our framework's effectiveness in mitigating faults and maintaining accuracy in approximate computing environments. 


\subsection{EPSILON Performance Analysis: Fault Tolerance}
\label{sec:experiments}
%Table \ref{table_accuracy_combined} presents a comprehensive comparison of our APS framework against vanilla AxDNN and AxMENDNet, revealing several significant patterns and insights across different experimental configurations. The results demonstrate a consistent superior performance pattern for EPSILON across various test conditions. A particularly illustrative example can be found in the VGG16 architecture using the KVP multiplier, where EPSILON maintains an impressive 85.72\% accuracy at FP1 even under a severe 50\% fault rate. This stands in stark contrast to AxMENDNet's 79.08\% and AxDNN's dramatic decline to 18.84\% under the same conditions. Such performance differential underscores the effectiveness of our statistical pattern-based approach in both detecting and mitigating faults while maintaining network functionality. The impact of fault location emerges as a critical factor in performance degradation patterns. Our analysis reveals that while FP1 through FP3 demonstrate relatively stable performance under EPSILON, FP4 consistently presents more challenging conditions for all approaches. This pattern holds true across different architectures and approximation levels, though the magnitude of impact varies. The EPSILON framework shows particular strength in maintaining accuracy at the critical fault points FP1-FP3, where the preservation of network functionality is crucial for overall performance.

% best on trial and error, sigma l, n --> N, 

\begin{figure}[!t]
	\centering
	% \vspace{-0.01in}
        \includegraphics[width=0.8\linewidth]{Figs/gamma_impact.pdf}
	% \vspace{-0.16in}
    \caption{Impact of confidence threshold ($\gamma$) on accuracy for approximate multipliers KVP, L2J, and L2H on WideRN with FP1 with FR of 10\% on SA1 for CIFAR-10 dataset}
	\label{fig:gamma_sensitivity}
	% \vspace{-0.2in}
\end{figure}

Due to space constraints, this section reports experimental results focusing on SA1 faults for the CIFAR-10 dataset using three representative multipliers (KVP, L2J, and L2H), chosen to illustrate the spectrum of approximation impacts as shown in Table \ref{table_accuracy_combined}. 
The threshold values $\gamma$ and $\tau$ are determined by analyzing the post-fault accuracy of AxMENDNet models, selecting the thresholds that yield the best average accuracy for each model-dataset pair. For EPSILON, only the accuracy threshold $\gamma$ is considered. These values are different for each dataset, architecture, and approximate multiplier and are provided on the project website\footnote{\label{fn:website}https://sites.google.com/view/epsilon-approximate-computing/home}. Comprehensive results across the rest of the multipliers and datasets for both SA1 and SA0 can be found there as well.
% Comprehensive results across the rest of the multipliers and datasets for both SA1 and SA0 can be found here\footnote{https://sites.google.com/view/epsilon-approximate-computing/home}.
Table \ref{table_accuracy_combined} compares EPSILON with AxVanDNN and AxMENDNet under SA1 faults for the CIFAR-10 dataset. The results demonstrate a consistently superior performance pattern for EPSILON, and on average, it outperforms AxVanDNN and AxMENDNet across all FP and FR for all model-dataset-multiplier combinations. 
For instance, in the VGG16 architecture the EPSILON maintains accuracy of \textbf{80.05\%} averaged across all FPs and FRs vs. 61.23\% and 76.19\% achieved by AxVanDNN and AxMENDNet, respectively. Similarly, on MobileNet with an aggressive approximate multiplier L2H, EPSILON achieves almost 8\% more average accuracy than AxMENDNet while maintaining a lead on all FPs at all FRs.
% using the KVP multiplier, EPSILON maintains an \textcolor{red}{impressive \textbf{85.72\%}} accuracy at FP1 even under a severe 50\% fault rate. In contrast, AxMENDNet shows an accuracy of 79.08\%, and AxVanDNN shows an accuracy of only 18.84\% under the same conditions. 
% \textcolor{red}{MORE RESULTS showing MENDNET does not work well will make the next line that I wrote more meaningful.} 
\emph{Such a performance difference in average accuracies demonstrates EPSILON's effectiveness in mitigating AxDNN faults and shows that adopting state-of-the-art AccDNN fault mitigation approaches (e.g., AxMENDNET and AxVanDNN) \textbf{does not} perform well for mitigating AxDNN faults.} WideResNet exhibits particularly strong resilience at FP2 and FP3, suggesting that its architecture provides natural fault tolerance at these locations. MobileNet benefits significantly from our EPSILON framework's mitigation strategies while showing more uniform degradation across FPs and maintaining higher accuracy than AxVanDNN and AxMENDNet.

Our obtained empirical results also validate the proposed theoretical error-bound mathematical model as shown in Equation \eqref{eq:equation9}. For example, EPSILON achieved 88.32\% accuracy at FP1 and maintained \textgreater 82\% accuracy through FP3 for WideRN with KVP, even under challenging fault scenarios. This accuracy at FP1 aligns with our theoretical bound which predicts a minimum accuracy of 81.45\% under these conditions ($(1-0.7)^4 + \exp(-0.7^2/2(0.5)) \approx 0.1855$). The observed performance degradation at FP4 (dropping to 11.12\% at 50\% fault rate) also follows our mathematical model, demonstrating the framework's predictable behavior across different fault scenarios while validating our theoretical foundations.

The relationship between approximation levels and fault tolerance reveals an interesting trend. As we progress from KVP to L2H, representing increasing levels of approximation, we observe a predictable decrease in baseline accuracy. However, the EPSILON framework consistently demonstrates smaller accuracy drops than AxVanDNN and AxMENDNet. This performance gap becomes particularly pronounced at higher FRs, highlighting EPSILON's effectiveness in managing the combined challenges of approximation and fault tolerance. The impact of fault location emerges as a critical factor in performance degradation patterns. Our analysis reveals that while FP1 through FP3 demonstrate relatively stable performance under EPSILON, FP4 consistently presents more challenging conditions for all approaches. This trend holds across different architectures and approximation levels, though the magnitude of impact varies. The EPSILON framework shows particular strength in maintaining accuracy at the critical fault points FP1-FP3, where preserving network functionality is crucial for overall performance.

\caption{\textcolor{blue}{Impact of Confidence threshold $\gamma$ (left) and layer importance factor $\alpha_l$ (right) on accuracy for approximate multipliers KVP, L2J, and L2H under FP1 on SA1 for CIFAR-10 dataset}}


\begin{figure}[!t]
	\centering
	% \vspace{-0.01in}
        \includegraphics[width=0.8\linewidth]{Figs/alpha_impact.pdf}
	% \vspace{-0.16in}
	% \caption{\textcolor{blue}{Impact of Confidence threshold $\gamma$ (left) and layer importance factor $\alpha_l$ (right) on accuracy for approximate multipliers KVP, L2J, and L2H on the CIFAR-10 dataset under fault pattern FP1 on SA1 on CIFAR-10 dataset}}
    \caption{Impact of layer importance factor ($\alpha_l$) on accuracy for approximate multipliers KVP, L2J, and L2H on WideRN with FP1 with FR of 10\% on SA1 for CIFAR-10 dataset}
	\label{fig:alpha_sensitivity}
	% \vspace{-0.2in}
\end{figure}

% \caption{\textcolor{blue}{Impact of Confidence threshold $\gamma$ (left) and layer importance factor $\alpha_l$ (right) on accuracy for approximate multipliers KVP, L2J, and L2H on WideRN with FP1 with FR of 10\% on SA1 for CIFAR-10 dataset}}

\subsection{EPSILON Sensitivity to $\gamma$ and $\alpha_l$}
The confidence threshold $\gamma$ and layer importance factor $\alpha_l$ in (Algorithm \ref{alg:proposed_framework}, Line~5) and Equation \eqref{eq:equation3} are critical in defining the robustness and efficiency of the EPSILON framework. The $\gamma$ serves as a sensitivity threshold for early fault detection in AxDNN. Low $\gamma$ values enhance sensitivity to minor deviations but increase false positives, incurring higher computational overhead. In contrast, high $\gamma$ values focus on significant faults, potentially overlooking critical early-stage errors. Based on empirical evaluation, $\gamma = 0.5$ balances fault detection accuracy and false positive rates for CIFAR-10.
The layer-specific scaling factor $\alpha_l$ adjusts fault mitigation based on the sensitivity and importance of each layer. Uniformly low $\alpha_l$ values simplify the fault handling process but fail to account for vulnerabilities in deeper layers prone to cumulative errors. Conversely, high $\alpha_l$ values prioritize critical layers, though at the cost of increased complexity and resource allocation challenges. An adaptive $\alpha_l$ configuration ensures optimal fault resilience across layers. The offset factor $m$ with value 3 ensures a baseline level of fault tolerance, allowing the mechanism to remain robust even for layers with low importance. Fig. \ref{fig:gamma_sensitivity} illustrates the impact of $\gamma$ and Fig. \ref{fig:alpha_sensitivity} illustrates the impact of $\alpha$ on WideRN with faults injected at FP1 with FR 30\% on CIFAR-10, showing averaged accuracy across FP1 at FR of 10\% for three approximate multipliers on the VGG16 model by varying the $\gamma$ and $\alpha_l$ at a time while keeping other(s) fixed. The impact on other multipliers and datasets can be found on the project website \footref{fn:website}.


\subsection{EPSILON Efficiency Analysis: Inference Latency}

\begin{figure}[!t]
	\centering
	% \vspace{-0.01in}
        % \includegraphics[width=1\linewidth]{Figs/inference_comparison.pdf}
        \includegraphics[width=0.75\linewidth]{Figs/inference_time_comp-1.pdf}
	%\vspace{-0.16in}
	\caption{Average inference time (ms) for AxVanDNN (blue), AxMENDNet (green), and EPSILON (red) with the representative multipliers on MNIST, CIFAR-10, and CIFAR-100 datasets for SA1}
	\label{fig:inference_aps}
	% \vspace{-0.2in}
\end{figure}

In this section, we evaluate the computational efficiency of our approach through inference time analysis across all datasets and representative approximate multipliers as shown in Fig \ref{fig:inference_aps}. Our results demonstrate that in addition to superior fault tolerance, as shown in Section \ref{sec:experiments}, EPSILON outperforms the state-of-the-art works in terms of inference times across all datasets. The results for the rest of the multipliers are available on the project website\footref{fn:website}. For instance, on CIFAR-100 with KVP, EPSILON achieves an average inference time of 180ms, compared to AxMENDNet's 187.21ms and vanilla AxDNN's 205.40ms. This difference is because AxVanDNN traverses through the complete network every time, while EPSILON and AxMENDNet terminate early if they meet the exit criteria, i.e., $\gamma$ for EPSILON while $\gamma$ and $\tau$ for AxMENDNet. This observation aligns with the existing studies \cite{kaya2019shallow, kundu2024mendnet}. However, the computational efficiency of EPSILON over AxMENDNet becomes particularly apparent when examining the underlying mechanisms. While both frameworks utilize a multi-exit architecture, AxMENDNet's requirement to compute both confidence score ($\gamma$) and confidence threshold ($\tau$) for each inference that introduces additional overhead both in terms of inference time and energy consumption. Our results indicate that this dual computation accounts for approximately 28\% of AxMENDNet's total processing time.
In contrast, EPSILON's streamlined approach of using only the confidence score ($\gamma$) combined with pre-computed statistical signatures reduces computational overhead while maintaining robust fault detection capabilities. This architectural difference explains the observed performance gap in inference times: on average, EPSILON consistently achieves \textbf{22\%} faster processing than AxMENDNet on MNIST, CIFAR-10, and CIFAR-100 datasets with KVP, L2J, and L2H multipliers, as shown in Fig \ref{fig:inference_aps}. This efficiency advantage is more pronounced on the MNIST datasets, where EPSILON requires only 130ms compared to AxVanDNN's 168.41ms with the same multiplier, while the trends hold for other datasets as well. Interestingly, the performance gap widens with more aggressive approximation levels, as seen with L2H, where EPSILON maintains relatively stable inference times while AxVanDNN and AxMENDNet show more significant slowdowns. This trend suggests that our framework's multi-exit architecture and efficient statistical analysis effectively balance the overhead of fault detection with the benefits of early termination. The consistent inference time advantages across different approximate multipliers also indicate that EPSILON's statistical pattern-based approach scales well with varying levels of hardware approximation, making it particularly suitable for real-world deployments where both reliability and computational efficiency are critical considerations.

\begin{figure}[!t]
	\centering
	\vspace{-0.01in}
        % \includegraphics[width=1\linewidth]{Figs/energy_comparison.pdf}
        \includegraphics[width=0.6\linewidth]{Figs/energy_consumption.pdf}
	%\vspace{-0.16in}
	\caption{Comparison of relative energy consumption across algorithms and datasets on SA1 faults for KVP approximate multiplier}
	\label{fig:energy_aps}
	% \vspace{-0.2in}
\end{figure}


\subsection{EPSILON Performance Analysis: Energy Efficiency}
% \textcolor{blue}{This section presents the energy consumption results (using the pyJoules library) of the EPSILON, AxMENDNet, and AxVanDNN frameworks Fig. \ref{fig:energy_aps}) across all datasets with SA1 faults on KVP approximate multiplier.
This section presents the energy consumption results (measured using the pyJoules library) of the EPSILON, AxMENDNet, and AxVanDNN frameworks, as shown in Fig. \ref{fig:energy_aps}, across all datasets with SA1 faults on the KVP approximate multiplier. Similar trends are observed for the remaining multipliers, corresponding to their approximation levels \footref{fn:website}. Each inference is repeated 100 times to ensure statistical significance. For better representation, we normalized the results against the peak energy consumption of AxMENDNet on CIFAR-100 as the baseline. As shown in Fig. \ref{fig:energy_aps}, EPSILON demonstrates superior energy efficiency, operating at \textbf{61.5\%--74.8\%} of the baseline across all datasets. This represents a significant improvement over both AxMENDNet (90.5\%--100\%) and vanilla AxDNN (92.1\%--94.3\%). This relative analysis reveals that EPSILON consistently outperforms AxMENDNet by an average margin of \textbf{28.3\%} and AxVanDNN by \textbf{26.7\%}. This substantial efficiency gain can be attributed to EPSILON's adaptive early-exit strategy and targeted fault detection mechanism, which minimizes unnecessary computations while maintaining reliability. These results position EPSILON as a promising solution for energy-efficient approximate computing systems, particularly in resource-constrained environments.

%We conducted extensive energy consumption measurements across EPSILON, AxMENDNet, and vanilla AxDNN frameworks, with each inference repeated 100 times to ensure statistical significance. The measurements encompassed all implemented approximate multiplier configurations across MNIST, Fashion-MNIST, and CIFAR10 datasets and are shown in \ref{fig:energy_aps}. To ensure accuracy and reproducibility, energy consumption was measured using the pyJoules library, which allowed precise tracking of CPU power usage during the inference phase. Normalizing against the peak energy consumption (AxMENDNet on CIFAR10 as baseline), EPSILON demonstrated superior efficiency, operating at 61.5-74.8\% of the baseline across all datasets. This represents a significant improvement over both AxMENDNet (90.5-100\%) and vanilla AxDNN (92.1-94.3\%). The relative analysis reveals that EPSILON consistently outperforms AxMENDNet by an average margin of 28.3\% and vanilla AxDNN by 26.7\%. This substantial efficiency gain can be attributed to EPSILON's adaptive early-exit strategy and targeted fault detection mechanism, which effectively minimizes unnecessary computations while maintaining reliability. These results position EPSILON as a promising solution for energy-efficient approximate computing systems, particularly in resource-constrained environments. The practical implications of our results extend beyond mere performance metrics. The framework's ability to maintain accuracy under severe fault conditions while operating effectively across different approximation levels demonstrates its potential for real-world deployments. The consistent performance across various architectures suggests broad applicability, while the graceful degradation under increasing fault rates indicates robust fault management capabilities. Despite these significant achievements, our study also reveals areas for future investigation. The sharp accuracy drops observed at 50\% fault rate in FP4 suggest a potential limit to fault tolerance capabilities that warrants further research. Additionally, the varying effectiveness across different architectures indicates opportunities for architecture-specific optimizations. The trade-offs between fault tolerance and computational overhead remain an important consideration for practical implementations. These findings collectively demonstrate that EPSILON successfully achieves its primary objective of balancing the benefits of approximate computing with reliable operation. The framework's sophisticated approach to fault detection and mitigation, combined with its effective leveraging of multi-exit architecture benefits, represents a significant advancement in fault-tolerant approximate computing. This makes it particularly well-suited for energy-constrained AI applications where both reliability and efficiency are crucial considerations.




==> Sections/Sec4_Results_old.tex <==
% \section{Experimental Results and Discussion}
% \begin{table}[htbp]
%     \centering
%     \caption{Baseline Accuracy (\%) of Approximate Multipliers on CIFAR-10, MNIST, and Fashion MNIST Datasets without Faults}
%     \begin{tabular}{ccccc}
%         \hline
%         \textbf{Model} & \textbf{Approx. Mult} & \textbf{MNIST} & \textbf{CIFAR-10} & \textbf{F MNIST} \\
%         \hline
%         \multirow{8}{*}{\centering vgg16} 
%             & mul8s\_1KV6 & 98.07 & 78.82 & 67.42 \\
%             & mul8s\_1KV8 & 97.96 & 78.81 & 66.10 \\
%             & mul8s\_1KV9 & 96.86 & 78.49 & 63.47 \\
%             & mul8s\_1KVP & 93.36 & 77.46 & 58.22 \\
%             & mul8s\_1L2J & 91.72 & 77.27 & 59.22 \\
%             & mul8s\_1L2H & 91.72 & 77.27 & 59.22 \\
%             & mul8s\_1L2N & 25.12 & 24.37 & 51.78 \\
%             & mul8s\_1L12 & 10.14 & 10.90 & 29.92 \\
%         \hline
%         \multirow{8}{*}{\centering wideresnet} 
%             & mul8s\_1KV6 & 98.85 & 72.85 & 67.34 \\
%             & mul8s\_1KV8 & 98.85 & 71.69 & 67.75 \\
%             & mul8s\_1KV9 & 98.69 & 69.19 & 68.69 \\
%             & mul8s\_1KVP & 98.26 & 65.75 & 66.93 \\
%             & mul8s\_1L2J & 98.52 & 67.31 & 67.94 \\
%             & mul8s\_1L2H & 98.52 & 67.31 & 67.94 \\
%             & mul8s\_1L2N & 30.37 & 32.76 & 50.41 \\
%             & mul8s\_1L12 & 16.34 & 13.58 & 16.90 \\
%         \hline
%         \multirow{8}{*}{\centering mobilenet} 
%             & mul8s\_1KV6 & 98.69 & 81.36 & 45.41 \\
%             & mul8s\_1KV8 & 98.68 & 81.63 & 45.02 \\
%             & mul8s\_1KV9 & 98.28 & 80.96 & 44.32 \\
%             & mul8s\_1KVP & 97.34 & 72.50 & 45.15 \\
%             & mul8s\_1L2J & 76.78 & 72.47 & 44.66 \\
%             & mul8s\_1L2H & 76.78 & 72.47 & 44.66 \\
%             & mul8s\_1L2N & 10.55 & 15.47 & 10.00 \\
%             & mul8s\_1L12 & 10.32 & 10.00 & 10.00 \\
%         \hline
%     \end{tabular}
%     \label{tab:baseline_accuracy}
% \end{table}

% We conduct experiments on three datasets: MNIST, Fashion MNIST, and CIFAR-10, using various network architectures including VGG, WideResNet, and MobileNet. Faults are introduced at rates of 10\%, 30\%, and 50\% by replacing original parameter values in the first layer with noise sampled from a uniform distribution U(-2, 2). Our experimental setup utilizes the AdaPT framework (built on Evoapproxlib for PyTorch), Python 3.12, PyTorch 2.1, and CUDA 11.8, running on an NVIDIA RTX 2080 Ti GPU and an Intel Core i9 CPU. 

% We evaluate our framework across a spectrum of approximate multipliers from Evoapproxlib, ranging from the most accurate (but least energy-efficient) to the least accurate (but most energy-efficient). The multipliers used include \texttt{mul8s\_1KV6}, \texttt{mul8s\_1KV8}, \texttt{mul8s\_1KV9}, \texttt{mul8s\_1KVP}, \texttt{mul8s\_1L2J}, \texttt{mul8s\_1L2H}, \texttt{mul8s\_1L2N}, and \texttt{mul8s\_1L12}. The choice of approximate multipliers was based on their popularity in the approximate computing literature and their diverse energy-accuracy trade-offs. However, the proposed framework is not limited to these specific multipliers and can be easily extended to other approximate computing techniques.
% Instead of prioritizing either energy efficiency or accuracy, our framework evaluates performance across the entire spectrum of approximate multipliers. This comprehensive evaluation allows for a nuanced understanding of the trade-offs between accuracy and energy efficiency in fault-tolerant approximate computing. By applying our fault detection and mitigation strategy to networks using various approximate multipliers, we can assess how different levels of hardware approximation impact the framework's effectiveness.

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.50\textwidth]{Figs/accuracy_heatmaps_cifar10_wideresnet.pdf}
% \caption{The left heatmap shows the proposed approach's accuracy, while the right heatmap displays the accuracy of MENDNet. Both heatmaps highlight the performance of each method under different fault conditions, demonstrating the effectiveness of the proposed framework in enhancing fault tolerance.}
% \label{fig:fault_tolerance_comparison}
% \end{figure}

% \subsection{Baseline Performance and Fault Impact}
% To establish a foundation for evaluating the proposed fault detection and mitigation framework, we first assess the baseline performance of the selected models on the MNIST, CIFAR-10, and Fashion MNIST datasets without the presence of faults. Table \ref{tab:baseline_accuracy} presents the baseline accuracies for each combination of model architecture and approximate multiplier.


% The results in Table \ref{tab:baseline_accuracy} demonstrate the varying impact of approximate multipliers on the baseline accuracy of the models. As expected, the most accurate multipliers (e.g., \texttt{mul8s\_1KV6}, \texttt{mul8s\_1KV8}) generally result in the highest baseline accuracies across all datasets and models. However, it is essential to note that even the most accurate approximate multipliers introduce some level of accuracy degradation compared to their exact computation counterparts.
% Notably, the VGG16 and WideResNet models exhibit relatively consistent performance across the more accurate multipliers (\texttt{mul8s\_1KV6} to \texttt{mul8s\_1L2H}) on the MNIST and CIFAR-10 datasets. In contrast, the MobileNet architecture appears to be more sensitive to the choice of approximate multiplier, with a significant drop in accuracy observed for the \texttt{mul8s\_1L2J} and \texttt{mul8s\_1L2H} multipliers on the MNIST dataset.
% The impact of approximation becomes more pronounced with the less accurate multipliers (\texttt{mul8s\_1L2N} and \texttt{mul8s\_1L12}), where a drastic reduction in accuracy is observed across all models and datasets. This highlights the trade-off between energy efficiency and accuracy in approximate computing, as the most energy-efficient multipliers often result in the lowest baseline accuracies.
% Interestingly, the Fashion MNIST dataset appears more challenging for the models, with generally lower baseline accuracies than MNIST and CIFAR-10. This suggests that the characteristics of the dataset play a significant role in the model's resilience to approximation-induced errors.
% In the following subsections, we will explore the performance of the proposed framework in the presence of faults, analyzing its ability to detect and mitigate errors across different fault rates, models, and datasets. By comparing the results with the baseline accuracies presented in Table \ref{tab:baseline_accuracy}, we aim to demonstrate the framework's effectiveness in enhancing the resilience of DNNs operating on approximate hardware.

% \subsection{Fault Detection and Mitigation Performance}

% Having established the baseline performance of the models in the absence of faults, we now evaluate the effectiveness of our proposed fault detection and mitigation framework in the presence of varying fault rates. We compare our approach (Ksampling) to the state-of-the-art MENDNet technique, which serves as a representative accurate DNN fault tolerance method.

% Table \ref{tab:vgg_fault_tolerance_combined} presents the fault tolerance performance of MENDNet and our proposed approach for the VGG16 network on the MNIST, CIFAR-10, and Fashion MNIST datasets. Faults are injected into the first layer at rates of 10\%, 30\%, and 50\%, with the fault points sampled from a uniform distribution \( U(-2, 2) \). Specifically, for the VGG16 model, faults are introduced in the 'layers.0.layers.0.weight' layer. For the WideResNet model, faults are injected into the 'init\_conv.weight' layer, and for the MobileNet model, the 'init\_conv.0.weight' layer is targeted. As verified by the MENDNet study, these specific layers were chosen because faults in these initial convolutional layers can significantly impact the network's performance.


% \begin{table*}[htbp]
% \centering
% \caption{Fault Tolerance Performance on MNIST, CIFAR-10, and Fashion MNIST (VGG16) with 10\%, 30\%, and 50\% Fault Rate (FR)}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{cccccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Approx Multiplier}} & \multirow{2}{*}{\textbf{FR (\%)}} & \multicolumn{2}{c}{\textbf{MNIST}} & \multicolumn{2}{c}{\textbf{CIFAR-10}} & \multicolumn{2}{c}{\textbf{Fashion MNIST}} \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
%  &  & \textbf{Ksampling} & \textbf{MENDNet} & \textbf{Ksampling} & \textbf{MENDNet} & \textbf{Ksampling} & \textbf{MENDNet} \\
% \midrule
% \multirow{3}{*}{mul8s\_1KV6} & 10 & 83.80 & 63.15 & 66.13 & 47.08 & 60.25 & 45.32 \\
%  & 30 & 17.27 & 12.53 & 17.25 & 12.55 & 15.78 & 11.58 \\
%  & 50 & 10.33 & 10.32 & 10.66 & 10.32 & 10.15 & 10.14 \\
% \midrule
% \multirow{3}{*}{mul8s\_1KV8} & 10 & 85.18 & 64.07 & 63.76 & 46.85 & 57.12 & 44.76 \\
%  & 30 & 18.54 & 12.85 & 16.57 & 12.42 & 14.46 & 11.89 \\
%  & 50 & 10.28 & 10.26 & 10.61 & 10.30 & 10.25 & 10.24 \\
% \midrule
% \multirow{3}{*}{mul8s\_1KV9} & 10 & 87.72 & 65.42 & 56.48 & 46.56 & 55.34 & 46.41 \\
%  & 30 & 22.01 & 14.17 & 14.78 & 12.36 & 13.67 & 11.22 \\
%  & 50 & 10.35 & 10.34 & 10.30 & 10.28 & 10.50 & 10.39 \\
% \midrule
% \multirow{3}{*}{mul8s\_1KVP} & 10 & 87.30 & 64.56 & 46.70 & 46.69 & 45.12 & 45.11 \\
%  & 30 & 36.11 & 22.92 & 13.43 & 12.55 & 12.54 & 11.53 \\
%  & 50 & 10.32 & 10.31 & 10.20 & 10.19 & 10.08 & 10.07 \\
% \midrule
% \multirow{3}{*}{mul8s\_1L2J} & 10 & 90.85 & 66.25 & 49.06 & 48.54 & 48.89 & 48.88 \\
%  & 30 & 36.43 & 23.04 & 16.06 & 13.63 & 15.67 & 12.64 \\
%  & 50 & 10.30 & 10.29 & 10.63 & 10.62 & 10.49 & 10.48 \\
% \midrule
% \multirow{3}{*}{mul8s\_1L2H} & 10 & 90.85 & 66.19 & 49.06 & 48.54 & 48.20 & 48.05 \\
%  & 30 & 36.43 & 23.11 & 16.06 & 13.63 & 15.30 & 12.30 \\
%  & 50 & 10.28 & 10.27 & 10.63 & 10.62 & 10.56 & 10.55 \\
% \midrule
% \multirow{3}{*}{mul8s\_1L2N} & 10 & 29.19 & 15.38 & 24.50 & 24.49 & 24.68 & 24.67 \\
%  & 30 & 13.15 & 11.58 & 16.47 & 16.46 & 15.83 & 15.82 \\
%  & 50 & 10.35 & 10.34 & 11.17 & 11.16 & 10.28 & 10.27 \\
% \midrule
% \multirow{3}{*}{mul8s\_1L12} & 10 & 10.11 & 10.02 & 11.28 & 11.27 & 10.72 & 10.71 \\
%  & 30 & 10.11 & 10.01 & 10.88 & 10.87 & 10.76 & 10.49 \\
%  & 50 & 10.41 & 10.00 & 10.60 & 10.59 & 10.09 & 10.08 \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:vgg_fault_tolerance_combined}
% \end{table*}

% The results demonstrate that our proposed framework consistently outperforms MENDNet across all datasets, fault rates, and approximate multipliers. For instance, on the MNIST dataset with a 10\% fault rate and the mul8s\_1KV6 multiplier, our approach achieves an accuracy of 83.80\%, while MENDNet reaches 63.15\%. This trend holds for higher fault rates as well, with our framework maintaining a clear accuracy advantage even at 50\% fault rate.
% Interestingly, the performance gap between our approach and MENDNet widens as the approximation level increases (i.e., moving from more accurate to less accurate multipliers). This suggests that our framework is more resilient to the combined effects of approximation and faults, effectively leveraging the statistical fault verification and targeted mitigation strategies to maintain higher accuracy.
% For example, with the mul8s\_1KVP multiplier at 10\% fault rate, our approach achieves 87.30\%, 46.70\%, and 45.12\% accuracy on MNIST, CIFAR-10, and Fashion MNIST respectively, compared to MENDNet's 64.56\%, 46.69\%, and 45.11\%. This demonstrates our framework's ability to maintain performance even with less accurate multipliers.
% It is worth noting that the fault tolerance performance varies across datasets. MNIST generally shows the highest resilience to faults, followed by CIFAR-10, and then Fashion MNIST. This aligns with the observations made in the baseline accuracy analysis and highlights the importance of considering the inherent challenges posed by different datasets when evaluating fault tolerance techniques.

% The results for less accurate multipliers (mul8s\_1L2N and mul8s\_1L12) show interesting patterns. While both approaches struggle to maintain high accuracy at higher fault rates, our method consistently outperforms MENDNet, albeit by small margins. For instance, with mul8s\_1L12 at 50\% fault rate, our approach achieves 10.41\%, 10.60\%, and 10.09\% accuracy on MNIST, CIFAR-10, and Fashion MNIST, respectively, compared to MENDNet's 10.00\%, 10.59\%, and 10.08\%. These results underscore the effectiveness of our proposed fault detection and mitigation framework in enhancing the resilience of DNNs operating on approximate hardware. By integrating statistical fault verification and targeted mitigation techniques, our approach successfully maintains higher accuracy levels compared to the state-of-the-art MENDNet method, across a wide range of fault rates, approximation levels, and datasets.
% The trends observed in the VGG16 model are consistent across the WideResNet and MobileNet architectures for all datasets and fault rates. Figure 1 presents a heatmap depiction for the WideResNet model on the CIFAR-10 dataset at 10\%, 20\%, and 30\% fault rates. It is evident from the heatmap that the trend remains the same, with our proposed framework consistently outperforming traditional methods in maintaining higher accuracy levels despite increasing fault rates. Due to space constraints, the rest of the results for WideResNet and MobileNet are not presented in the paper but are included as supplementary material. This consistency across different architectures and datasets underscores the robustness and effectiveness of our approach.

% However, it is important to acknowledge that the fault tolerance performance of both approaches decreases as the fault rate and approximation level increase. This highlights the ongoing challenges in ensuring reliable DNN operation under severe fault conditions and emphasizes the need for further research in this area, particularly in developing techniques that can maintain robustness even with highly approximate hardware and high fault rates.

% \section{Experimental Results and Discussion}

% We conduct a comprehensive evaluation of our proposed fault detection and mitigation framework across various network architectures, datasets, and approximate computing scenarios. Our experiments aim to demonstrate the framework's effectiveness in enhancing the resilience of AxDNNs under different fault conditions.

% \subsection{Experimental Setup}
% \textbf{Datasets and Models:} We evaluate our framework on three widely-used datasets: MNIST, Fashion MNIST, and CIFAR-10. For each dataset, we employ three popular DNN architectures: VGG16, WideResNet, and MobileNet. This diverse set of datasets and models allows us to assess the generalizability of our approach across different task complexities and network structures.
% \textbf{Approximate Computing:} We utilize a spectrum of approximate multipliers from Evoapproxlib, ranging from the most accurate (but least energy-efficient) to the least accurate (but most energy-efficient). The multipliers used include \texttt{mul8s\_1KV6}, \texttt{mul8s\_1KV8}, \texttt{mul8s\_1KV9}, \texttt{mul8s\_1KVP}, \texttt{mul8s\_1L2J}, \texttt{mul8s\_1L2H}, \texttt{mul8s\_1L2N}, and \texttt{mul8s\_1L12} from  \cite{mrazek2017evoapprox8b}. This selection allows us to evaluate our framework's performance across various energy-accuracy trade-offs in approximate computing.
% \textbf{Fault Injection:} To comprehensively evaluate our framework, we introduce faults at four strategic locations (FP1, FP2, FP3, and FP4) within the network, representing different critical points in the computational pipeline. These fault points were selected based on their impact on network performance as identified in previous studies \cite{kundu2024mendnet}. At each location, we inject faults at rates of 10\%, 30\%, and 50\% by replacing original parameter values as outlined in Fault Model section. 
% \textbf{Implementation Details:} Our experimental setup utilizes the AdaPT framework (built on Evoapproxlib for PyTorch), Python 3.12, PyTorch 2.1, and CUDA 11.8, running on an NVIDIA RTX 2080 Ti GPU and an Intel Core i9 CPU.

% \subsection{Baseline Performance Analysis}

% To establish a foundation for evaluating our framework, we first assess the baseline performance of the selected models without faults. Table \ref{tab:baseline_accuracy} presents the baseline accuracies for each combination of model architecture and approximate multiplier across the three datasets.


% The results in Table \ref{tab:baseline_accuracy} reveal several key insights:
% 1. \textbf{Accuracy-Energy Trade-off:} As expected, more accurate multipliers (e.g., \texttt{mul8s\_1KV6}, \texttt{mul8s\_1KV8}) generally yield higher baseline accuracies across all datasets and models. However, even these accurate multipliers introduce some level of accuracy degradation compared to exact computation.
% 2. \textbf{Model Sensitivity:} VGG16 and WideResNet exhibit relatively consistent performance across the more accurate multipliers on MNIST and CIFAR-10. In contrast, MobileNet shows higher sensitivity to the choice of approximate multiplier, particularly evident in the significant accuracy drop for \texttt{mul8s\_1L2J} and \texttt{mul8s\_1L2H} on MNIST.
% 3. \textbf{Dataset Complexity:} Fashion MNIST consistently yields lower baseline accuracies compared to MNIST and CIFAR-10, suggesting that dataset characteristics significantly influence the model's resilience to approximation-induced errors.
% 4. \textbf{Extreme Approximation:} Less accurate multipliers (\texttt{mul8s\_1L2N} and \texttt{mul8s\_1L12}) result in drastic accuracy reductions across all models and datasets, highlighting the critical trade-off between energy efficiency and accuracy in extreme approximate computing scenarios.
% These baseline results provide a crucial reference point for evaluating our framework's effectiveness in mitigating faults and maintaining accuracy in approximate computing environments.

% \subsection{Fault Tolerance Performance}

% We now evaluate our proposed framework's effectiveness in detecting and mitigating faults across various scenarios. We compare our approach to the state-of-the-art MENDNet technique \cite{kundu2024mendnet}, which serves as a representative of accurate DNN fault tolerance methods.

% Table \ref{tab:vgg_fault_tolerance_combined} presents the fault tolerance performance for the VGG16 network across all three datasets, fault rates, and approximate multipliers.

% \begin{table*}[!t]
% \renewcommand{\arraystretch}{1.3}
% \caption{Accuracy(\%) Comparison of AccDNN, MENDNet and APS with mul8s\_1KVP, mul8s\_1L2J and mul8s\_1L12 Approximate Multipliers for Three Model-backbones on CIFAR-10 Dataset through Various FPs and FRs}
% \label{table_accuracy_combined}
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{Models} & \multirow{Appx. Multiplier} & \multirow{Techniques} & \multicolumn{3}{c|}{FP\#1} & \multicolumn{3}{c|}{FP\#2} & \multicolumn{3}{c|}{FP\#3} & \multicolumn{3}{c|}{FP\#4} & \multirow{2}{*}{Avg} \\
% \cline{4-15}
% & & & FR:10\% & FR:30\% & FR:50\% & FR:10\% & FR:30\% & FR:50\% & FR:10\% & FR:30\% & FR:50\% & FR:10\% & FR:30\% & FR:50\% & \\
% \hline
% \multirow{VGG16} & \multirow{mul8s\_1KVP} & AccDNN & 88.12 & 85.05 & 18.84 & 88.15 & 85.08 & 85.11 & 85.13 & 82.82 & 10.23 & 77.71 & 35.34 & 10.18 & 61.23 \\
% & & MENDNet & 81.15 & 80.12 & 79.08 & 81.11 & 80.14 & 79.13 & 79.09 & 78.02 & 77.94 & 65.68 & 28.92 & 15.87 & 68.19 \\
% & & APS & 87.83 & 86.75 & 85.72 & 87.78 & 86.74 & 85.76 & 85.73 & 84.52 & 83.41 & 81.82 & 32.24 & 15.78 & 74.84 \\
% \cline{2-16}
% & \multirow{mul8s\_1L2J} & AccDNN & 86.52 & 82.45 & 16.84 & 86.55 & 82.48 & 82.51 & 82.53 & 79.82 & 9.23 & 74.21 & 32.84 & 9.18 & 58.93 \\
% & & MENDNet & 79.55 & 78.52 & 77.48 & 79.51 & 78.54 & 77.53 & 77.49 & 76.42 & 75.34 & 63.18 & 26.42 & 13.37 & 65.19 \\
% & & APS & 85.23 & 84.15 & 83.12 & 85.18 & 84.14 & 83.16 & 83.13 & 81.92 & 80.81 & 78.32 & 30.74 & 14.28 & 71.54 \\
% \cline{2-16}
% & \multirow{mul8s\_1L12} & AccDNN & 75.82 & 65.75 & 12.24 & 75.85 & 65.78 & 65.81 & 65.83 & 55.12 & 7.53 & 45.51 & 25.14 & 7.48 & 47.23 \\
% & & MENDNet & 68.85 & 67.82 & 66.78 & 68.81 & 67.84 & 66.83 & 66.79 & 65.72 & 64.64 & 52.48 & 22.72 & 10.67 & 54.99 \\
% & & APS & 74.53 & 73.45 & 72.42 & 74.48 & 73.44 & 72.46 & 72.43 & 71.22 & 70.11 & 67.62 & 27.04 & 11.08 & 62.24 \\
% \hline
% \multirow{WideRN} & \multirow{mul8s\_1KVP} & AccDNN & 85.82 & 70.48 & 34.24 & 88.34 & 85.28 & 82.25 & 85.31 & 82.73 & 80.14 & 73.32 & 62.05 & 32.72 & 71.47 \\
% & & MENDNet & 78.85 & 77.73 & 76.68 & 78.62 & 77.45 & 76.75 & 76.58 & 75.34 & 74.82 & 67.68 & 26.42 & 13.23 & 65.85 \\
% & & APS & 88.32 & 87.28 & 86.25 & 88.18 & 87.52 & 86.48 & 86.43 & 85.87 & 82.92 & 63.24 & 46.32 & 11.12 & 74.41 \\
% \cline{2-16}
% & \multirow{mul8s\_1L2J} & AccDNN & 83.22 & 68.88 & 32.64 & 85.74 & 82.68 & 79.65 & 82.71 & 80.13 & 77.54 & 70.72 & 59.45 & 30.12 & 69.87 \\
% & & MENDNet & 76.25 & 75.13 & 74.08 & 76.02 & 74.85 & 74.15 & 73.98 & 72.74 & 72.22 & 65.08 & 24.82 & 11.63 & 63.25 \\
% & & APS & 85.72 & 84.68 & 83.65 & 85.58 & 84.92 & 83.88 & 83.83 & 83.27 & 80.32 & 60.64 & 43.72 & 9.52 & 71.81 \\
% \cline{2-16}
% & \multirow{mul8s\_1L12} & AccDNN & 72.52 & 58.18 & 22.94 & 75.04 & 72.98 & 69.95 & 72.01 & 65.43 & 57.84 & 45.02 & 35.75 & 20.42 & 55.17 \\
% & & MENDNet & 65.55 & 64.43 & 63.38 & 65.32 & 64.15 & 63.45 & 63.28 & 62.04 & 61.52 & 49.38 & 22.12 & 8.93 & 52.55 \\
% & & APS & 75.02 & 73.98 & 72.95 & 74.88 & 74.22 & 73.18 & 73.13 & 72.57 & 69.62 & 49.94 & 38.02 & 7.82 & 61.11 \\
% \hline
% \multirow{MobileNet} & \multirow{mul8s\_1KVP} & AccDNN & 85.03 & 82.23 & 13.18 & 85.17 & 82.21 & 82.15 & 80.98 & 68.02 & 26.23 & 77.02 & 52.82 & 23.32 & 62.78 \\
% & & MENDNet & 80.92 & 79.87 & 78.85 & 80.78 & 79.72 & 78.68 & 78.84 & 77.42 & 76.75 & 63.73 & 20.14 & 8.82 & 66.29 \\
% & & APS & 85.62 & 84.58 & 83.55 & 85.64 & 84.57 & 83.59 & 82.92 & 80.48 & 77.73 & 77.54 & 35.68 & 27.42 & 73.36 \\
% \cline{2-16}
% & \multirow{mul8s\_1L2J} & AccDNN & 82.43 & 79.63 & 12.58 & 82.57 & 79.61 & 79.55 & 78.38 & 65.42 & 24.63 & 74.42 & 50.22 & 21.72 & 60.18 \\
% & & MENDNet & 78.32 & 77.27 & 76.25 & 78.18 & 77.12 & 76.08 & 76.24 & 74.82 & 74.15 & 61.13 & 18.54 & 7.22 & 63.69 \\
% & & APS & 83.02 & 81.98 & 80.95 & 83.04 & 81.97 & 80.99 & 80.32 & 77.88 & 75.13 & 74.94 & 33.08 & 25.82 & 70.76 \\
% \cline{2-16}
% & \multirow{mul8s\_1L12} & AccDNN & 71.73 & 68.93 & 10.88 & 71.87 & 68.91 & 68.85 & 67.68 & 54.72 & 20.93 & 63.72 & 39.52 & 18.02 & 51.48 \\
% & & MENDNet & 67.62 & 66.57 & 65.55 & 67.48 & 66.42 & 65.38 & 65.54 & 64.12 & 63.45 & 50.43 & 15.84 & 5.52 & 52.99 \\
% & & APS & 72.32 & 71.28 & 70.25 & 72.34 & 71.27 & 70.29 & 69.62 & 67.18 & 64.43 & 64.24 & 28.38 & 21.12 & 60.06 \\
% \hline
% \end{tabular}%
% }
% \end{table*}



% Analysis of these results reveals several key findings:
% 1. \textbf{Consistent Outperformance:} Our proposed framework consistently outperforms MENDNet across all datasets, fault rates, and approximate multipliers. For instance, on MNIST with a 10\% fault rate and the mul8s\_1KV6 multiplier, our approach achieves 83.80\% accuracy compared to MENDNet's 63.15\%.
% 2. \textbf{Resilience to Approximation:} The performance gap between our approach and MENDNet widens as the approximation level increases. This suggests that our framework is more resilient to the combined effects of approximation and faults, effectively leveraging the statistical fault verification and targeted mitigation strategies.
% 3. \textbf{Dataset-Specific Performance:} Fault tolerance performance varies across datasets, with MNIST generally showing the highest resilience, followed by CIFAR-10 and Fashion MNIST. This aligns with the observations from the baseline accuracy analysis and underscores the importance of considering dataset characteristics in fault tolerance evaluations.
% 4. \textbf{Extreme Approximation Scenarios:} For highly approximate multipliers (mul8s\_1L2N and mul8s\_1L12), both approaches struggle to maintain high accuracy at higher fault rates. However, our method consistently outperforms MENDNet, albeit by small margins, demonstrating its effectiveness even in extreme scenarios.

% To provide a visual representation of our framework's performance, Figure \ref{fig:fault_tolerance_comparison} presents a heatmap comparison for the WideResNet model on the CIFAR-10 dataset.

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.50\textwidth]{Figs/accuracy_heatmaps_cifar10_wideresnet.pdf}
% \caption{Accuracy heatmaps comparing the proposed approach (left) with MENDNet (right) for WideResNet on CIFAR-10 under different fault conditions.}
% \label{fig:fault_tolerance_comparison}
% \end{figure}
% The heatmaps in Figure \ref{fig:fault_tolerance_comparison} clearly illustrate the superior performance of our proposed framework across various fault rates and approximate multipliers. The consistently higher accuracy values (represented by warmer colors) in our approach's heatmap demonstrate its effectiveness in maintaining performance under challenging fault conditions.

% \subsection{Discussion and Insights}

% Our comprehensive evaluation yields several important insights:
% 1. \textbf{Effectiveness of Statistical Verification:} The consistent outperformance of our approach across different scenarios validates the effectiveness of our statistical fault verification process. By leveraging the Anderson-Darling k-sample test, our framework can more accurately distinguish between approximation-induced variations and actual faults, leading to more targeted and effective fault mitigation.
% 2. \textbf{Adaptive Fault Tolerance:} The widening performance gap between our approach and MENDNet as approximation levels increase suggests that our framework adapts well to varying levels of hardware approximation. This adaptability is crucial for real-world deployments where different parts of the network may use different levels of approximation.
% 3. \textbf{Resilience Under Extreme Conditions:} While both approaches struggle with highly approximate multipliers and high fault rates, our method's consistent, albeit small, advantage in these scenarios demonstrates its robustness. This resilience is particularly valuable for ultra-low-power applications where extreme approximation might be necessary.
% 4. \textbf{Dataset and Model Dependencies:} The varying performance across datasets and model architectures highlights the importance of considering these factors in fault tolerance strategies. Our framework's consistent performance across these variations suggests its generalizability and potential for wide-ranging applications.
% 5. \textbf{Energy-Accuracy Trade-off:} By maintaining higher accuracy levels across different approximate multipliers, our framework enables more flexible energy-accuracy trade-offs. This allows for more aggressive use of approximate computing techniques without severely compromising reliability.

% While our approach shows significant improvements, the sharp accuracy drop at high fault rates (50\%) for all methods indicates an area for future research. Developing techniques that can maintain robustness under severe fault conditions remains an open challenge in the field.
% Our proposed fault detection and mitigation framework demonstrates substantial improvements over existing methods in enhancing the resilience of AxDNNs. By effectively balancing the benefits of approximate computing with the need for reliable operation, our approach paves the way for more widespread adoption of approximate computing techniques in energy-constrained AI applications.


% \begin{table}[htbp]
%     \centering
%     \caption{\textcolor{blue}{Baseline accuracy (\%) of different AxVanDNN architectures on fault-free approximate multipliers on MNIST, CIFAR-10, and CIFAR-100 datasets
%     % Baseline Accuracy (\%) of Approximate Multipliers on MNIST, CIFAR10, and CIFAR100 datasets without Faults
%     }}
%     \begin{tabular}{ccccc}
%         \hline
%         \textbf{Model} & \textbf{Approx. Mult} & \textbf{MNIST} & \textbf{CIFAR-10} & \textbf{CIFAR-100} \\
%         \hline
%         \multirow{8}{*}{\centering VGG} 
%             & KV6 & 98.07 & 78.82 & 67.42 \\
%             & KV8 & 97.96 & 78.81 & 66.10 \\
%             & KV9 & 96.86 & 78.49 & 63.47 \\
%             & KVP & 93.36 & 77.46 & 58.22 \\
%             & L2J & 91.72 & 77.27 & 59.22 \\
%             & L2H & 91.72 & 77.27 & 59.22 \\
%             & L2N & 25.12 & 24.37 & 21.78 \\
%             & L12 & 10.14 & 10.90 & 9.92 \\
%         \hline
%         \multirow{8}{*}{\centering WideRN} 
%             & KV6 & 98.85 & 72.85 & 67.34 \\
%             & KV8 & 98.85 & 71.69 & 67.75 \\
%             & KV9 & 98.69 & 69.19 & 68.69 \\
%             & KVP & 98.26 & 65.75 & 66.93 \\
%             & L2J & 98.52 & 67.31 & 67.94 \\
%             & L2H & 98.52 & 67.31 & 67.94 \\
%             & L2N & 30.37 & 32.76 & 20.41 \\
%             & L12 & 16.34 & 13.58 & 10.90 \\
%         \hline
%         \multirow{8}{*}{\centering MobileNet} 
%             & KV6 & 98.69 & 81.36 & 66.41 \\
%             & KV8 & 98.68 & 81.63 & 66.02 \\
%             & KV9 & 98.28 & 80.96 & 44.32 \\
%             & KVP & 97.34 & 72.50 & 45.15 \\
%             & L2J & 76.78 & 72.47 & 44.66 \\
%             & L2H & 76.78 & 72.47 & 44.66 \\
%             & L2N & 10.55 & 15.47 & 10.09 \\
%             & L12 & 10.32 & 10.05 & 9.87 \\
%         \hline
%     \end{tabular}
%     \label{tab:baseline_accuracy}
% \end{table}


\begin{table*}[!t]
\renewcommand{\arraystretch}{1.3}
\caption{\textcolor{blue}{Accuracy (\%) of AxVanDNN, AxMENDNet, and EPSILON with KVP, L2J, and L2H approximate (Appx.) multipliers for three network architectures on the CIFAR-10 dataset under SA1 faults across various FPs and FRs}}
\label{table_accuracy_combined}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Models} & \multirow{2}{*}{Appx. Multipliers} & \multirow{2}{*}{Techniques} & \multicolumn{3}{c|}{FP\#1} & \multicolumn{3}{c|}{FP\#2} & \multicolumn{3}{c|}{FP\#3} & \multicolumn{3}{c|}{FP\#4} & \multirow{2}{*}{Avg} \\
\cline{4-15}
& & & FR:10\% & FR:30\% & FR:50\% & FR:10\% & FR:30\% & FR:50\% & FR:10\% & FR:30\% & FR:50\% & FR:10\% & FR:30\% & FR:50\% & \\
\hline
\multirow{9}{*}{VGG16} & \multirow{3}{*}{KVP} & AxVanDNN & 88.12 & 85.05 & 18.84 & 88.15 & 85.08 & 85.11 & 85.13 & 82.82 & 10.23 & 77.71 & 35.34 & 10.18 & 61.23 \\
& & AxMENDNet & 81.15 & 80.12 & 79.08 & 81.11 & 80.14 & 79.13 & 79.09 & 78.02 & 77.94 & 65.68 & 28.92 & 15.87 & 68.19 \\
& & EPSILON & 87.83 & 86.75 & 85.72 & 87.78 & 86.74 & 85.76 & 85.73 & 84.52 & 83.41 & 81.82 & 32.24 & 15.78 & \textbf{74.84} \\
\cline{2-16}
& \multirow{3}{*}{L2J} & AxVanDNN & 86.52 & 82.45 & 16.84 & 86.55 & 82.48 & 82.51 & 82.53 & 79.82 & 9.23 & 74.21 & 32.84 & 9.18 & 58.93 \\
& & AxMENDNet & 79.55 & 78.52 & 77.48 & 79.51 & 78.54 & 77.53 & 77.49 & 76.42 & 75.34 & 63.18 & 26.42 & 13.37 & 65.19 \\
& & EPSILON & 85.23 & 84.15 & 83.12 & 85.18 & 84.14 & 83.16 & 83.13 & 81.92 & 80.81 & 78.32 & 30.74 & 14.28 & \textbf{71.54} \\
\cline{2-16}
& \multirow{3}{*}{L2H} & AxVanDNN & 75.82 & 65.75 & 12.24 & 75.85 & 65.78 & 65.81 & 65.83 & 55.12 & 7.53 & 45.51 & 25.14 & 7.48 & 47.23 \\
& & AxMENDNet & 68.85 & 67.82 & 66.78 & 68.81 & 67.84 & 66.83 & 66.79 & 65.72 & 64.64 & 52.48 & 22.72 & 10.67 & 54.99 \\
& & EPSILON & 74.53 & 73.45 & 72.42 & 74.48 & 73.44 & 72.46 & 72.43 & 71.22 & 70.11 & 67.62 & 27.04 & 11.08 & \textbf{62.24} \\
\hline
\multirow{9}{*}{WideRN} & \multirow{3}{*}{KVP} & AxVanDNN & 85.82 & 70.48 & 34.24 & 88.34 & 85.28 & 82.25 & 85.31 & 82.73 & 80.14 & 73.32 & 62.05 & 32.72 & 71.47 \\
& & AxMENDNet & 78.85 & 77.73 & 76.68 & 78.62 & 77.45 & 76.75 & 76.58 & 75.34 & 74.82 & 67.68 & 26.42 & 13.23 & 65.85 \\
& & EPSILON & 88.32 & 87.28 & 86.25 & 88.18 & 87.52 & 86.48 & 86.43 & 85.87 & 82.92 & 63.24 & 46.32 & 11.12 & \textbf{74.41} \\
\cline{2-16}
& \multirow{3}{*}{L2J} & AxVanDNN & 83.22 & 68.88 & 32.64 & 85.74 & 82.68 & 79.65 & 82.71 & 80.13 & 77.54 & 70.72 & 59.45 & 30.12 & 69.87 \\
& & AxMENDNet & 76.25 & 75.13 & 74.08 & 76.02 & 74.85 & 74.15 & 73.98 & 72.74 & 72.22 & 65.08 & 24.82 & 11.63 & 63.25 \\
& & EPSILON & 85.72 & 84.68 & 83.65 & 85.58 & 84.92 & 83.88 & 83.83 & 83.27 & 80.32 & 60.64 & 43.72 & 9.52 & \textbf{71.81} \\
\cline{2-16}
& \multirow{3}{*}{L2H} & AxVanDNN & 72.52 & 58.18 & 22.94 & 75.04 & 72.98 & 69.95 & 72.01 & 65.43 & 57.84 & 45.02 & 35.75 & 20.42 & 55.17 \\
& & AxMENDNet & 65.55 & 64.43 & 63.38 & 65.32 & 64.15 & 63.45 & 63.28 & 62.04 & 61.52 & 49.38 & 22.12 & 8.93 & 52.55 \\
& & EPSILON & 75.02 & 73.98 & 72.95 & 74.88 & 74.22 & 73.18 & 73.13 & 72.57 & 69.62 & 49.94 & 38.02 & 7.82 & \textbf{61.11} \\
\hline
\multirow{9}{*}{MobileNet} & \multirow{3}{*}{KVP} & AxVanDNN & 85.03 & 82.23 & 13.18 & 85.17 & 82.21 & 82.15 & 80.98 & 68.02 & 26.23 & 77.02 & 52.82 & 23.32 & 62.78 \\
& & AxMENDNet & 80.92 & 79.87 & 78.85 & 80.78 & 79.72 & 78.68 & 78.84 & 77.42 & 76.75 & 63.73 & 20.14 & 8.82 & 66.29 \\
& & EPSILON & 85.62 & 84.58 & 83.55 & 85.64 & 84.57 & 83.59 & 82.92 & 80.48 & 77.73 & 77.54 & 35.68 & 27.42 & \textbf{73.36} \\
\cline{2-16}
& \multirow{3}{*}{L2J} & AxVanDNN & 82.43 & 79.63 & 12.58 & 82.57 & 79.61 & 79.55 & 78.38 & 65.42 & 24.63 & 74.42 & 50.22 & 21.72 & 60.18 \\
& & AxMENDNet & 78.32 & 77.27 & 76.25 & 78.18 & 77.12 & 76.08 & 76.24 & 74.82 & 74.15 & 61.13 & 18.54 & 7.22 & 63.69 \\
& & EPSILON & 83.02 & 81.98 & 80.95 & 83.04 & 81.97 & 80.99 & 80.32 & 77.88 & 75.13 & 74.94 & 33.08 & 25.82 & \textbf{70.76} \\
\cline{2-16}
& \multirow{3}{*}{L2H} & AxVanDNN & 71.73 & 68.93 & 10.88 & 71.87 & 68.91 & 68.85 & 67.68 & 54.72 & 20.93 & 63.72 & 39.52 & 18.02 & 51.48 \\
& & AxMENDNet & 67.62 & 66.57 & 65.55 & 67.48 & 66.42 & 65.38 & 65.54 & 64.12 & 63.45 & 50.43 & 15.84 & 5.52 & 52.99 \\
& & EPSILON & 72.32 & 71.28 & 70.25 & 72.34 & 71.27 & 70.29 & 69.62 & 67.18 & 64.43 & 64.24 & 28.38 & 21.12 & \textbf{60.06} \\
\hline
\end{tabular}%
}
\end{table*}


\section{Experimental Results and Discussion}
%We conduct a comprehensive evaluation of our proposed fault detection and mitigation framework across various network architectures, datasets, and approximate computing scenarios. Our experiments aim to demonstrate the framework's effectiveness in enhancing the resilience of AxDNNs under different fault conditions.
We conduct a comprehensive evaluation of our proposed fault detection and mitigation framework across various network architectures, datasets, and approximate computing scenarios. The details are presented in the following subsections. 

\subsection{Experimental Setup}
We employ three widely-used datasets: MNIST, CIFAR-10, and CIFAR-100. For each dataset, we implement three popular DNN architectures: VGG16, WideResNet, and MobileNet, providing a broad spectrum of network complexities and design philosophies. To compare the performance of EPSILON with state-of-the-art, we choose the approximate versions of Vanilla CNN and MENDNet \cite{kundu2024mendnet}, denoted as \textcolor{blue}{AxVanDNN and AxMENDNet}, respectively. We selected MENDNet since it meets the JIT criteria and achieve state-of-the-art performance in AccDNNs. Furthermore, like EPSILON, MENDNet is built on top of the SDN network, ensuring a fair comparison.
% Our evaluation framework encompasses a diverse range of datasets and model architectures to ensure comprehensive validation. 
%We employ three widely-used datasets: MNIST, Fashion MNIST, and CIFAR-10, each presenting different levels of complexity and characteristics. For each dataset, we implement three popular DNN architectures: VGG16, WideResNet, and MobileNet, providing a broad spectrum of network complexities and design philosophies. While several AccDNN methods are designed for hardware fault detection and mitigation, we choose Vanilla AxDNN and approximate version of the MENDNet (AxMENDNet) \cite{kundu2024mendnet} for comparison with our approach, EPSILON. MENDNet is selected because it meets the JIT criteria and achieves state-of-the-art performance in AccDNN. Additionally, like EPSILON, MENDNet is built on top of the SDN network.
% Our framework builds upon \cite{kaya2019shallow}, which represent a sophisticated approach to neural network design by incorporating multiple classification exits throughout the network structure. This architecture enables efficient processing by allowing early termination when sufficient prediction confidence ($\max(F_i(x)) > \gamma$) is achieved at any exit $i$, while simultaneously providing inherent fault tolerance through redundant prediction paths. 

To leverage the approximate computing \textcolor{blue}{in VGG16, WideResNet, and MobileNet models}, we leverage a comprehensive selection of 8-bit signed approximate multipliers from Evoapproxlib \cite{mrazek2017evoapprox8b}. \textcolor{blue}{We focus on multipliers as they dominate energy consumption in DNNs compared to other arithmetic units, such as adders \cite{10028723}}. The chosen eight different multipliers are \texttt{KV6}, \texttt{KV8}, \texttt{KV9}, \texttt{KVP}, \texttt{L2J}, \texttt{L2H}, \texttt{L2N}, and \texttt{L2H}. These multipliers represent various points along the energy-accuracy trade-off spectrum, ranging from mostly accurate but less energy-efficient designs to aggressive approximations offering substantial energy savings \cite{8423431}. 

To thoroughly evaluate fault tolerance, we implement a strategic fault injection methodology. Faults are introduced at four carefully selected \textcolor{blue}{fault points (FP): FP1, FP2, FP3, and FP4} within the network, representing critical stages in the computational pipeline. These FPs were specifically chosen based on their demonstrated impact on network performance, as established through state-of-the-art \cite{kundu2024mendnet}. \textcolor{blue}{The FPs are evenly distributed throughout the network architecture, with FP1 at the first conv layer, FP4 at the second-to-last layer, and FP2-FP3 equally spaced between them. At each location, we inject faults at three different fault rates (FR) (10\%, 30\%, and 50\%), creating a comprehensive test matrix. These FPs and FRs aligned well with our theoretical analysis, which predicts a bounded error probability of miss detection as shown in Eq. \eqref{eq:equation11}. For instance, with our chosen confidence threshold $\gamma = 0.7$ and N = 4 exits (i.e FP1-FP4), the theoretical bound predicts maintainable accuracy even at 50\% fault rate when layer importance $\alpha_l$ is sufficiently high (\textgreater0.7).} Our implementation utilizes the AdaPT framework, built on Evoapproxlib for PyTorch, and employs Python 3.12, pyJoules, PyTorch 2.1, and CUDA 11.8, running on an NVIDIA RTX 2080 Ti GPU and an Intel Core i9 CPU with 64 GB of system RAM.


\section{Experimental Results and Discussion}

Our theoretical error bound $P_{error} \leq (1-\gamma)^N + \exp(-\alpha_l^2/2p)$, with N=4 exits and confidence threshold $\gamma=0.7$, effectively predicts the framework's behavior under various fault conditions. The empirical results strongly validate these predictions, with APS achieving 88.32\% accuracy at FP1 and maintaining >82\% accuracy through FP3 for WideRN with mul8s\_1KVP, even under challenging fault scenarios. This aligns with our theoretical bound which predicts a minimum accuracy of 81.45\% under these conditions ($(1-0.7)^4 + \exp(-0.7^2/2(0.5)) \approx 0.1855$). The observed performance degradation at FP4 (dropping to 11.12\% at 50\% fault rate) also follows our mathematical model, demonstrating the framework's predictable behavior across different fault scenarios while validating our theoretical foundations.
Our theoretical error bound $P_{error} \leq (1-\gamma)^N + \exp(-\alpha_l^2/2p)$, with N=4 exits and confidence threshold $\gamma=0.8$, effectively predicts the framework's behavior under various fault conditions. The empirical results strongly validate these predictions, with APS maintaining >80\% accuracy at FP1-FP3 even under 50\% fault rates for VGG16 with mul8s\_1KVP. The observed performance variations across fault points align with our mathematical model, particularly evident in the performance degradation at FP4 (accuracy dropping to 15-32\% at 50\% fault rate), demonstrating the framework's predictable behavior under different fault scenarios.
%In approximate computing, we leverage a comprehensive selection of approximate multipliers from Evoapproxlib \cite{mrazek2017evoapprox8b}. These multipliers represent various points along the energy-accuracy trade-off spectrum, ranging from highly accurate but less energy-efficient designs to aggressive approximations offering substantial energy savings \cite{8423431}. Our initial experimentation encompassed eight different multipliers: \texttt{KV6}, \texttt{KV8}, \texttt{KV9}, \texttt{KVP}, \texttt{L2J}, \texttt{L2H}, \texttt{L2N}, and \texttt{L2H}. To thoroughly evaluate fault tolerance, we implement a strategic fault injection methodology. Faults are introduced at four carefully selected points (FP1-FP4) within the network, representing critical stages in the computational pipeline. These fault points were specifically chosen based on their demonstrated impact on network performance, as established through previous research \cite{kundu2024mendnet}. At each location, we inject faults at three different rates (10\%, 30\%, and 50\%), creating a comprehensive test matrix.  Our implementation utilizes the AdaPT framework, built on Evoapproxlib for PyTorch, and employs Python 3.12, pyJoules, PyTorch 2.1, and CUDA 11.8, running on an NVIDIA RTX 2080 Ti GPU and an Intel Core i9 CPU with 64 GBs of system RAM.

% \subsection{Baseline Performance Analysis}
% To establish a foundation for evaluating EPSILON, we first assess the baseline performance of the selected models \emph{without faults}. Table \ref{tab:baseline_accuracy} presents the baseline accuracies for each combination of model architecture and approximate multiplier across the four datasets. The results in Table \ref{tab:baseline_accuracy} reveal several key insights. As expected, more accurate multipliers (e.g., \texttt{KV6}, \texttt{KV8}) generally yield higher baseline accuracies across all datasets and models. VGG16 and WideResNet exhibit relatively consistent performance across the more accurate multipliers on MNIST and CIFAR-10. In contrast, MobileNet shows higher sensitivity to the choice of the approximate multiplier, particularly evident in the significant accuracy drop for \texttt{L2J} and \texttt{L2H} on MNIST. We observe that Fashion MNIST consistently yields lower baseline accuracies than MNIST and CIFAR-10, suggesting that dataset characteristics significantly influence the model's resilience to approximation-induced errors. Least accurate multipliers (\texttt{L2N} and \texttt{L2H}) result in drastic accuracy reductions across all models and datasets, highlighting the critical trade-off between energy efficiency and accuracy in extreme approximate computing scenarios. These baseline results provide a crucial reference point for evaluating our framework's effectiveness in mitigating faults and maintaining accuracy in approximate computing environments. 

\begin{figure}[!t]
	\centering
	% \vspace{-0.01in}
        \includegraphics[width=1\linewidth]{Figs/inference_comparison.pdf}
	%\vspace{-0.16in}
	\caption{Average inference time (ms) for AxVanDNN, AxMENDNet, and EPSILON with KVP, L2J, and L2H multipliers on MNIST, CIFAR-10, and CIFAR-100 dataset}
	\label{fig:inference_aps}
	% \vspace{-0.2in}
\end{figure}

\subsection{EPSILON Performance Analysis: Fault Tolerance}
\label{sec:experiments}
%Table \ref{table_accuracy_combined} presents a comprehensive comparison of our APS framework against vanilla AxDNN and AxMENDNet, revealing several significant patterns and insights across different experimental configurations. The results demonstrate a consistent superior performance pattern for EPSILON across various test conditions. A particularly illustrative example can be found in the VGG16 architecture using the KVP multiplier, where EPSILON maintains an impressive 85.72\% accuracy at FP1 even under a severe 50\% fault rate. This stands in stark contrast to AxMENDNet's 79.08\% and AxDNN's dramatic decline to 18.84\% under the same conditions. Such performance differential underscores the effectiveness of our statistical pattern-based approach in both detecting and mitigating faults while maintaining network functionality. The impact of fault location emerges as a critical factor in performance degradation patterns. Our analysis reveals that while FP1 through FP3 demonstrate relatively stable performance under EPSILON, FP4 consistently presents more challenging conditions for all approaches. This pattern holds true across different architectures and approximation levels, though the magnitude of impact varies. The EPSILON framework shows particular strength in maintaining accuracy at the critical fault points FP1-FP3, where the preservation of network functionality is crucial for overall performance.
\textcolor{blue}{Due to space constraints, this section reports experimental results focusing on SA1 faults for CIFAR-10 dataset using three representative multipliers (KVP, L2J, and L2H), chosen to illustrate the spectrum of approximation impacts as shown in Table \ref{table_accuracy_combined}. Comprehensive results across the rest of the multipliers and datasets can be found here\footnote{Google Site URL goes here}.}
Table \ref{table_accuracy_combined} compares EPSILON with AxVanDNN and AxMENDNet \textcolor{blue}{under SA1 faults for the CIFAR-10 dataset. The results demonstrate a consistently superior performance pattern for EPSILON, and on average, it outperforms AxVanDNN and AxMENDNet across all FP and FR for all model-dataset-multiplier combinations}. For instance, in the VGG16 architecture using the KVP multiplier, EPSILON maintains an impressive 85.72\% accuracy at FP1 even under a severe 50\% fault rate. In contrast, AxMENDNet shows an accuracy of 79.08\%, and AxVanDNN shows an accuracy of only 18.84\% under the same conditions. Such performance differential underscores the effectiveness of our statistical pattern-based approach in both detecting and mitigating faults while maintaining network functionality. WideResNet exhibits particularly strong resilience at FP2 and FP3, suggesting that its architecture provides natural fault tolerance at these locations. MobileNet benefits significantly from our EPSILON framework's mitigation strategies while showing more uniform degradation across FPs and maintaining higher accuracy levels compared to AxVanDNN and AxMENDNet. \textcolor{blue}{These empirical results strongly validate our theoretical error-bound mathematical model. For example, with EPSILON achieving 88.32\% accuracy at FP1 and maintaining \textgreater 82\% accuracy through FP3 for WideRN with KVP, even under challenging fault scenarios. This aligns with our theoretical bound which predicts a minimum accuracy of 81.45\% under these conditions ($(1-0.7)^4 + \exp(-0.7^2/2(0.5)) \approx 0.1855$). The observed performance degradation at FP4 (dropping to 11.12\% at 50\% fault rate) also follows our mathematical model, demonstrating the framework's predictable behavior across different fault scenarios while validating our theoretical foundations.}

The relationship between approximation levels and fault tolerance reveals an interesting trend. As we progress from KVP to L2H, representing increasing levels of approximation, we observe a predictable decrease in baseline accuracy. However, the EPSILON framework consistently demonstrates smaller accuracy drops than AxVanDNN and AxMENDNet. This performance gap becomes particularly pronounced at higher FRs, highlighting EPSILON's effectiveness in managing the combined challenges of approximation and fault tolerance. The impact of fault location emerges as a critical factor in performance degradation patterns. Our analysis reveals that while FP1 through FP3 demonstrate relatively stable performance under EPSILON, FP4 consistently presents more challenging conditions for all approaches. This trend holds true across different architectures and approximation levels, though the magnitude of impact varies. The EPSILON framework shows particular strength in maintaining accuracy at the critical fault points FP1-FP3, where preserving network functionality is crucial for overall performance.
%Architecture-specific responses to faults present another fascinating dimension of our findings. The VGG16 architecture demonstrates remarkable consistency across different fault points, maintaining relatively stable performance even under increasing fault rates. WideResNet exhibits particularly strong resilience at FP2 and FP3, suggesting that its architecture provides natural fault tolerance at these locations. MobileNet, while showing more uniform degradation across fault points, benefits significantly from our EPSILON framework's mitigation strategies, maintaining higher accuracy levels compared to baseline approaches.The relationship between approximation levels and fault tolerance reveals complex interactions. As we progress from KVP to L2H, representing increasing levels of approximation, we observe a predictable decrease in baseline accuracy. However, the EPSILON framework consistently demonstrates smaller accuracy drops compared to both vanilla AxDNN and AxMENDNet. This performance gap becomes particularly pronounced at higher fault rates, highlighting EPSILON's effectiveness in managing the combined challenges of approximation and fault tolerance.



\subsection{EPSILON Performance Analysis: Inference Time}
%Our comprehensive evaluation reveals several profound insights into the effectiveness of the EPSILON framework and its implications for fault-tolerant approximate computing. The consistent superior performance of EPSILON across various test conditions validates our fundamental approach of using statistical patterns for fault detection and mitigation. By effectively distinguishing between approximation-induced variations and actual faults, the framework enables more precise and targeted mitigation strategies, resulting in better overall system reliability. The multi-exit architecture proves to be a particularly valuable component of our design. Beyond its primary function of enabling early exits for efficient processing, the architecture provides natural fault tolerance through its redundant paths \cite{kundu2024mendnet}. The confidence-based progression through the network allows for dynamic adaptation to both input complexity and fault conditions, contributing significantly to the framework's robustness.

\begin{figure}[!t]
	\centering
	\vspace{-0.01in}
        \includegraphics[width=1\linewidth]{Figs/energy_comparison.pdf}
	%\vspace{-0.16in}
	\caption{Comparison of relative energy consumption across algorithms and datasets}
	\label{fig:energy_aps}
	% \vspace{-0.2in}
\end{figure}

%Beyond accuracy considerations, we also evaluate the computational efficiency of our approach through inference time analysis, as shown in Fig \ref{fig:inference_aps}. The results demonstrate that EPSILON not only achieves superior fault tolerance but also maintains competitive inference times across all datasets and approximate multipliers. For instance, on CIFAR-10 with KVP, EPSILON achieves an average inference time of 180ms, compared to AxMENDNet's 187.21ms and vanilla AxDNN's 205.40ms. This difference is because AxDNN traverses through the complete network every time, while EPSILON and AxMENDNet terminate early if they meet the criteria, i.e., $\gamma$ for EPSILON while $\gamma$ and $\tau$ for AxMENDNet. This observation is inline with the existing studies \cite{kaya2019shallow, kundu2024mendnet}. However, the computational efficiency advantage of EPSILON over AxMENDNet becomes particularly apparent when examining the underlying mechanisms. While both frameworks utilize a multi-exit architecture, AxMENDNet's requirement to compute both confidence score ($\gamma$) and detection threshold ($\tau$) for each inference introduces additional overhead. Our measurements indicate that this dual computation accounts for approximately 28\% of AxMENDNet's total processing time. In contrast, EPSILON's streamlined approach of using only the confidence score ($\gamma$) combined with pre-computed statistical signatures reduces computational overhead while maintaining robust fault detection capabilities. This architectural difference explains the observed performance gap in inference times: EPSILON consistently achieves 22\% faster processing compared to AxMENDNet across all tested configurations. This efficiency advantage becomes more pronounced on simpler datasets like MNIST, where APS requires only 130ms compared to AxDNN's 168.41ms with the same multiplier. Interestingly, the performance gap widens with more aggressive approximation levels, as seen with L2H, where EPSILON maintains relatively stable inference times while both AxDNN and AxMENDNet show more significant slowdowns. This pattern suggests that our framework's multi-exit architecture and efficient statistical analysis effectively balance the overhead of fault detection with the benefits of early termination. The consistent time advantages across different approximate multipliers also indicate that EPSILON's pattern-based approach scales well with varying levels of hardware approximation, making it particularly suitable for real-world deployments where both reliability and computational efficiency are critical considerations.

In this section, we evaluate the computational efficiency of our approach through inference time analysis, as shown in Fig \ref{fig:inference_aps}. Our results demonstrate that in addition to superior fault tolerance, as shown in \textcolor{blue}{\ref{sec:experiments}}, EPSILON outperforms the state-of-the-art works in terms of inference times across all datasets and approximate multipliers. For instance, on CIFAR-10 with KVP, EPSILON achieves an average inference time of 180ms, compared to AxMENDNet's 187.21ms and vanilla AxDNN's 205.40ms. This difference is because AxVanDNN traverses through the complete network every time, while EPSILON and AxMENDNet terminate early if they meet the exit criteria, i.e., $\gamma$ for EPSILON while $\gamma$ and $\tau$ for AxMENDNet. This observation aligns with the existing studies \cite{kaya2019shallow, kundu2024mendnet}. However, the computational efficiency of EPSILON over AxMENDNet becomes particularly apparent when examining the underlying mechanisms. While both frameworks utilize a multi-exit architecture, AxMENDNet's requirement to compute both confidence score ($\gamma$) and detection threshold ($\tau$) for each inference that introduces additional overhead \textcolor{blue}{both in terms of latency and energy}. Our results indicate that this dual computation accounts for approximately 28\% of AxMENDNet's total processing time. In contrast, EPSILON's streamlined approach of using only the confidence score ($\gamma$) combined with pre-computed statistical signatures reduces computational overhead while maintaining robust fault detection capabilities. This architectural difference explains the observed performance gap in inference times: on average EPSILON consistently achieves 22\% faster processing than AxMENDNet on MNIST, CIFAR-10 and CIFAR-100 datsets with KVP, L2J and L2H multipliers, as shown in Fig \ref{fig:inference_aps}. This efficiency advantage is more pronounced on the MNIST datasets, where EPSILON requires only 130 ms compared to AxVanDNN's 168.41ms with the same multiplier, \textcolor{blue}{while the trends hold for other datasets as well}. Interestingly, the performance gap widens with more aggressive approximation levels, as seen with L2H, where EPSILON maintains relatively stable inference times while AxVanDNN and AxMENDNet show more significant slowdowns. This trend suggests that our framework's multi-exit architecture and efficient statistical analysis effectively balance the overhead of fault detection with the benefits of early termination. The consistent inference time advantages across different approximate multipliers also indicate that EPSILON's pattern-based approach scales well with varying levels of hardware approximation, making it particularly suitable for real-world deployments where both reliability and computational efficiency are critical considerations.

\subsection{EPSILON Performance Analysis: Energy Efficiency}
This section presents the energy consumption results (using the pyJoules library) of the EPSILON, AxMENDNet, and AxVanDNN frameworks, as shown in Fig \ref{fig:energy_aps}. Each inference is repeated 100 times to ensure statistical significance. \textcolor{blue}{For better representation, we normalized the results against the peak energy consumption of AxMENDNet on CIFAR-10 as the baseline}. As shown in \ref{fig:energy_aps}, EPSILON demonstrates superior energy efficiency, operating at 61.5--74.8\% of the baseline across all datasets. This represents a significant improvement over both AxMENDNet (90.5-100\%) and vanilla AxDNN (92.1-94.3\%). This relative analysis reveals that EPSILON consistently outperforms AxMENDNet by an average margin of 28.3\% and AxVanDNN by 26.7\%. This substantial efficiency gain can be attributed to EPSILON's adaptive early-exit strategy and targeted fault detection mechanism, which minimizes unnecessary computations while maintaining reliability. These results position EPSILON as a promising solution for energy-efficient approximate computing systems, particularly in resource-constrained environments.

%We conducted extensive energy consumption measurements across EPSILON, AxMENDNet, and vanilla AxDNN frameworks, with each inference repeated 100 times to ensure statistical significance. The measurements encompassed all implemented approximate multiplier configurations across MNIST, Fashion-MNIST, and CIFAR10 datasets and are shown in \ref{fig:energy_aps}. To ensure accuracy and reproducibility, energy consumption was measured using the pyJoules library, which allowed precise tracking of CPU power usage during the inference phase. Normalizing against the peak energy consumption (AxMENDNet on CIFAR10 as baseline), EPSILON demonstrated superior efficiency, operating at 61.5-74.8\% of the baseline across all datasets. This represents a significant improvement over both AxMENDNet (90.5-100\%) and vanilla AxDNN (92.1-94.3\%). The relative analysis reveals that EPSILON consistently outperforms AxMENDNet by an average margin of 28.3\% and vanilla AxDNN by 26.7\%. This substantial efficiency gain can be attributed to EPSILON's adaptive early-exit strategy and targeted fault detection mechanism, which effectively minimizes unnecessary computations while maintaining reliability. These results position EPSILON as a promising solution for energy-efficient approximate computing systems, particularly in resource-constrained environments. The practical implications of our results extend beyond mere performance metrics. The framework's ability to maintain accuracy under severe fault conditions while operating effectively across different approximation levels demonstrates its potential for real-world deployments. The consistent performance across various architectures suggests broad applicability, while the graceful degradation under increasing fault rates indicates robust fault management capabilities. Despite these significant achievements, our study also reveals areas for future investigation. The sharp accuracy drops observed at 50\% fault rate in FP4 suggest a potential limit to fault tolerance capabilities that warrants further research. Additionally, the varying effectiveness across different architectures indicates opportunities for architecture-specific optimizations. The trade-offs between fault tolerance and computational overhead remain an important consideration for practical implementations. These findings collectively demonstrate that EPSILON successfully achieves its primary objective of balancing the benefits of approximate computing with reliable operation. The framework's sophisticated approach to fault detection and mitigation, combined with its effective leveraging of multi-exit architecture benefits, represents a significant advancement in fault-tolerant approximate computing. This makes it particularly well-suited for energy-constrained AI applications where both reliability and efficiency are crucial considerations.



==> Sections/Sec5_Conclusion.tex <==

% \section{Conclusion}
% \label{sec:conclusion}
% %\vspace{-0.05in}


% % In this paper, we introduced a novel framework for fault detection and mitigation in deep neural networks (DNNs) on approximate hardware, enhancing existing state-of-the-art methods with statistical techniques for real-time operation. The experimental results demonstrate that our framework consistently outperforms the traditional state-of-the-art accurate DNN method across various datasets, fault rates, and approximate multipliers, achieving an improvement of up to 20\% in accuracy. This is achieved through the use of energy-based uncertainty quantification and the Anderson-Darling k-sample test, which together provide a powerful mechanism for distinguishing between approximation-induced errors and genuine hardware faults.
% % This work bridges a critical gap in deploying DNNs on approximate hardware, enhancing fault tolerance and energy efficiency. These insights contribute to designing future AI systems, enabling the benefits of approximate computing without compromising reliability.

% % Despite promising results, challenges remain in extreme fault conditions. Future work will refine detection strategies, explore alternative statistical methods, and extend the framework to other architectures and techniques. We also plan to integrate hardware-level fault tolerance for a comprehensive solution.
% \section{Conclusion}
% \label{sec:conclusion}
% We presented a novel framework for fault detection and mitigation in Approximate Deep Neural Networks (AxDNNs), aimed at enhancing reliability in energy-constrained AI systems. Leveraging advanced statistical techniques, including energy-based uncertainty quantification and the Anderson-Darling k-sample test, our method effectively distinguishes between approximation-induced errors and hardware faults in real-time.
% Experimental results show up to 66\% accuracy improvement over baseline methods across multiple datasets, fault rates, and architectures. The framework's adaptability to varying levels of hardware approximation highlights its potential for deployment in diverse energy-constrained environments. This work bridges a key gap in the deployment of DNNs on approximate hardware, offering a practical solution that balances fault tolerance and energy efficiency.

% While promising, further research is required to refine detection under extreme fault rates and extend applicability to dynamic approximation scenarios. Overall, our framework advances the field of approximate computing by providing a robust, energy-efficient solution for reliable AI systems.

\section{Conclusion}
\label{sec:conclusion}
This paper presented EPSILON, a novel framework for enhancing the reliability of Approximate Deep Neural Networks (AxDNNs) in energy-constrained environments. By leveraging multi-exit neural network architecture and statistical pattern analysis, EPSILON effectively distinguishes between intentional approximation effects and permanent hardware faults while maintaining computational efficiency. Our comprehensive evaluation across multiple datasets and network architectures demonstrates EPSILON's superior fault tolerance, inference time, and energy efficiency performance, outperforming other state-of-the-art approaches. 

Though EPSILON exhibits great prospects, our results also reveal some areas that demand further investigation. The accuracy decrease observed at 50\% fault rate at fault point FP4 suggests a potential limit to fault tolerance capabilities, which could be explored further. Additionally, the varying effectiveness of EPSILON across different architectures indicates opportunities for architecture-specific optimizations. In the future, we plan to investigate these areas and evaluate EPSILON on larger datasets.




%This paper presented EPSILON, a novel framework for enhancing the reliability of Approximate Deep Neural Networks (AxDNNs) in energy-constrained environments. By leveraging multi-exit neural network architecture and statistical pattern analysis, EPSILON effectively distinguishes between intentional approximation effects and harmful hardware faults while maintaining computational efficiency. Our comprehensive evaluation across multiple datasets and network architectures demonstrates EPSILON's superior performance. The framework achieves significant improvements over existing approaches, maintaining up to 66\% accuracy. Furthermore, EPSILON demonstrates improved computational efficiency, reducing inference time by up to 22\% compared to vanilla AxDNN while providing enhanced fault tolerance.The key innovations of EPSILON—statistical pattern-based fault detection, layer-importance aware analysis, and adaptive mitigation strategies—provide a robust foundation for reliable approximate computing. The framework's effectiveness across different approximate multipliers and fault scenarios demonstrates its practical applicability in real-world deployments where both energy efficiency and reliability are crucial. While promising, further research is required to refine detection under extreme fault rates and extend applicability to dynamic approximation scenarios. Overall, our framework advances the field of approximate computing by providing a robust, energy-efficient solution for reliable AI systems.


% While these results represent a significant advancement in fault-tolerant approximate computing, several challenges remain for future research. These include maintaining reliability under extreme fault rates (>50%) at deeper network layers, optimizing pattern signatures for dynamic approximation scenarios, and extending the framework to other approximation techniques beyond multiplier arrays. Nevertheless, APS establishes a promising direction for developing energy-efficient, fault-tolerant AI systems, particularly crucial for edge computing and IoT applications where resource constraints and reliability requirements intersect.


% \section{Experimental Results and Discussion}

% We conduct a comprehensive evaluation of our proposed framework across various network architectures, datasets, and approximate computing scenarios. The fault points (FP1-FP4) are evenly distributed throughout the network architecture, with FP1 at the first convolutional layer, FP4 at the second-to-last layer, and FP2-FP3 equally spaced between them, following standard practices in fault impact analysis \cite{kundu2024mendnet}. Our choice of fault rates (10%, 30%, and 50%) aligns with previous fault tolerance studies \cite{reagen2018ares, zhang2018thundervolt}, enabling direct comparison while validating our theoretical error bound $P_{error} \leq (1-\gamma)^N + \exp(-\alpha_l^2/2p)$ across different fault scenarios.

% \section{Experimental Results and Discussionss}

% We conduct a comprehensive evaluation of our proposed fault detection and mitigation framework across various network architectures, datasets, and approximate computing scenarios. The experimental parameters are carefully chosen to validate our theoretical error bounds and assess real-world performance. The fault rates (FR) of 10\%, 30\%, and 50\% are selected based on our theoretical analysis, which predicts a bounded error probability of $P_{error} \leq (1-\gamma)^N + \exp(-\alpha_l^2/2p)$. For instance, with our chosen confidence threshold $\gamma = 0.8$ and N = 3 exits, the theoretical bound predicts maintainable accuracy even at 50\% fault rate when layer importance $\alpha_l$ is sufficiently high (\textgreater0.7). Our empirical results strongly align with these predictions, as evidenced by APS maintaining \textgreater80\% accuracy at FP1-FP3 even under 50\% fault rates for VGG16 with mul8s\_1KVP.

% The selection of fault points (FP1-FP4) is guided by our layer-importance metric $\alpha_l$, with FP1 corresponding to early layers ($\alpha_l \approx 0.9$), FP2 and FP3 to middle layers ($\alpha_l \approx 0.7$), and FP4 to later layers ($\alpha_l \approx 0.5$). The observed performance degradation at FP4 (accuracy dropping to 15-32\% at 50\% fault rate) aligns with our theoretical bound, as the lower $\alpha_l$ value results in a higher error probability. This correlation between theoretical predictions and empirical results validates our mathematical framework while demonstrating its practical utility in predicting system behavior under various fault conditions.

% The chosen approximate multipliers (from mul8s\_1KV6 to mul8s\_1L12) represent a spectrum of approximation levels, with error rates ranging from 0.1\% to 15\%. These selections enable us to evaluate the framework's effectiveness across different energy-accuracy trade-offs while validating our theoretical assumptions about fault propagation and detection sensitivity. The experimental results demonstrate that our statistical pattern-matching approach effectively maintains the theoretical error bounds across all approximation levels, with performance degradation closely following predicted patterns based on the interaction between fault rates and approximation errors.

==> Sections/Sec8_Biograpahy.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figs/Ayesha.jpg}}]{Ayesha Siddique} received her B.Sc. degree in electrical engineering from the Army Public College of Management and Sciences, Rawalpindi, Pakistan, in 2013, and her M.S. degree in electrical engineering from the National University of Sciences and Technology (NUST), Islamabad, Pakistan, in 2018. She is currently pursuing her Ph.D. degree in electrical and computer engineering and working as a graduate research assistant at the Dependable Cyber-Physical Systems (DCPS) Laboratory in the University of Missouri-Columbia. She also served as a Research Associate and Design Engineer with the Center for Advanced Research in Engineering, Islamabad, Pakistan, from 2013 to 2017 after her Bachelor's degree. She is a recipient of the Richard Newton Fellowship at DAC 2018. Her research interests include formal analysis and verification of embedded systems, reliable and secure machine learning, energy-efficient systems, and digital image processing.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figs/DrHoque.png}}]{Khaza Anuarul Hoque} received his M.Sc. and Ph.D. degrees from the Department of Electrical and Computer Engineering at Concordia University, Montreal, Canada in 2011 and 2016, respectively. He is currently an Assistant Professor in the Department of Electrical Engineering and Computer Science at the University of Missouri-Columbia (MU) where he directs the Dependable Cyber-Physical Systems (DCPS) Laboratory. His research interests include Cyber-physical and Embedded Systems, Machine Learning, Cybersecurity, and Formal Methods. Before joining MU, he was an FRQNT postdoctoral fellow at the University of Oxford, UK. Dr. Hoque has received several awards and distinctions, including FQRNT Postdoctoral Fellowship Award (2016), FQRNT Doctoral Research Award (2012), and Best Paper Award in 8th IEEE International NEWCAS Conference (2011). He is a senior member of IEEE, and a member of ACM, AAAS, and IEEE Technical Committee on Cyber-Physical Systems (CPS). 
\end{IEEEbiography}

